Evaluation and Optimization of Leave-one-out Cross-validation for the Lasso

I develop an algorithm to produce the piecewise quadratic that computes leave-one-out cross-validation for the lasso as a function of its hyperparameter. The algorithm can be used to find exact hyperparameters that optimize leave-one-out cross-validation either globally or locally, and its practicality is demonstrated on real-world data sets. I also show how the algorithm can be modified to compute approximate leave-one-out cross-validation, making it suitable for larger data sets.

==> data/sim1-data.tex <==
0.0 & \phz0.0 & 0.280 & 0.00012 & 0.00314 & 0.00012 & 0.00314 & 0.00012 & 0.00314 \cr
0.1 & \phz3.3 & 0.258 & 0.00095 & 0.00280 & 0.00051 & 0.00282 & 0.00021 & 0.00285 \cr
0.2 & \phz5.3 & 0.240 & 0.00221 & 0.00265 & 0.00109 & 0.00265 & 0.00029 & 0.00267 \cr
0.3 & \phz7.2 & 0.226 & 0.00354 & 0.00255 & 0.00171 & 0.00253 & 0.00040 & 0.00254 \cr
0.4 & \phz9.1 & 0.215 & 0.00486 & 0.00250 & 0.00232 & 0.00246 & 0.00052 & 0.00245 \cr
0.5 & 10.9 & 0.206 & 0.00612 & 0.00250 & 0.00290 & 0.00244 & 0.00062 & 0.00242 \cr
0.6 & 12.6 & 0.200 & 0.00729 & 0.00254 & 0.00343 & 0.00246 & 0.00071 & 0.00244 \cr
0.7 & 14.4 & 0.197 & 0.00837 & 0.00263 & 0.00391 & 0.00254 & 0.00082 & 0.00251 \cr
0.8 & 16.1 & 0.195 & 0.00939 & 0.00277 & 0.00437 & 0.00266 & 0.00094 & 0.00264 \cr
0.9 & 17.7 & 0.196 & 0.01036 & 0.00295 & 0.00483 & 0.00284 & 0.00106 & 0.00283 \cr
1.0 & 19.3 & 0.198 & 0.01133 & 0.00317 & 0.00529 & 0.00307 & 0.00119 & 0.00307 \cr
1.1 & 20.8 & 0.202 & 0.01234 & 0.00345 & 0.00575 & 0.00334 & 0.00133 & 0.00336 \cr
1.2 & 22.2 & 0.207 & 0.01339 & 0.00376 & 0.00624 & 0.00366 & 0.00146 & 0.00371 \cr
1.3 & 23.5 & 0.212 & 0.01453 & 0.00413 & 0.00675 & 0.00403 & 0.00158 & 0.00411 \cr
1.4 & 24.7 & 0.218 & 0.01574 & 0.00454 & 0.00729 & 0.00445 & 0.00170 & 0.00456 \cr
1.5 & 25.8 & 0.225 & 0.01704 & 0.00499 & 0.00787 & 0.00491 & 0.00183 & 0.00507 \cr
1.6 & 26.8 & 0.232 & 0.01842 & 0.00549 & 0.00848 & 0.00543 & 0.00195 & 0.00563 \cr
1.7 & 27.8 & 0.240 & 0.01987 & 0.00604 & 0.00913 & 0.00601 & 0.00209 & 0.00625 \cr
1.8 & 28.7 & 0.248 & 0.02140 & 0.00664 & 0.00981 & 0.00664 & 0.00223 & 0.00693 \cr
1.9 & 29.5 & 0.256 & 0.02300 & 0.00729 & 0.01051 & 0.00734 & 0.00239 & 0.00769 \cr
2.0 & 30.3 & 0.265 & 0.02469 & 0.00799 & 0.01126 & 0.00810 & 0.00255 & 0.00853 \cr


==> figure/alo-comp/alo-cmd.tex <==
\draw (0.0, 1.0) .. controls (0.0031089745929078726, 1.0) and (0.006217949185815745, 1.0) .. (0.009326923778723618, 1.0)
	-- (0.009326923778723618, 0.9424951895631226) .. controls (0.010084532457759303, 0.9398091347885766) and (0.010842141136794988, 0.9371647292245138) .. (0.011599749815830673, 0.9345619728709341)
	-- (0.011599749815830673, 0.9366602896052927) .. controls (0.018779314421083826, 0.9032250524300172) and (0.025958879026336982, 0.8732717381982331) .. (0.03313844363159014, 0.8468003469099404)
	-- (0.03313844363159014, 0.8174665137647945) .. controls (0.0401641668364731, 0.7844244263787878) and (0.047189890041356056, 0.7550360364218189) .. (0.05421561324623901, 0.7293013438938877)
	-- (0.05421561324623901, 0.7226655950325616) .. controls (0.05670082079366587, 0.71275458502384) and (0.05918602834109271, 0.7033087415907651) .. (0.06167123588851956, 0.694328064733337)
	-- (0.06167123588851956, 0.7020383130639353) .. controls (0.061858351570195716, 0.7013557980117494) and (0.06204546725187188, 0.7006757246904639) .. (0.06223258293354803, 0.6999980931000788)
	-- (0.06223258293354803, 0.7081680289730838) .. controls (0.0714754528889599, 0.6751605050501932) and (0.08071832284437176, 0.6474076723054114) .. (0.08996119279978362, 0.624909530738738)
	-- (0.08996119279978362, 0.6208874650597743) .. controls (0.0960809611970541, 0.6072040689228737) and (0.10220072959432458, 0.5952435671151498) .. (0.10832049799159504, 0.585005959636603)
	-- (0.10832049799159504, 0.5828991589795319) .. controls (0.10875007649709406, 0.5821376183142823) and (0.10917965500259309, 0.5813837432523762) .. (0.10960923350809212, 0.5806375337938137)
	-- (0.10960923350809212, 0.5877786049830879) .. controls (0.10987557191128802, 0.5872932282833527) and (0.11014191031448392, 0.5868105766410358) .. (0.1104082487176798, 0.586330650056137)
	-- (0.1104082487176798, 0.5919741397783583) .. controls (0.11371011110346205, 0.5859351709792641) and (0.11701197348924432, 0.5802757221297901) .. (0.12031383587502659, 0.5749957932299361)
	-- (0.12031383587502659, 0.5789393589771726) .. controls (0.1203499143329166, 0.578881526822438) and (0.12038599279080661, 0.5788237353821519) .. (0.12042207124869665, 0.5787659846563139)
	-- (0.12042207124869665, 0.5859293994377991) .. controls (0.12139690086878513, 0.5843341641607248) and (0.12237173048887362, 0.5827662065207034) .. (0.12334656010896212, 0.5812255265177352)
	-- (0.12334656010896212, 0.5859448056130809) .. controls (0.12631886667397274, 0.5811593843012827) and (0.12929117323898337, 0.5766089457069417) .. (0.132263479803994, 0.5722934898300577)
	-- (0.132263479803994, 0.5777452223759837) .. controls (0.13232803062515222, 0.5776488927131146) and (0.13239258144631047, 0.5775526686986208) .. (0.13245713226746872, 0.5774565503325023)
	-- (0.13245713226746872, 0.5841917735060004) .. controls (0.13284493904239422, 0.583608334134816) and (0.1332327458173197, 0.583028449987358) .. (0.1336205525922452, 0.582452121063626)
	-- (0.1336205525922452, 0.5878474867746434) .. controls (0.1339807563550987, 0.5872771479690448) and (0.13434096011795219, 0.5867099933099706) .. (0.13470116388080566, 0.5861460227974209)
	-- (0.13470116388080566, 0.5926629112732886) .. controls (0.13723607721553263, 0.589241529601367) and (0.13977099055025963, 0.5859317305320858) .. (0.1423059038849866, 0.5827335140654447)
	-- (0.1423059038849866, 0.5865184934768765) .. controls (0.1425455468083536, 0.5861712720225813) and (0.1427851897317206, 0.5858251222926546) .. (0.1430248326550876, 0.5854800442870964)
	-- (0.1430248326550876, 0.5912829841570942) .. controls (0.14491918992090821, 0.5884230281565692) and (0.14681354718672882, 0.5856322753041204) .. (0.14870790445254942, 0.5829107255997481)
	-- (0.14870790445254942, 0.5890316301873959) .. controls (0.14879999878794922, 0.5889122611412453) and (0.14889209312334903, 0.5887930220843381) .. (0.14898418745874883, 0.5886739130166743)
	-- (0.14898418745874883, 0.5955940847703127) .. controls (0.14953421933483504, 0.5948123044702108) and (0.15008425121092128, 0.5940354701132282) .. (0.1506342830870075, 0.5932635816993647)
	-- (0.1506342830870075, 0.6001009335803488) .. controls (0.15195635701282867, 0.5982287217513458) and (0.15327843093864985, 0.5963843303916911) .. (0.15460050486447102, 0.5945677595013851)
	-- (0.15460050486447102, 0.6006430660204602) .. controls (0.15658660811129677, 0.5978387166093231) and (0.1585727113581225, 0.5950978454281702) .. (0.16055881460494825, 0.5924204524770018)
	-- (0.16055881460494825, 0.5995865904572156) .. controls (0.16231415201901594, 0.5972478794060841) and (0.16406948943308364, 0.5949560350747573) .. (0.16582482684715133, 0.5927110574632353)
	-- (0.16582482684715133, 0.5990266710397629) .. controls (0.1721275220649221, 0.5912501262850042) and (0.1784302172826929, 0.5840089342822848) .. (0.1847329125004637, 0.5773030950316047)
	-- (0.1847329125004637, 0.5834519749791228) .. controls (0.18726189359151701, 0.580664265563645) and (0.1897908746825703, 0.5779616222543971) .. (0.1923198557736236, 0.5753440450513789)
	-- (0.1923198557736236, 0.583663839624812) .. controls (0.19270225765007595, 0.5832655120412287) and (0.1930846595265283, 0.582868992672959) .. (0.19346706140298064, 0.582474281520003)
	-- (0.19346706140298064, 0.5895536182293158) .. controls (0.19530219208054372, 0.5876916065812856) and (0.1971373227581068, 0.5858673375538093) .. (0.19897245343566988, 0.5840808111468866)
	-- (0.19897245343566988, 0.5900341714905087) .. controls (0.2002396119201627, 0.588684172304418) and (0.2015067704046556, 0.5873535113738084) .. (0.2027739288891484, 0.5860421886986797)
	-- (0.2027739288891484, 0.594581065282892) .. controls (0.2032384614060752, 0.5941034996643094) and (0.203702993923002, 0.5936284261691287) .. (0.20416752643992883, 0.5931558447973502)
	-- (0.20416752643992883, 0.599218064656757) .. controls (0.206255486684769, 0.597100959518074) and (0.2083434469296092, 0.5950330535155699) .. (0.2104314071744494, 0.593014346649245)
	-- (0.2104314071744494, 0.5993561964688885) .. controls (0.21354559162826736, 0.5964665641001505) and (0.21665977608208534, 0.5936723437710715) .. (0.2197739605359033, 0.590973535481651)
	-- (0.2197739605359033, 0.5977700719601349) .. controls (0.21997059737511557, 0.5975943313545574) and (0.22016723421432782, 0.5974189539716587) .. (0.22036387105354008, 0.5972439398114386)
	-- (0.22036387105354008, 0.6045520554392936) .. controls (0.22265105298588425, 0.6023806262619457) and (0.22493823491822842, 0.6002616327459434) .. (0.2272254168505726, 0.5981950748912865)
	-- (0.2272254168505726, 0.6066785648678638) .. controls (0.22937498808971543, 0.6047769316150761) and (0.23152455932885826, 0.6029182088215878) .. (0.2336741305680011, 0.601102396487399)
	-- (0.2336741305680011, 0.6095184497277136) .. controls (0.23610070658537452, 0.607319553076021) and (0.23852728260274791, 0.6051782412227968) .. (0.24095385862012134, 0.6030945141680409)
	-- (0.24095385862012134, 0.6097658325125972) .. controls (0.24113814342946194, 0.6096095106866327) and (0.24132242823880257, 0.6094535077189598) .. (0.24150671304814322, 0.6092978236095782)
	-- (0.24150671304814322, 0.6163265563193191) .. controls (0.24564548182561713, 0.6128429210476265) and (0.24978425060309106, 0.6095105037664544) .. (0.253923019380565, 0.6063293044758031)
	-- (0.253923019380565, 0.6130908790234009) .. controls (0.25576503559845754, 0.6116509258289793) and (0.25760705181635, 0.6102401990534944) .. (0.25944906803424256, 0.6088586986969462)
	-- (0.25944906803424256, 0.6149261165462585) .. controls (0.2601414982773786, 0.6145111541089714) and (0.2608339285205146, 0.6140986933307311) .. (0.2615263587636507, 0.6136887342115377)
	-- (0.2615263587636507, 0.6228067300077839) .. controls (0.2621835940567589, 0.6223075876820143) and (0.262840829349867, 0.6218111535595435) .. (0.2634980646429752, 0.6213174276403711)
	-- (0.2634980646429752, 0.6294017594987762) .. controls (0.2683621041420661, 0.6254826510717407) and (0.27322614364115705, 0.6217204476188924) .. (0.2780901831402479, 0.6181151491402314)
	-- (0.2780901831402479, 0.6258021886653203) .. controls (0.2796274195354873, 0.6246651933982215) and (0.2811646559307267, 0.623543689245817) .. (0.2827018923259661, 0.6224376762081067)
	-- (0.2827018923259661, 0.628745924610077) .. controls (0.2835856321152991, 0.6281350007323769) and (0.28446937190463206, 0.6275286596778727) .. (0.28535311169396504, 0.6269269014465644)
	-- (0.28535311169396504, 0.6345727191032849) .. controls (0.28568674697744856, 0.6343442538217997) and (0.286020382260932, 0.6341163890081114) .. (0.2863540175444155, 0.6338891246622202)
	-- (0.2863540175444155, 0.6419433699049778) .. controls (0.29286805385490694, 0.6371555173083059) and (0.2993820901653984, 0.6326098022057676) .. (0.3058961264758898, 0.6283062245973631)
	-- (0.3058961264758898, 0.6349072203978) .. controls (0.30632280570713777, 0.634622380716999) and (0.3067494849383858, 0.6343385344721605) .. (0.3071761641696338, 0.6340556816632846)
	-- (0.3071761641696338, 0.6434514085739869) .. controls (0.308055954771515, 0.6428729079328626) and (0.30893574537339613, 0.6422982843282551) .. (0.30981553597527733, 0.6417275377601647)
	-- (0.30981553597527733, 0.6492627211461786) .. controls (0.3113209369068347, 0.64822907320865) and (0.3128263378383921, 0.6472070438575115) .. (0.31433173876994946, 0.6461966330927629)
	-- (0.31433173876994946, 0.657254285666245) .. controls (0.31445769501777265, 0.6571709325684303) and (0.31458365126559584, 0.6570876540431397) .. (0.31470960751341903, 0.6570044500903733)
	-- (0.31470960751341903, 0.6670324566866891) .. controls (0.3160588901742894, 0.6660780676471669) and (0.3174081728351598, 0.6651326870585403) .. (0.3187574554960302, 0.6641963149208092)
	-- (0.3187574554960302, 0.6736965255627015) .. controls (0.3191097663531292, 0.6734599057471068) and (0.31946207721022823, 0.6732238427262788) .. (0.31981438806732726, 0.6729883365002178)
	-- (0.31981438806732726, 0.6824186683694966) .. controls (0.3250433258186711, 0.678611402338445) and (0.33027226357001493, 0.6749378797880081) .. (0.3355012013213588, 0.6713981007181863)
	-- (0.3355012013213588, 0.6646862218034576) .. controls (0.3384492718212808, 0.6627767825686649) and (0.3413973423212029, 0.6609068143421947) .. (0.3443454128211249, 0.6590763171240468)
	-- (0.3443454128211249, 0.6662404294647598) .. controls (0.3461977976431066, 0.6650430142438524) and (0.34805018246508834, 0.6638616002245888) .. (0.34990256728707003, 0.6626961874069691)
	-- (0.34990256728707003, 0.6722262904801041) .. controls (0.35097665265114175, 0.6715410479956214) and (0.35205073801521336, 0.6708611321327479) .. (0.353124823379285, 0.6701865428914834)
	-- (0.353124823379285, 0.6780699733020437) .. controls (0.35555297007425535, 0.6765527768363897) and (0.3579811167692256, 0.6750621811494935) .. (0.36040926346419594, 0.673598186241355)
	-- (0.36040926346419594, 0.6831189940859741) .. controls (0.3606271675862494, 0.682996389878004) and (0.3608450717083029, 0.6828739645923441) .. (0.36106297583035635, 0.6827517182289944)
	-- (0.36106297583035635, 0.6928321515755577) .. controls (0.3645626061370407, 0.6905888244164287) and (0.36806223644372515, 0.6883996846145526) .. (0.37156186675040953, 0.6862647321699297)
	-- (0.37156186675040953, 0.6752045939121909) .. controls (0.3720613792329752, 0.6749176074224782) and (0.37256089171554085, 0.674631639164149) .. (0.37306040419810654, 0.6743466891372031)
	-- (0.37306040419810654, 0.6852813252787544) .. controls (0.3740911286670354, 0.6846660718530245) and (0.37512185313596424, 0.6840553641396006) .. (0.3761525776048931, 0.6834492021384826)
	-- (0.3761525776048931, 0.673033995416643) .. controls (0.3763541222267123, 0.6729331930849066) and (0.37655566684853137, 0.6728325202386465) .. (0.3767572114703505, 0.6727319768778627)
	-- (0.3767572114703505, 0.6844164885645084) .. controls (0.38102925420525074, 0.6820704829685841) and (0.38530129694015103, 0.6797845375515286) .. (0.38957333967505126, 0.6775586523133419)
	-- (0.38957333967505126, 0.6866655085573165) .. controls (0.3906837855646794, 0.6860669234298912) and (0.39179423145430764, 0.6854723494253426) .. (0.39290467734393586, 0.6848817865436709)
	-- (0.39290467734393586, 0.6940048480549248) .. controls (0.3943861593578793, 0.6931676249181813) and (0.39586764137182273, 0.6923379197966618) .. (0.39734912338576617, 0.6915157326903665)
	-- (0.39734912338576617, 0.7010861327263525) .. controls (0.39998202765630825, 0.6996956199095389) and (0.4026149319268504, 0.6983262238173933) .. (0.40524783619739246, 0.6969779444499155)
	-- (0.40524783619739246, 0.7088940543607344) .. controls (0.4076023988147729, 0.707613647301826) and (0.4099569614321533, 0.7063508203379417) .. (0.41231152404953375, 0.7051055734690814)
	-- (0.41231152404953375, 0.7132783352492997) .. controls (0.41708720164056023, 0.7109319864045993) and (0.4218628792315866, 0.7086459949319529) .. (0.4266385568226131, 0.7064203608313602)
	-- (0.4266385568226131, 0.7192849866757093) .. controls (0.4278999676261074, 0.7186477427859623) and (0.4291613784296016, 0.7180149542448928) .. (0.43042278923309585, 0.7173866210525006)
	-- (0.43042278923309585, 0.7290955543271002) .. controls (0.4315264247233843, 0.7285534391055387) and (0.4326300602136728, 0.7280144685568333) .. (0.43373369570396125, 0.727478642680984)
	-- (0.43373369570396125, 0.7357784046390564) .. controls (0.4349224272999106, 0.735197217504113) and (0.43611115889585994, 0.7346194636621743) .. (0.4372998904918093, 0.7340451431132404)
	-- (0.4372998904918093, 0.7452102990874154) .. controls (0.44424096012838704, 0.7418528277382277) and (0.4511820297649648, 0.7386033651714937) .. (0.4581230994015426, 0.7354619113872136)
	-- (0.4581230994015426, 0.7439388169986075) .. controls (0.4599997250794202, 0.743029501471563) and (0.46187635075729777, 0.7421286433672798) .. (0.4637529764351754, 0.7412362426857579)
	-- (0.4637529764351754, 0.750733253500263) .. controls (0.4680005168279545, 0.7487728816074335) and (0.4722480572207336, 0.7468523713341907) .. (0.47649559761351273, 0.7449717226805346)
	-- (0.47649559761351273, 0.7576470801910623) .. controls (0.47730779358671394, 0.7572607641483842) and (0.4781199895599152, 0.7568760403181204) .. (0.4789321855331165, 0.7564929087002706)
	-- (0.4789321855331165, 0.7462782909785649) .. controls (0.48163674942722723, 0.7450927302399794) and (0.484341313321338, 0.7439226520932188) .. (0.4870458772154487, 0.7427680565382837)
	-- (0.4870458772154487, 0.7536975682958713) .. controls (0.4879577262342575, 0.7532756996524801) and (0.4888695752530664, 0.7528557298676032) .. (0.48978142427187527, 0.7524376589412407)
	-- (0.48978142427187527, 0.7398313220185911) .. controls (0.4957040969698785, 0.7371710172246245) and (0.5016267696678818, 0.7345890425100761) .. (0.507549442365885, 0.7320853978749456)
	-- (0.507549442365885, 0.742795923597198) .. controls (0.5078481191496669, 0.7426686586330343) and (0.5081467959334488, 0.7425415944669267) .. (0.5084454727172307, 0.7424147310988755)
	-- (0.5084454727172307, 0.7543859474332446) .. controls (0.5091568423901689, 0.7540883512546284) and (0.5098682120631071, 0.7537918423442539) .. (0.5105795817360452, 0.753496420702121)
	-- (0.5105795817360452, 0.7647877115266252) .. controls (0.5108639327021247, 0.7646646324037037) and (0.5111482836682042, 0.7645417300833457) .. (0.5114326346342837, 0.7644190045655509)
	-- (0.5114326346342837, 0.7781941285888857) .. controls (0.512057294267584, 0.7779250997558854) and (0.5126819539008843, 0.7776568920889209) .. (0.5133066135341846, 0.777389505587992)
	-- (0.5133066135341846, 0.7904527097926974) .. controls (0.5168879457983934, 0.7888998976247654) and (0.5204692780626021, 0.7873745227994522) .. (0.5240506103268109, 0.7858765853167576)
	-- (0.5240506103268109, 0.7958899814956704) .. controls (0.525535111412402, 0.795264711464471) and (0.5270196124979931, 0.7946441183469903) .. (0.5285041135835842, 0.7940282021432286)
	-- (0.5285041135835842, 0.8060264542491046) .. controls (0.5305313840678376, 0.8051703363918847) and (0.5325586545520912, 0.8043230482843126) .. (0.5345859250363446, 0.8034845899263878)
	-- (0.5345859250363446, 0.815146014910074) .. controls (0.5352747669410154, 0.8148544587115849) and (0.5359636088456862, 0.814563944355435) .. (0.536652450750357, 0.814274471841624)
	-- (0.536652450750357, 0.8272265389910236) .. controls (0.5504044031516475, 0.8213394448202643) and (0.5641563555529381, 0.8158684473345698) .. (0.5779083079542287, 0.81081354653394)
	-- (0.5779083079542287, 0.8210952302949158) .. controls (0.5801694843108051, 0.8202551340547403) and (0.5824306606673816, 0.8194265367696559) .. (0.584691837023958, 0.8186094384396629)
	-- (0.584691837023958, 0.8067999501422809) .. controls (0.5850873215192897, 0.8066621334640538) and (0.5854828060146214, 0.8065246481704169) .. (0.5858782905099532, 0.8063874942613706)
	-- (0.5858782905099532, 0.8183870562315934) .. controls (0.5880486942021774, 0.8176237091143543) and (0.5902190978944015, 0.8168702410559253) .. (0.5923895015866256, 0.8161266520563063)
	-- (0.5923895015866256, 0.8275380190362334) .. controls (0.5933141002436046, 0.8272053517656733) and (0.5942386989005837, 0.8268745440920634) .. (0.5951632975575626, 0.8265455960154037)
	-- (0.5951632975575626, 0.8409671517128617) .. controls (0.600887942682514, 0.8390137763457785) and (0.6066125878074653, 0.8371250853109542) .. (0.6123372329324167, 0.8353010786083889)
	-- (0.6123372329324167, 0.8489481118178581) .. controls (0.6130092490241426, 0.8487308636238741) and (0.6136812651158685, 0.8485144845144761) .. (0.6143532812075945, 0.848298974489664)
	-- (0.6143532812075945, 0.8671828577815888) .. controls (0.6177741210389923, 0.8660098707717522) and (0.6211949608703901, 0.8648608604545495) .. (0.6246158007017879, 0.8637358268299805)
	-- (0.6246158007017879, 0.876770229090982) .. controls (0.6340015017277171, 0.8738812340168481) and (0.6433872027536462, 0.8711492197627468) .. (0.6527729037795753, 0.868574186328678)
	-- (0.6527729037795753, 0.881157604697078) .. controls (0.6532551900810797, 0.8810240802001682) and (0.6537374763825843, 0.8808909466676675) .. (0.6542197626840888, 0.8807582040995757)
	-- (0.6542197626840888, 0.9018780041004206) .. controls (0.6579912741339918, 0.9008112013943302) and (0.6617627855838949, 0.89976727794082) .. (0.665534297033798, 0.8987462337398898)
	-- (0.665534297033798, 0.9118836803191135) .. controls (0.680422671053875, 0.9077556436769479) and (0.6953110450739519, 0.9039860107987994) .. (0.710199419094029, 0.9005747816846678)
	-- (0.710199419094029, 0.9158888629996343) .. controls (0.7138854321574809, 0.9150311190099878) and (0.717571445220933, 0.9141958835009023) .. (0.7212574582843849, 0.9133831564723778)
	-- (0.7212574582843849, 0.9260896072253137) .. controls (0.7231456268811578, 0.9256920322039623) and (0.7250337954779306, 0.9252997365848417) .. (0.7269219640747034, 0.9249127203679512)
	-- (0.7269219640747034, 0.9428705572664426) .. controls (0.7305177815365222, 0.9420616703279098) and (0.7341135989983409, 0.9412731320221528) .. (0.7377094164601598, 0.9405049423491718)
	-- (0.7377094164601598, 0.9571887920277214) .. controls (0.7463565686030001, 0.9552803770335262) and (0.7550037207458407, 0.9534900351057971) .. (0.763650872888681, 0.9518177662445341)
	-- (0.763650872888681, 0.9697540286341902) .. controls (0.765436107302756, 0.9694073858538352) and (0.767221341716831, 0.9690656043559033) .. (0.7690065761309058, 0.9687286841403946)
	-- (0.7690065761309058, 0.985187398506081) .. controls (0.7715685076011496, 0.9846902393344172) and (0.7741304390713932, 0.9842025279679549) .. (0.7766923705416371, 0.9837242644066935)
	-- (0.7766923705416371, 1.001194151451796) .. controls (0.7821125867883745, 1.0001300880169766) and (0.7875328030351116, 0.999108643467889) .. (0.792953019281849, 0.9981298178045337)
	-- (0.792953019281849, 1.0158325547320584) .. controls (0.8129813066603195, 1.0119986130152656) and (0.8330095940387903, 1.0088180037983836) .. (0.8530378814172608, 1.006290727081412)
	-- (0.8530378814172608, 0.9898493553122281) .. controls (0.859896564810497, 0.9890797879647002) and (0.8667552482037333, 0.9883756339169543) .. (0.8736139315969697, 0.9877368931689903)
	-- (0.8736139315969697, 1.0041967724729237) .. controls (0.8759633160437523, 1.003964193469939) and (0.8783127004905349, 1.0037400206285023) .. (0.8806620849373175, 1.0035242539486133)
	-- (0.8806620849373175, 0.9832892012512021) .. controls (0.886867466089884, 0.9828048853251483) and (0.8930728472424505, 0.982368438123465) .. (0.8992782283950169, 0.9819798596461523)
	-- (0.8992782283950169, 0.9973108030242579) .. controls (0.9070082156145383, 0.9967709937428364) and (0.9147382028340596, 0.9963125395917894) .. (0.9224681900535808, 0.9959354405711174)
	-- (0.9224681900535808, 1.015416856970325) .. controls (0.9257332677392704, 1.0152698883936615) and (0.92899834542496, 1.0151385382723972) .. (0.9322634231106496, 1.0150228066065319)
	-- (0.9322634231106496, 0.9947083105039808) .. controls (0.9324539094198541, 0.994701812548191) and (0.9326443957290584, 0.9946953645512732) .. (0.9328348820382629, 0.9946889665132276)
	-- (0.9328348820382629, 1.0147269181195997) .. controls (0.9334206412442843, 1.0147099145535006) and (0.9340064004503055, 1.0146933158312255) .. (0.9345921596563267, 1.0146771219527742)
	-- (0.9345921596563267, 1.0369841128677892) .. controls (0.9421675936134503, 1.0366799693573254) and (0.9497430275705738, 1.0364493737847076) .. (0.9573184615276973, 1.0362923261499357)
	-- (0.9573184615276973, 1.0600574013382134) .. controls (0.9582871607027179, 1.0600387444264283) and (0.9592558598777383, 1.060021143878607) .. (0.9602245590527588, 1.0600045996947491)
	-- (0.9602245590527588, 1.083155749892645) .. controls (0.9670213246077533, 1.0830034703015416) and (0.9738180901627478, 1.0829092287798459) .. (0.9806148557177423, 1.0828730253275578)
	-- (0.9806148557177423, 1.1073791012037701) .. controls (0.985437410073277, 1.1073509714536618) and (0.9902599644288117, 1.1073517006455564) .. (0.9950825187843464, 1.1073812887794543)
	-- (0.9950825187843464, 1.1322896534764273) .. controls (0.9959922932780054, 1.1322994992422497) and (0.9969020677716646, 1.13231043044481) .. (0.9978118422653237, 1.1323224470841082)
	-- (0.9978118422653237, 1.1099117060458559) .. controls (0.9985412281768825, 1.1099226288719402) and (0.9992706140884413, 1.1099341578371202) .. (1.0, 1.1099462929413955)
	;


==> figure/alo-comp/lo-cmd.tex <==
\draw (0.0, 1.0) .. controls (0.002, 1.0) and (0.004, 1.0) .. (0.006, 1.0)
	-- (0.006, 0.952) .. controls (0.006, 0.95) and (0.007, 0.948) .. (0.007, 0.947)
	-- (0.007, 0.942) .. controls (0.008, 0.942) and (0.008, 0.942) .. (0.008, 0.941)
	-- (0.008, 0.937) .. controls (0.009, 0.936) and (0.009, 0.936) .. (0.009, 0.936)
	-- (0.009, 0.933) .. controls (0.009, 0.933) and (0.01, 0.933) .. (0.01, 0.933)
	-- (0.01, 0.93) .. controls (0.011, 0.93) and (0.011, 0.93) .. (0.011, 0.93)
	-- (0.011, 0.926) .. controls (0.012, 0.926) and (0.012, 0.926) .. (0.012, 0.926)
	-- (0.012, 0.922) .. controls (0.013, 0.922) and (0.013, 0.922) .. (0.013, 0.922)
	-- (0.013, 0.918) .. controls (0.013, 0.917) and (0.014, 0.917) .. (0.014, 0.917)
	-- (0.014, 0.915) .. controls (0.014, 0.914) and (0.014, 0.912) .. (0.015, 0.91)
	-- (0.015, 0.91) .. controls (0.016, 0.905) and (0.016, 0.901) .. (0.017, 0.896)
	-- (0.017, 0.896) .. controls (0.018, 0.893) and (0.018, 0.89) .. (0.019, 0.887)
	-- (0.019, 0.884) .. controls (0.021, 0.874) and (0.023, 0.863) .. (0.024, 0.854)
	-- (0.024, 0.852) .. controls (0.025, 0.849) and (0.026, 0.846) .. (0.026, 0.842)
	-- (0.026, 0.842) .. controls (0.027, 0.84) and (0.027, 0.837) .. (0.028, 0.835)
	-- (0.028, 0.831) .. controls (0.028, 0.83) and (0.029, 0.829) .. (0.029, 0.829)
	-- (0.029, 0.826) .. controls (0.029, 0.825) and (0.03, 0.824) .. (0.03, 0.823)
	-- (0.03, 0.82) .. controls (0.03, 0.82) and (0.03, 0.82) .. (0.031, 0.82)
	-- (0.031, 0.815) .. controls (0.031, 0.815) and (0.032, 0.815) .. (0.032, 0.815)
	-- (0.032, 0.811) .. controls (0.033, 0.811) and (0.033, 0.81) .. (0.033, 0.81)
	-- (0.033, 0.806) .. controls (0.034, 0.806) and (0.034, 0.806) .. (0.034, 0.806)
	-- (0.034, 0.802) .. controls (0.034, 0.802) and (0.035, 0.802) .. (0.035, 0.802)
	-- (0.035, 0.799) .. controls (0.035, 0.798) and (0.035, 0.798) .. (0.036, 0.798)
	-- (0.036, 0.797) .. controls (0.036, 0.796) and (0.036, 0.794) .. (0.037, 0.793)
	-- (0.037, 0.789) .. controls (0.037, 0.789) and (0.037, 0.789) .. (0.038, 0.789)
	-- (0.038, 0.785) .. controls (0.039, 0.784) and (0.039, 0.783) .. (0.039, 0.782)
	-- (0.039, 0.779) .. controls (0.042, 0.769) and (0.044, 0.759) .. (0.046, 0.749)
	-- (0.046, 0.749) .. controls (0.046, 0.748) and (0.046, 0.747) .. (0.047, 0.745)
	-- (0.047, 0.743) .. controls (0.047, 0.742) and (0.048, 0.741) .. (0.048, 0.74)
	-- (0.048, 0.737) .. controls (0.049, 0.737) and (0.049, 0.737) .. (0.049, 0.736)
	-- (0.049, 0.735) .. controls (0.049, 0.733) and (0.05, 0.732) .. (0.05, 0.731)
	-- (0.05, 0.728) .. controls (0.05, 0.728) and (0.05, 0.728) .. (0.051, 0.728)
	-- (0.051, 0.725) .. controls (0.051, 0.724) and (0.052, 0.724) .. (0.052, 0.724)
	-- (0.052, 0.721) .. controls (0.052, 0.721) and (0.053, 0.721) .. (0.053, 0.721)
	-- (0.053, 0.717) .. controls (0.054, 0.717) and (0.054, 0.717) .. (0.054, 0.717)
	-- (0.054, 0.714) .. controls (0.054, 0.714) and (0.054, 0.714) .. (0.055, 0.714)
	-- (0.055, 0.711) .. controls (0.055, 0.711) and (0.055, 0.711) .. (0.056, 0.711)
	-- (0.056, 0.708) .. controls (0.057, 0.708) and (0.057, 0.707) .. (0.057, 0.707)
	-- (0.057, 0.705) .. controls (0.057, 0.705) and (0.058, 0.705) .. (0.058, 0.705)
	-- (0.058, 0.702) .. controls (0.058, 0.702) and (0.058, 0.702) .. (0.059, 0.702)
	-- (0.059, 0.699) .. controls (0.059, 0.699) and (0.059, 0.699) .. (0.06, 0.699)
	-- (0.06, 0.696) .. controls (0.06, 0.696) and (0.061, 0.696) .. (0.061, 0.696)
	-- (0.061, 0.694) .. controls (0.061, 0.694) and (0.061, 0.694) .. (0.062, 0.694)
	-- (0.062, 0.692) .. controls (0.063, 0.692) and (0.063, 0.692) .. (0.063, 0.692)
	-- (0.063, 0.69) .. controls (0.064, 0.69) and (0.064, 0.69) .. (0.064, 0.69)
	-- (0.064, 0.687) .. controls (0.065, 0.687) and (0.065, 0.687) .. (0.065, 0.687)
	-- (0.065, 0.685) .. controls (0.066, 0.685) and (0.066, 0.685) .. (0.066, 0.685)
	-- (0.066, 0.682) .. controls (0.066, 0.682) and (0.066, 0.682) .. (0.067, 0.682)
	-- (0.067, 0.68) .. controls (0.067, 0.68) and (0.067, 0.679) .. (0.068, 0.679)
	-- (0.068, 0.676) .. controls (0.068, 0.676) and (0.068, 0.676) .. (0.069, 0.676)
	-- (0.069, 0.674) .. controls (0.069, 0.674) and (0.069, 0.673) .. (0.07, 0.672)
	-- (0.07, 0.67) .. controls (0.07, 0.67) and (0.07, 0.67) .. (0.071, 0.669)
	-- (0.071, 0.667) .. controls (0.071, 0.667) and (0.071, 0.667) .. (0.072, 0.666)
	-- (0.072, 0.664) .. controls (0.072, 0.664) and (0.072, 0.664) .. (0.073, 0.663)
	-- (0.073, 0.662) .. controls (0.073, 0.661) and (0.073, 0.66) .. (0.074, 0.66)
	-- (0.074, 0.66) .. controls (0.074, 0.658) and (0.075, 0.656) .. (0.076, 0.654)
	-- (0.076, 0.652) .. controls (0.076, 0.651) and (0.076, 0.651) .. (0.077, 0.65)
	-- (0.077, 0.65) .. controls (0.078, 0.646) and (0.079, 0.641) .. (0.081, 0.637)
	-- (0.081, 0.637) .. controls (0.081, 0.636) and (0.082, 0.635) .. (0.082, 0.633)
	-- (0.082, 0.633) .. controls (0.083, 0.632) and (0.083, 0.631) .. (0.084, 0.629)
	-- (0.084, 0.628) .. controls (0.084, 0.627) and (0.084, 0.627) .. (0.085, 0.627)
	-- (0.085, 0.625) .. controls (0.086, 0.624) and (0.086, 0.624) .. (0.086, 0.623)
	-- (0.086, 0.623) .. controls (0.086, 0.622) and (0.086, 0.622) .. (0.087, 0.622)
	-- (0.087, 0.62) .. controls (0.087, 0.62) and (0.087, 0.62) .. (0.088, 0.619)
	-- (0.088, 0.618) .. controls (0.089, 0.617) and (0.089, 0.617) .. (0.089, 0.617)
	-- (0.089, 0.616) .. controls (0.089, 0.616) and (0.09, 0.616) .. (0.09, 0.616)
	-- (0.09, 0.614) .. controls (0.09, 0.614) and (0.091, 0.614) .. (0.091, 0.614)
	-- (0.091, 0.612) .. controls (0.091, 0.612) and (0.091, 0.612) .. (0.092, 0.612)
	-- (0.092, 0.61) .. controls (0.093, 0.61) and (0.093, 0.609) .. (0.093, 0.609)
	-- (0.093, 0.608) .. controls (0.094, 0.607) and (0.094, 0.606) .. (0.095, 0.605)
	-- (0.095, 0.603) .. controls (0.096, 0.603) and (0.096, 0.602) .. (0.096, 0.601)
	-- (0.096, 0.601) .. controls (0.097, 0.601) and (0.097, 0.6) .. (0.097, 0.6)
	-- (0.097, 0.6) .. controls (0.098, 0.598) and (0.099, 0.596) .. (0.1, 0.594)
	-- (0.1, 0.594) .. controls (0.1, 0.593) and (0.101, 0.591) .. (0.102, 0.59)
	-- (0.102, 0.589) .. controls (0.102, 0.589) and (0.102, 0.588) .. (0.103, 0.588)
	-- (0.103, 0.587) .. controls (0.103, 0.587) and (0.103, 0.587) .. (0.104, 0.586)
	-- (0.104, 0.585) .. controls (0.104, 0.585) and (0.104, 0.585) .. (0.105, 0.585)
	-- (0.105, 0.584) .. controls (0.105, 0.584) and (0.106, 0.584) .. (0.106, 0.583)
	-- (0.106, 0.583) .. controls (0.106, 0.583) and (0.107, 0.582) .. (0.107, 0.582)
	-- (0.107, 0.582) .. controls (0.107, 0.582) and (0.108, 0.582) .. (0.108, 0.582)
	-- (0.108, 0.582) .. controls (0.108, 0.582) and (0.108, 0.582) .. (0.109, 0.582)
	-- (0.109, 0.582) .. controls (0.11, 0.582) and (0.11, 0.582) .. (0.11, 0.582)
	-- (0.11, 0.582) .. controls (0.11, 0.582) and (0.111, 0.582) .. (0.111, 0.582)
	-- (0.111, 0.582) .. controls (0.111, 0.582) and (0.111, 0.582) .. (0.112, 0.582)
	-- (0.112, 0.581) .. controls (0.112, 0.581) and (0.112, 0.581) .. (0.113, 0.581)
	-- (0.113, 0.581) .. controls (0.114, 0.581) and (0.114, 0.581) .. (0.114, 0.581)
	-- (0.114, 0.58) .. controls (0.114, 0.58) and (0.114, 0.58) .. (0.115, 0.58)
	-- (0.115, 0.58) .. controls (0.115, 0.58) and (0.116, 0.58) .. (0.116, 0.58)
	-- (0.116, 0.58) .. controls (0.116, 0.58) and (0.117, 0.58) .. (0.117, 0.579)
	-- (0.117, 0.579) .. controls (0.117, 0.579) and (0.117, 0.579) .. (0.118, 0.579)
	-- (0.118, 0.579) .. controls (0.118, 0.579) and (0.118, 0.579) .. (0.119, 0.579)
	-- (0.119, 0.579) .. controls (0.119, 0.579) and (0.119, 0.579) .. (0.12, 0.579)
	-- (0.12, 0.579) .. controls (0.121, 0.579) and (0.121, 0.579) .. (0.121, 0.579)
	-- (0.121, 0.579) .. controls (0.122, 0.579) and (0.122, 0.579) .. (0.122, 0.579)
	-- (0.122, 0.579) .. controls (0.122, 0.579) and (0.122, 0.579) .. (0.123, 0.579)
	-- (0.123, 0.58) .. controls (0.123, 0.58) and (0.124, 0.58) .. (0.124, 0.58)
	-- (0.124, 0.58) .. controls (0.125, 0.58) and (0.125, 0.58) .. (0.125, 0.58)
	-- (0.125, 0.58) .. controls (0.125, 0.58) and (0.125, 0.58) .. (0.126, 0.58)
	-- (0.126, 0.58) .. controls (0.126, 0.58) and (0.127, 0.58) .. (0.127, 0.58)
	-- (0.127, 0.58) .. controls (0.128, 0.58) and (0.128, 0.58) .. (0.128, 0.58)
	-- (0.128, 0.579) .. controls (0.128, 0.579) and (0.129, 0.579) .. (0.129, 0.579)
	-- (0.129, 0.58) .. controls (0.13, 0.58) and (0.13, 0.58) .. (0.13, 0.58)
	-- (0.13, 0.58) .. controls (0.13, 0.58) and (0.13, 0.58) .. (0.131, 0.58)
	-- (0.131, 0.58) .. controls (0.132, 0.58) and (0.132, 0.58) .. (0.132, 0.58)
	-- (0.132, 0.581) .. controls (0.132, 0.581) and (0.132, 0.581) .. (0.133, 0.581)
	-- (0.133, 0.581) .. controls (0.134, 0.581) and (0.134, 0.581) .. (0.134, 0.581)
	-- (0.134, 0.582) .. controls (0.134, 0.582) and (0.135, 0.582) .. (0.135, 0.582)
	-- (0.135, 0.583) .. controls (0.135, 0.583) and (0.135, 0.583) .. (0.136, 0.583)
	-- (0.136, 0.583) .. controls (0.136, 0.583) and (0.136, 0.583) .. (0.137, 0.583)
	-- (0.137, 0.584) .. controls (0.137, 0.584) and (0.138, 0.584) .. (0.138, 0.584)
	-- (0.138, 0.584) .. controls (0.139, 0.584) and (0.139, 0.584) .. (0.139, 0.584)
	-- (0.139, 0.585) .. controls (0.139, 0.585) and (0.14, 0.585) .. (0.14, 0.585)
	-- (0.14, 0.585) .. controls (0.14, 0.585) and (0.141, 0.585) .. (0.141, 0.585)
	-- (0.141, 0.585) .. controls (0.141, 0.585) and (0.142, 0.585) .. (0.142, 0.585)
	-- (0.142, 0.585) .. controls (0.142, 0.585) and (0.143, 0.585) .. (0.143, 0.585)
	-- (0.143, 0.586) .. controls (0.143, 0.586) and (0.143, 0.586) .. (0.144, 0.586)
	-- (0.144, 0.586) .. controls (0.144, 0.586) and (0.144, 0.586) .. (0.145, 0.586)
	-- (0.145, 0.586) .. controls (0.146, 0.586) and (0.146, 0.586) .. (0.146, 0.586)
	-- (0.146, 0.586) .. controls (0.147, 0.586) and (0.147, 0.586) .. (0.147, 0.586)
	-- (0.147, 0.587) .. controls (0.147, 0.587) and (0.148, 0.587) .. (0.148, 0.587)
	-- (0.148, 0.587) .. controls (0.149, 0.587) and (0.149, 0.587) .. (0.149, 0.587)
	-- (0.149, 0.587) .. controls (0.15, 0.587) and (0.15, 0.587) .. (0.15, 0.587)
	-- (0.15, 0.587) .. controls (0.151, 0.587) and (0.151, 0.587) .. (0.151, 0.588)
	-- (0.151, 0.588) .. controls (0.151, 0.588) and (0.152, 0.588) .. (0.152, 0.588)
	-- (0.152, 0.588) .. controls (0.152, 0.588) and (0.152, 0.588) .. (0.153, 0.588)
	-- (0.153, 0.588) .. controls (0.154, 0.588) and (0.154, 0.588) .. (0.154, 0.588)
	-- (0.154, 0.588) .. controls (0.154, 0.588) and (0.155, 0.588) .. (0.155, 0.588)
	-- (0.155, 0.588) .. controls (0.155, 0.588) and (0.155, 0.588) .. (0.156, 0.588)
	-- (0.156, 0.588) .. controls (0.156, 0.588) and (0.157, 0.588) .. (0.157, 0.588)
	-- (0.157, 0.588) .. controls (0.157, 0.588) and (0.158, 0.588) .. (0.158, 0.588)
	-- (0.158, 0.588) .. controls (0.159, 0.588) and (0.159, 0.588) .. (0.159, 0.588)
	-- (0.159, 0.588) .. controls (0.159, 0.588) and (0.159, 0.588) .. (0.16, 0.588)
	-- (0.16, 0.588) .. controls (0.16, 0.588) and (0.16, 0.588) .. (0.161, 0.588)
	-- (0.161, 0.588) .. controls (0.162, 0.588) and (0.162, 0.588) .. (0.162, 0.588)
	-- (0.162, 0.588) .. controls (0.162, 0.588) and (0.162, 0.588) .. (0.163, 0.588)
	-- (0.163, 0.587) .. controls (0.163, 0.587) and (0.164, 0.587) .. (0.164, 0.587)
	-- (0.164, 0.587) .. controls (0.164, 0.587) and (0.164, 0.587) .. (0.165, 0.587)
	-- (0.165, 0.587) .. controls (0.166, 0.587) and (0.166, 0.587) .. (0.166, 0.587)
	-- (0.166, 0.587) .. controls (0.166, 0.587) and (0.166, 0.587) .. (0.167, 0.587)
	-- (0.167, 0.587) .. controls (0.167, 0.587) and (0.168, 0.587) .. (0.168, 0.587)
	-- (0.168, 0.587) .. controls (0.168, 0.587) and (0.168, 0.587) .. (0.169, 0.587)
	-- (0.169, 0.586) .. controls (0.17, 0.586) and (0.17, 0.586) .. (0.17, 0.586)
	-- (0.17, 0.586) .. controls (0.17, 0.586) and (0.17, 0.586) .. (0.171, 0.586)
	-- (0.171, 0.586) .. controls (0.171, 0.586) and (0.172, 0.586) .. (0.172, 0.586)
	-- (0.172, 0.585) .. controls (0.173, 0.585) and (0.173, 0.585) .. (0.173, 0.585)
	-- (0.173, 0.585) .. controls (0.173, 0.585) and (0.174, 0.585) .. (0.174, 0.585)
	-- (0.174, 0.585) .. controls (0.174, 0.585) and (0.174, 0.585) .. (0.175, 0.585)
	-- (0.175, 0.584) .. controls (0.175, 0.584) and (0.175, 0.584) .. (0.176, 0.584)
	-- (0.176, 0.584) .. controls (0.177, 0.584) and (0.177, 0.584) .. (0.177, 0.584)
	-- (0.177, 0.584) .. controls (0.177, 0.584) and (0.178, 0.584) .. (0.178, 0.584)
	-- (0.178, 0.584) .. controls (0.179, 0.584) and (0.179, 0.584) .. (0.179, 0.584)
	-- (0.179, 0.584) .. controls (0.179, 0.584) and (0.179, 0.584) .. (0.18, 0.584)
	-- (0.18, 0.583) .. controls (0.181, 0.583) and (0.181, 0.583) .. (0.181, 0.583)
	-- (0.181, 0.583) .. controls (0.181, 0.583) and (0.182, 0.583) .. (0.182, 0.583)
	-- (0.182, 0.583) .. controls (0.182, 0.583) and (0.182, 0.583) .. (0.183, 0.583)
	-- (0.183, 0.583) .. controls (0.183, 0.583) and (0.184, 0.583) .. (0.184, 0.583)
	-- (0.184, 0.583) .. controls (0.184, 0.583) and (0.184, 0.583) .. (0.185, 0.583)
	-- (0.185, 0.583) .. controls (0.186, 0.583) and (0.186, 0.583) .. (0.186, 0.583)
	-- (0.186, 0.583) .. controls (0.186, 0.583) and (0.187, 0.583) .. (0.187, 0.583)
	-- (0.187, 0.583) .. controls (0.187, 0.583) and (0.188, 0.583) .. (0.188, 0.583)
	-- (0.188, 0.583) .. controls (0.188, 0.583) and (0.189, 0.583) .. (0.189, 0.583)
	-- (0.189, 0.584) .. controls (0.19, 0.584) and (0.19, 0.584) .. (0.19, 0.584)
	-- (0.19, 0.584) .. controls (0.191, 0.584) and (0.191, 0.584) .. (0.191, 0.584)
	-- (0.191, 0.584) .. controls (0.191, 0.584) and (0.191, 0.584) .. (0.192, 0.584)
	-- (0.192, 0.585) .. controls (0.192, 0.585) and (0.192, 0.585) .. (0.193, 0.585)
	-- (0.193, 0.585) .. controls (0.193, 0.585) and (0.193, 0.585) .. (0.194, 0.585)
	-- (0.194, 0.586) .. controls (0.194, 0.586) and (0.194, 0.586) .. (0.195, 0.586)
	-- (0.195, 0.586) .. controls (0.195, 0.586) and (0.195, 0.586) .. (0.196, 0.586)
	-- (0.196, 0.586) .. controls (0.196, 0.586) and (0.196, 0.586) .. (0.197, 0.586)
	-- (0.197, 0.587) .. controls (0.197, 0.587) and (0.197, 0.587) .. (0.198, 0.587)
	-- (0.198, 0.587) .. controls (0.199, 0.587) and (0.199, 0.587) .. (0.199, 0.587)
	-- (0.199, 0.588) .. controls (0.2, 0.588) and (0.2, 0.588) .. (0.2, 0.588)
	-- (0.2, 0.588) .. controls (0.2, 0.588) and (0.201, 0.588) .. (0.201, 0.588)
	-- (0.201, 0.588) .. controls (0.201, 0.588) and (0.202, 0.589) .. (0.202, 0.589)
	-- (0.202, 0.589) .. controls (0.202, 0.589) and (0.202, 0.589) .. (0.203, 0.589)
	-- (0.203, 0.589) .. controls (0.203, 0.589) and (0.204, 0.589) .. (0.204, 0.589)
	-- (0.204, 0.59) .. controls (0.204, 0.59) and (0.204, 0.59) .. (0.205, 0.59)
	-- (0.205, 0.59) .. controls (0.206, 0.59) and (0.206, 0.59) .. (0.206, 0.59)
	-- (0.206, 0.591) .. controls (0.206, 0.591) and (0.207, 0.591) .. (0.207, 0.591)
	-- (0.207, 0.591) .. controls (0.207, 0.591) and (0.207, 0.591) .. (0.208, 0.591)
	-- (0.208, 0.591) .. controls (0.208, 0.591) and (0.209, 0.592) .. (0.209, 0.592)
	-- (0.209, 0.592) .. controls (0.21, 0.592) and (0.21, 0.592) .. (0.21, 0.592)
	-- (0.21, 0.592) .. controls (0.21, 0.592) and (0.21, 0.592) .. (0.211, 0.592)
	-- (0.211, 0.593) .. controls (0.212, 0.593) and (0.212, 0.593) .. (0.212, 0.593)
	-- (0.212, 0.593) .. controls (0.213, 0.593) and (0.213, 0.593) .. (0.213, 0.593)
	-- (0.213, 0.594) .. controls (0.213, 0.594) and (0.214, 0.594) .. (0.214, 0.594)
	-- (0.214, 0.594) .. controls (0.214, 0.594) and (0.215, 0.594) .. (0.215, 0.594)
	-- (0.215, 0.595) .. controls (0.216, 0.595) and (0.216, 0.595) .. (0.216, 0.595)
	-- (0.216, 0.595) .. controls (0.216, 0.595) and (0.217, 0.595) .. (0.217, 0.595)
	-- (0.217, 0.595) .. controls (0.217, 0.595) and (0.218, 0.595) .. (0.218, 0.595)
	-- (0.218, 0.596) .. controls (0.218, 0.596) and (0.218, 0.596) .. (0.219, 0.596)
	-- (0.219, 0.596) .. controls (0.219, 0.596) and (0.22, 0.596) .. (0.22, 0.596)
	-- (0.22, 0.597) .. controls (0.22, 0.597) and (0.221, 0.597) .. (0.221, 0.597)
	-- (0.221, 0.597) .. controls (0.221, 0.597) and (0.222, 0.597) .. (0.222, 0.597)
	-- (0.222, 0.598) .. controls (0.222, 0.598) and (0.223, 0.598) .. (0.223, 0.598)
	-- (0.223, 0.598) .. controls (0.223, 0.598) and (0.224, 0.598) .. (0.224, 0.598)
	-- (0.224, 0.598) .. controls (0.224, 0.598) and (0.225, 0.598) .. (0.225, 0.598)
	-- (0.225, 0.599) .. controls (0.225, 0.599) and (0.226, 0.599) .. (0.226, 0.599)
	-- (0.226, 0.599) .. controls (0.226, 0.599) and (0.226, 0.599) .. (0.227, 0.599)
	-- (0.227, 0.599) .. controls (0.228, 0.6) and (0.228, 0.6) .. (0.228, 0.6)
	-- (0.228, 0.6) .. controls (0.228, 0.6) and (0.229, 0.6) .. (0.229, 0.6)
	-- (0.229, 0.6) .. controls (0.229, 0.6) and (0.229, 0.6) .. (0.23, 0.6)
	-- (0.23, 0.6) .. controls (0.231, 0.6) and (0.231, 0.6) .. (0.231, 0.6)
	-- (0.231, 0.601) .. controls (0.231, 0.601) and (0.232, 0.601) .. (0.232, 0.601)
	-- (0.232, 0.601) .. controls (0.232, 0.601) and (0.233, 0.601) .. (0.233, 0.601)
	-- (0.233, 0.601) .. controls (0.233, 0.601) and (0.233, 0.601) .. (0.234, 0.601)
	-- (0.234, 0.602) .. controls (0.234, 0.602) and (0.235, 0.602) .. (0.235, 0.602)
	-- (0.235, 0.602) .. controls (0.235, 0.602) and (0.236, 0.602) .. (0.236, 0.602)
	-- (0.236, 0.602) .. controls (0.236, 0.602) and (0.236, 0.602) .. (0.237, 0.602)
	-- (0.237, 0.603) .. controls (0.237, 0.603) and (0.238, 0.603) .. (0.238, 0.603)
	-- (0.238, 0.603) .. controls (0.239, 0.603) and (0.239, 0.603) .. (0.239, 0.603)
	-- (0.239, 0.603) .. controls (0.239, 0.603) and (0.239, 0.603) .. (0.24, 0.603)
	-- (0.24, 0.604) .. controls (0.24, 0.604) and (0.241, 0.604) .. (0.241, 0.604)
	-- (0.241, 0.604) .. controls (0.241, 0.604) and (0.242, 0.604) .. (0.242, 0.604)
	-- (0.242, 0.605) .. controls (0.243, 0.605) and (0.243, 0.605) .. (0.243, 0.605)
	-- (0.243, 0.605) .. controls (0.244, 0.605) and (0.244, 0.605) .. (0.244, 0.605)
	-- (0.244, 0.605) .. controls (0.244, 0.605) and (0.244, 0.605) .. (0.245, 0.605)
	-- (0.245, 0.606) .. controls (0.245, 0.606) and (0.245, 0.606) .. (0.246, 0.606)
	-- (0.246, 0.606) .. controls (0.247, 0.606) and (0.247, 0.606) .. (0.247, 0.606)
	-- (0.247, 0.607) .. controls (0.247, 0.607) and (0.247, 0.607) .. (0.248, 0.607)
	-- (0.248, 0.607) .. controls (0.249, 0.607) and (0.249, 0.607) .. (0.249, 0.607)
	-- (0.249, 0.608) .. controls (0.25, 0.608) and (0.25, 0.608) .. (0.25, 0.608)
	-- (0.25, 0.608) .. controls (0.25, 0.608) and (0.251, 0.608) .. (0.251, 0.608)
	-- (0.251, 0.609) .. controls (0.251, 0.609) and (0.251, 0.609) .. (0.252, 0.609)
	-- (0.252, 0.609) .. controls (0.252, 0.609) and (0.252, 0.609) .. (0.253, 0.609)
	-- (0.253, 0.61) .. controls (0.253, 0.61) and (0.254, 0.61) .. (0.254, 0.61)
	-- (0.254, 0.611) .. controls (0.255, 0.611) and (0.255, 0.611) .. (0.255, 0.611)
	-- (0.255, 0.611) .. controls (0.255, 0.611) and (0.256, 0.611) .. (0.256, 0.611)
	-- (0.256, 0.612) .. controls (0.256, 0.612) and (0.257, 0.612) .. (0.257, 0.612)
	-- (0.257, 0.613) .. controls (0.258, 0.613) and (0.258, 0.613) .. (0.258, 0.613)
	-- (0.258, 0.613) .. controls (0.259, 0.613) and (0.259, 0.613) .. (0.259, 0.613)
	-- (0.259, 0.614) .. controls (0.26, 0.614) and (0.26, 0.614) .. (0.26, 0.614)
	-- (0.26, 0.615) .. controls (0.261, 0.615) and (0.261, 0.615) .. (0.261, 0.615)
	-- (0.261, 0.616) .. controls (0.261, 0.616) and (0.262, 0.616) .. (0.262, 0.616)
	-- (0.262, 0.616) .. controls (0.263, 0.616) and (0.263, 0.616) .. (0.263, 0.616)
	-- (0.263, 0.617) .. controls (0.263, 0.617) and (0.263, 0.617) .. (0.264, 0.617)
	-- (0.264, 0.617) .. controls (0.264, 0.617) and (0.264, 0.617) .. (0.265, 0.617)
	-- (0.265, 0.618) .. controls (0.265, 0.618) and (0.265, 0.618) .. (0.266, 0.618)
	-- (0.266, 0.619) .. controls (0.267, 0.619) and (0.267, 0.619) .. (0.267, 0.619)
	-- (0.267, 0.619) .. controls (0.267, 0.619) and (0.267, 0.619) .. (0.268, 0.619)
	-- (0.268, 0.62) .. controls (0.268, 0.62) and (0.269, 0.62) .. (0.269, 0.62)
	-- (0.269, 0.62) .. controls (0.269, 0.621) and (0.269, 0.621) .. (0.27, 0.621)
	-- (0.27, 0.621) .. controls (0.271, 0.621) and (0.271, 0.621) .. (0.271, 0.621)
	-- (0.271, 0.622) .. controls (0.271, 0.622) and (0.272, 0.622) .. (0.272, 0.622)
	-- (0.272, 0.622) .. controls (0.272, 0.622) and (0.273, 0.622) .. (0.273, 0.622)
	-- (0.273, 0.623) .. controls (0.273, 0.623) and (0.273, 0.623) .. (0.274, 0.623)
	-- (0.274, 0.623) .. controls (0.274, 0.623) and (0.275, 0.623) .. (0.275, 0.623)
	-- (0.275, 0.624) .. controls (0.275, 0.624) and (0.276, 0.624) .. (0.276, 0.624)
	-- (0.276, 0.624) .. controls (0.276, 0.624) and (0.276, 0.624) .. (0.277, 0.624)
	-- (0.277, 0.625) .. controls (0.277, 0.625) and (0.278, 0.625) .. (0.278, 0.625)
	-- (0.278, 0.625) .. controls (0.278, 0.625) and (0.279, 0.625) .. (0.279, 0.625)
	-- (0.279, 0.626) .. controls (0.279, 0.626) and (0.279, 0.626) .. (0.28, 0.626)
	-- (0.28, 0.627) .. controls (0.28, 0.627) and (0.28, 0.627) .. (0.281, 0.627)
	-- (0.281, 0.627) .. controls (0.281, 0.627) and (0.281, 0.627) .. (0.282, 0.627)
	-- (0.282, 0.628) .. controls (0.283, 0.628) and (0.283, 0.628) .. (0.283, 0.628)
	-- (0.283, 0.628) .. controls (0.283, 0.628) and (0.284, 0.628) .. (0.284, 0.628)
	-- (0.284, 0.629) .. controls (0.285, 0.629) and (0.285, 0.629) .. (0.285, 0.629)
	-- (0.285, 0.63) .. controls (0.285, 0.63) and (0.285, 0.63) .. (0.286, 0.63)
	-- (0.286, 0.63) .. controls (0.287, 0.63) and (0.287, 0.63) .. (0.287, 0.63)
	-- (0.287, 0.631) .. controls (0.287, 0.631) and (0.287, 0.631) .. (0.288, 0.631)
	-- (0.288, 0.631) .. controls (0.289, 0.631) and (0.289, 0.631) .. (0.289, 0.631)
	-- (0.289, 0.632) .. controls (0.289, 0.632) and (0.289, 0.632) .. (0.29, 0.632)
	-- (0.29, 0.632) .. controls (0.29, 0.633) and (0.291, 0.633) .. (0.291, 0.633)
	-- (0.291, 0.633) .. controls (0.292, 0.633) and (0.292, 0.633) .. (0.292, 0.633)
	-- (0.292, 0.634) .. controls (0.292, 0.634) and (0.292, 0.634) .. (0.293, 0.634)
	-- (0.293, 0.634) .. controls (0.293, 0.634) and (0.293, 0.634) .. (0.294, 0.634)
	-- (0.294, 0.635) .. controls (0.294, 0.635) and (0.295, 0.635) .. (0.295, 0.635)
	-- (0.295, 0.635) .. controls (0.295, 0.635) and (0.295, 0.635) .. (0.296, 0.635)
	-- (0.296, 0.636) .. controls (0.296, 0.636) and (0.297, 0.636) .. (0.297, 0.636)
	-- (0.297, 0.637) .. controls (0.298, 0.637) and (0.298, 0.637) .. (0.298, 0.637)
	-- (0.298, 0.637) .. controls (0.299, 0.637) and (0.299, 0.637) .. (0.299, 0.637)
	-- (0.299, 0.638) .. controls (0.299, 0.638) and (0.3, 0.638) .. (0.3, 0.638)
	-- (0.3, 0.638) .. controls (0.3, 0.638) and (0.301, 0.638) .. (0.301, 0.638)
	-- (0.301, 0.639) .. controls (0.302, 0.639) and (0.302, 0.639) .. (0.302, 0.639)
	-- (0.302, 0.64) .. controls (0.303, 0.64) and (0.303, 0.64) .. (0.303, 0.64)
	-- (0.303, 0.64) .. controls (0.304, 0.64) and (0.304, 0.64) .. (0.304, 0.64)
	-- (0.304, 0.641) .. controls (0.304, 0.641) and (0.304, 0.641) .. (0.305, 0.641)
	-- (0.305, 0.642) .. controls (0.306, 0.642) and (0.306, 0.642) .. (0.306, 0.642)
	-- (0.306, 0.642) .. controls (0.307, 0.642) and (0.307, 0.642) .. (0.307, 0.642)
	-- (0.307, 0.643) .. controls (0.307, 0.643) and (0.308, 0.643) .. (0.308, 0.643)
	-- (0.308, 0.643) .. controls (0.308, 0.643) and (0.308, 0.643) .. (0.309, 0.644)
	-- (0.309, 0.644) .. controls (0.31, 0.644) and (0.31, 0.644) .. (0.31, 0.644)
	-- (0.31, 0.645) .. controls (0.31, 0.645) and (0.311, 0.645) .. (0.311, 0.645)
	-- (0.311, 0.646) .. controls (0.311, 0.646) and (0.311, 0.646) .. (0.312, 0.646)
	-- (0.312, 0.646) .. controls (0.313, 0.646) and (0.313, 0.646) .. (0.313, 0.646)
	-- (0.313, 0.647) .. controls (0.314, 0.647) and (0.314, 0.647) .. (0.314, 0.647)
	-- (0.314, 0.648) .. controls (0.315, 0.648) and (0.315, 0.648) .. (0.315, 0.648)
	-- (0.315, 0.648) .. controls (0.315, 0.648) and (0.315, 0.648) .. (0.316, 0.648)
	-- (0.316, 0.649) .. controls (0.317, 0.649) and (0.317, 0.649) .. (0.317, 0.649)
	-- (0.317, 0.65) .. controls (0.317, 0.65) and (0.318, 0.65) .. (0.318, 0.65)
	-- (0.318, 0.65) .. controls (0.319, 0.65) and (0.319, 0.65) .. (0.319, 0.65)
	-- (0.319, 0.651) .. controls (0.32, 0.651) and (0.32, 0.651) .. (0.32, 0.651)
	-- (0.32, 0.651) .. controls (0.32, 0.651) and (0.321, 0.651) .. (0.321, 0.651)
	-- (0.321, 0.652) .. controls (0.321, 0.652) and (0.322, 0.652) .. (0.322, 0.652)
	-- (0.322, 0.652) .. controls (0.322, 0.652) and (0.323, 0.652) .. (0.323, 0.652)
	-- (0.323, 0.653) .. controls (0.324, 0.653) and (0.324, 0.653) .. (0.324, 0.653)
	-- (0.324, 0.653) .. controls (0.324, 0.653) and (0.324, 0.653) .. (0.325, 0.653)
	-- (0.325, 0.654) .. controls (0.325, 0.654) and (0.326, 0.654) .. (0.326, 0.654)
	-- (0.326, 0.654) .. controls (0.327, 0.654) and (0.327, 0.655) .. (0.327, 0.655)
	-- (0.327, 0.655) .. controls (0.327, 0.655) and (0.328, 0.655) .. (0.328, 0.655)
	-- (0.328, 0.656) .. controls (0.328, 0.656) and (0.328, 0.656) .. (0.329, 0.656)
	-- (0.329, 0.656) .. controls (0.329, 0.656) and (0.33, 0.656) .. (0.33, 0.656)
	-- (0.33, 0.657) .. controls (0.33, 0.657) and (0.33, 0.657) .. (0.331, 0.657)
	-- (0.331, 0.657) .. controls (0.332, 0.657) and (0.332, 0.657) .. (0.332, 0.657)
	-- (0.332, 0.658) .. controls (0.332, 0.658) and (0.333, 0.658) .. (0.333, 0.658)
	-- (0.333, 0.658) .. controls (0.333, 0.658) and (0.333, 0.658) .. (0.334, 0.658)
	-- (0.334, 0.659) .. controls (0.335, 0.659) and (0.335, 0.659) .. (0.335, 0.659)
	-- (0.335, 0.659) .. controls (0.336, 0.659) and (0.336, 0.659) .. (0.336, 0.659)
	-- (0.336, 0.66) .. controls (0.337, 0.66) and (0.337, 0.66) .. (0.337, 0.66)
	-- (0.337, 0.66) .. controls (0.338, 0.66) and (0.338, 0.66) .. (0.338, 0.66)
	-- (0.338, 0.661) .. controls (0.338, 0.661) and (0.338, 0.661) .. (0.339, 0.661)
	-- (0.339, 0.661) .. controls (0.339, 0.661) and (0.34, 0.662) .. (0.34, 0.662)
	-- (0.34, 0.662) .. controls (0.34, 0.662) and (0.341, 0.662) .. (0.341, 0.662)
	-- (0.341, 0.663) .. controls (0.341, 0.663) and (0.341, 0.663) .. (0.342, 0.663)
	-- (0.342, 0.663) .. controls (0.342, 0.663) and (0.342, 0.663) .. (0.343, 0.663)
	-- (0.343, 0.664) .. controls (0.343, 0.664) and (0.343, 0.664) .. (0.344, 0.664)
	-- (0.344, 0.664) .. controls (0.345, 0.664) and (0.345, 0.664) .. (0.345, 0.664)
	-- (0.345, 0.665) .. controls (0.346, 0.665) and (0.346, 0.665) .. (0.346, 0.665)
	-- (0.346, 0.665) .. controls (0.347, 0.665) and (0.347, 0.665) .. (0.347, 0.665)
	-- (0.347, 0.666) .. controls (0.348, 0.666) and (0.348, 0.666) .. (0.348, 0.666)
	-- (0.348, 0.667) .. controls (0.348, 0.667) and (0.349, 0.667) .. (0.349, 0.667)
	-- (0.349, 0.667) .. controls (0.349, 0.667) and (0.349, 0.667) .. (0.35, 0.667)
	-- (0.35, 0.668) .. controls (0.35, 0.668) and (0.351, 0.668) .. (0.351, 0.668)
	-- (0.351, 0.668) .. controls (0.351, 0.668) and (0.352, 0.668) .. (0.352, 0.668)
	-- (0.352, 0.669) .. controls (0.352, 0.669) and (0.353, 0.669) .. (0.353, 0.669)
	-- (0.353, 0.67) .. controls (0.353, 0.67) and (0.354, 0.67) .. (0.354, 0.67)
	-- (0.354, 0.67) .. controls (0.355, 0.67) and (0.355, 0.67) .. (0.355, 0.67)
	-- (0.355, 0.671) .. controls (0.355, 0.671) and (0.356, 0.671) .. (0.356, 0.671)
	-- (0.356, 0.672) .. controls (0.356, 0.672) and (0.356, 0.672) .. (0.357, 0.672)
	-- (0.357, 0.672) .. controls (0.358, 0.672) and (0.358, 0.672) .. (0.358, 0.672)
	-- (0.358, 0.673) .. controls (0.358, 0.673) and (0.358, 0.673) .. (0.359, 0.673)
	-- (0.359, 0.674) .. controls (0.359, 0.674) and (0.359, 0.674) .. (0.36, 0.674)
	-- (0.36, 0.674) .. controls (0.361, 0.674) and (0.361, 0.674) .. (0.361, 0.674)
	-- (0.361, 0.675) .. controls (0.362, 0.675) and (0.362, 0.675) .. (0.362, 0.675)
	-- (0.362, 0.676) .. controls (0.363, 0.676) and (0.363, 0.676) .. (0.363, 0.676)
	-- (0.363, 0.676) .. controls (0.364, 0.676) and (0.364, 0.676) .. (0.364, 0.676)
	-- (0.364, 0.677) .. controls (0.364, 0.677) and (0.364, 0.677) .. (0.365, 0.677)
	-- (0.365, 0.678) .. controls (0.365, 0.678) and (0.365, 0.678) .. (0.366, 0.678)
	-- (0.366, 0.678) .. controls (0.366, 0.678) and (0.366, 0.679) .. (0.367, 0.679)
	-- (0.367, 0.679) .. controls (0.367, 0.679) and (0.368, 0.679) .. (0.368, 0.679)
	-- (0.368, 0.68) .. controls (0.368, 0.68) and (0.368, 0.68) .. (0.369, 0.68)
	-- (0.369, 0.681) .. controls (0.369, 0.681) and (0.369, 0.681) .. (0.37, 0.681)
	-- (0.37, 0.681) .. controls (0.37, 0.682) and (0.37, 0.682) .. (0.371, 0.682)
	-- (0.371, 0.682) .. controls (0.371, 0.682) and (0.371, 0.682) .. (0.372, 0.682)
	-- (0.372, 0.683) .. controls (0.373, 0.683) and (0.373, 0.683) .. (0.373, 0.683)
	-- (0.373, 0.684) .. controls (0.373, 0.684) and (0.373, 0.684) .. (0.374, 0.684)
	-- (0.374, 0.685) .. controls (0.374, 0.685) and (0.375, 0.685) .. (0.375, 0.685)
	-- (0.375, 0.686) .. controls (0.376, 0.686) and (0.376, 0.686) .. (0.376, 0.686)
	-- (0.376, 0.686) .. controls (0.376, 0.686) and (0.377, 0.686) .. (0.377, 0.686)
	-- (0.377, 0.687) .. controls (0.377, 0.687) and (0.377, 0.687) .. (0.378, 0.687)
	-- (0.378, 0.688) .. controls (0.378, 0.688) and (0.378, 0.688) .. (0.379, 0.688)
	-- (0.379, 0.689) .. controls (0.38, 0.689) and (0.38, 0.689) .. (0.38, 0.689)
	-- (0.38, 0.69) .. controls (0.38, 0.69) and (0.38, 0.69) .. (0.381, 0.69)
	-- (0.381, 0.691) .. controls (0.382, 0.691) and (0.382, 0.691) .. (0.382, 0.691)
	-- (0.382, 0.692) .. controls (0.383, 0.692) and (0.383, 0.692) .. (0.383, 0.692)
	-- (0.383, 0.693) .. controls (0.383, 0.693) and (0.383, 0.693) .. (0.384, 0.693)
	-- (0.384, 0.693) .. controls (0.384, 0.693) and (0.385, 0.693) .. (0.385, 0.693)
	-- (0.385, 0.694) .. controls (0.385, 0.694) and (0.386, 0.694) .. (0.386, 0.694)
	-- (0.386, 0.695) .. controls (0.387, 0.695) and (0.387, 0.695) .. (0.387, 0.695)
	-- (0.387, 0.696) .. controls (0.387, 0.696) and (0.387, 0.696) .. (0.388, 0.696)
	-- (0.388, 0.697) .. controls (0.389, 0.697) and (0.389, 0.697) .. (0.389, 0.697)
	-- (0.389, 0.698) .. controls (0.39, 0.698) and (0.39, 0.698) .. (0.39, 0.698)
	-- (0.39, 0.699) .. controls (0.391, 0.699) and (0.391, 0.699) .. (0.391, 0.699)
	-- (0.391, 0.699) .. controls (0.391, 0.699) and (0.392, 0.699) .. (0.392, 0.699)
	-- (0.392, 0.7) .. controls (0.392, 0.7) and (0.392, 0.7) .. (0.393, 0.7)
	-- (0.393, 0.701) .. controls (0.393, 0.701) and (0.394, 0.701) .. (0.394, 0.701)
	-- (0.394, 0.702) .. controls (0.395, 0.702) and (0.395, 0.702) .. (0.395, 0.702)
	-- (0.395, 0.703) .. controls (0.395, 0.703) and (0.396, 0.703) .. (0.396, 0.703)
	-- (0.396, 0.704) .. controls (0.396, 0.704) and (0.396, 0.704) .. (0.397, 0.704)
	-- (0.397, 0.704) .. controls (0.397, 0.704) and (0.398, 0.704) .. (0.398, 0.704)
	-- (0.398, 0.705) .. controls (0.398, 0.705) and (0.399, 0.705) .. (0.399, 0.705)
	-- (0.399, 0.706) .. controls (0.399, 0.706) and (0.399, 0.706) .. (0.4, 0.706)
	-- (0.4, 0.707) .. controls (0.4, 0.707) and (0.4, 0.707) .. (0.401, 0.707)
	-- (0.401, 0.708) .. controls (0.401, 0.708) and (0.401, 0.708) .. (0.402, 0.708)
	-- (0.402, 0.708) .. controls (0.402, 0.708) and (0.403, 0.708) .. (0.403, 0.709)
	-- (0.403, 0.709) .. controls (0.403, 0.709) and (0.404, 0.709) .. (0.404, 0.709)
	-- (0.404, 0.71) .. controls (0.405, 0.71) and (0.405, 0.71) .. (0.405, 0.71)
	-- (0.405, 0.711) .. controls (0.405, 0.711) and (0.406, 0.711) .. (0.406, 0.711)
	-- (0.406, 0.712) .. controls (0.407, 0.712) and (0.407, 0.712) .. (0.407, 0.712)
	-- (0.407, 0.712) .. controls (0.408, 0.713) and (0.408, 0.713) .. (0.408, 0.713)
	-- (0.408, 0.713) .. controls (0.408, 0.713) and (0.408, 0.713) .. (0.409, 0.713)
	-- (0.409, 0.714) .. controls (0.41, 0.714) and (0.41, 0.714) .. (0.41, 0.714)
	-- (0.41, 0.715) .. controls (0.41, 0.715) and (0.411, 0.715) .. (0.411, 0.715)
	-- (0.411, 0.716) .. controls (0.411, 0.716) and (0.411, 0.716) .. (0.412, 0.716)
	-- (0.412, 0.717) .. controls (0.412, 0.717) and (0.413, 0.717) .. (0.413, 0.717)
	-- (0.413, 0.717) .. controls (0.413, 0.717) and (0.413, 0.717) .. (0.414, 0.717)
	-- (0.414, 0.718) .. controls (0.414, 0.718) and (0.414, 0.718) .. (0.415, 0.718)
	-- (0.415, 0.719) .. controls (0.416, 0.719) and (0.416, 0.719) .. (0.416, 0.719)
	-- (0.416, 0.72) .. controls (0.416, 0.72) and (0.416, 0.72) .. (0.417, 0.72)
	-- (0.417, 0.721) .. controls (0.417, 0.721) and (0.418, 0.721) .. (0.418, 0.721)
	-- (0.418, 0.721) .. controls (0.418, 0.721) and (0.419, 0.721) .. (0.419, 0.721)
	-- (0.419, 0.722) .. controls (0.419, 0.722) and (0.419, 0.722) .. (0.42, 0.722)
	-- (0.42, 0.723) .. controls (0.421, 0.723) and (0.421, 0.723) .. (0.421, 0.723)
	-- (0.421, 0.724) .. controls (0.421, 0.724) and (0.421, 0.724) .. (0.422, 0.724)
	-- (0.422, 0.725) .. controls (0.422, 0.725) and (0.422, 0.725) .. (0.423, 0.725)
	-- (0.423, 0.725) .. controls (0.423, 0.725) and (0.424, 0.725) .. (0.424, 0.725)
	-- (0.424, 0.726) .. controls (0.424, 0.726) and (0.424, 0.726) .. (0.425, 0.726)
	-- (0.425, 0.727) .. controls (0.426, 0.727) and (0.426, 0.727) .. (0.426, 0.727)
	-- (0.426, 0.728) .. controls (0.426, 0.728) and (0.426, 0.728) .. (0.427, 0.728)
	-- (0.427, 0.729) .. controls (0.427, 0.729) and (0.427, 0.729) .. (0.428, 0.729)
	-- (0.428, 0.729) .. controls (0.429, 0.729) and (0.429, 0.729) .. (0.429, 0.729)
	-- (0.429, 0.73) .. controls (0.429, 0.73) and (0.429, 0.73) .. (0.43, 0.73)
	-- (0.43, 0.731) .. controls (0.431, 0.731) and (0.431, 0.731) .. (0.431, 0.731)
	-- (0.431, 0.732) .. controls (0.431, 0.732) and (0.432, 0.732) .. (0.432, 0.732)
	-- (0.432, 0.733) .. controls (0.432, 0.733) and (0.432, 0.733) .. (0.433, 0.733)
	-- (0.433, 0.733) .. controls (0.434, 0.733) and (0.434, 0.733) .. (0.434, 0.733)
	-- (0.434, 0.734) .. controls (0.434, 0.734) and (0.434, 0.734) .. (0.435, 0.734)
	-- (0.435, 0.735) .. controls (0.435, 0.735) and (0.435, 0.735) .. (0.436, 0.735)
	-- (0.436, 0.736) .. controls (0.436, 0.736) and (0.437, 0.736) .. (0.437, 0.736)
	-- (0.437, 0.736) .. controls (0.437, 0.737) and (0.438, 0.737) .. (0.438, 0.737)
	-- (0.438, 0.737) .. controls (0.438, 0.737) and (0.438, 0.737) .. (0.439, 0.737)
	-- (0.439, 0.738) .. controls (0.44, 0.738) and (0.44, 0.738) .. (0.44, 0.738)
	-- (0.44, 0.739) .. controls (0.44, 0.739) and (0.44, 0.739) .. (0.441, 0.739)
	-- (0.441, 0.74) .. controls (0.441, 0.74) and (0.441, 0.74) .. (0.442, 0.74)
	-- (0.442, 0.74) .. controls (0.442, 0.74) and (0.442, 0.74) .. (0.443, 0.74)
	-- (0.443, 0.741) .. controls (0.443, 0.741) and (0.444, 0.741) .. (0.444, 0.741)
	-- (0.444, 0.742) .. controls (0.444, 0.742) and (0.444, 0.742) .. (0.445, 0.742)
	-- (0.445, 0.743) .. controls (0.445, 0.743) and (0.446, 0.743) .. (0.446, 0.743)
	-- (0.446, 0.743) .. controls (0.446, 0.743) and (0.446, 0.743) .. (0.447, 0.743)
	-- (0.447, 0.744) .. controls (0.448, 0.744) and (0.448, 0.744) .. (0.448, 0.744)
	-- (0.448, 0.745) .. controls (0.448, 0.745) and (0.448, 0.745) .. (0.449, 0.745)
	-- (0.449, 0.745) .. controls (0.45, 0.745) and (0.45, 0.745) .. (0.45, 0.746)
	-- (0.45, 0.746) .. controls (0.451, 0.746) and (0.451, 0.746) .. (0.451, 0.746)
	-- (0.451, 0.747) .. controls (0.451, 0.747) and (0.451, 0.747) .. (0.452, 0.747)
	-- (0.452, 0.747) .. controls (0.452, 0.747) and (0.452, 0.748) .. (0.453, 0.748)
	-- (0.453, 0.748) .. controls (0.453, 0.748) and (0.453, 0.748) .. (0.454, 0.748)
	-- (0.454, 0.749) .. controls (0.454, 0.749) and (0.455, 0.749) .. (0.455, 0.749)
	-- (0.455, 0.75) .. controls (0.455, 0.75) and (0.455, 0.75) .. (0.456, 0.75)
	-- (0.456, 0.75) .. controls (0.456, 0.75) and (0.456, 0.75) .. (0.457, 0.75)
	-- (0.457, 0.751) .. controls (0.458, 0.751) and (0.458, 0.751) .. (0.458, 0.751)
	-- (0.458, 0.752) .. controls (0.458, 0.752) and (0.458, 0.752) .. (0.459, 0.752)
	-- (0.459, 0.752) .. controls (0.46, 0.752) and (0.46, 0.752) .. (0.46, 0.752)
	-- (0.46, 0.753) .. controls (0.461, 0.753) and (0.461, 0.753) .. (0.461, 0.753)
	-- (0.461, 0.754) .. controls (0.462, 0.754) and (0.462, 0.754) .. (0.462, 0.754)
	-- (0.462, 0.754) .. controls (0.463, 0.754) and (0.463, 0.754) .. (0.463, 0.754)
	-- (0.463, 0.755) .. controls (0.463, 0.755) and (0.463, 0.755) .. (0.464, 0.755)
	-- (0.464, 0.756) .. controls (0.465, 0.756) and (0.465, 0.756) .. (0.465, 0.756)
	-- (0.465, 0.756) .. controls (0.465, 0.756) and (0.466, 0.756) .. (0.466, 0.756)
	-- (0.466, 0.757) .. controls (0.467, 0.757) and (0.467, 0.757) .. (0.467, 0.757)
	-- (0.467, 0.758) .. controls (0.468, 0.758) and (0.468, 0.758) .. (0.468, 0.758)
	-- (0.468, 0.758) .. controls (0.469, 0.758) and (0.469, 0.758) .. (0.469, 0.758)
	-- (0.469, 0.759) .. controls (0.47, 0.759) and (0.47, 0.759) .. (0.47, 0.759)
	-- (0.47, 0.76) .. controls (0.47, 0.76) and (0.47, 0.76) .. (0.471, 0.76)
	-- (0.471, 0.76) .. controls (0.472, 0.76) and (0.472, 0.76) .. (0.472, 0.76)
	-- (0.472, 0.761) .. controls (0.472, 0.761) and (0.472, 0.761) .. (0.473, 0.761)
	-- (0.473, 0.762) .. controls (0.474, 0.762) and (0.474, 0.762) .. (0.474, 0.762)
	-- (0.474, 0.762) .. controls (0.474, 0.762) and (0.475, 0.762) .. (0.475, 0.762)
	-- (0.475, 0.763) .. controls (0.475, 0.763) and (0.476, 0.763) .. (0.476, 0.763)
	-- (0.476, 0.763) .. controls (0.476, 0.763) and (0.476, 0.763) .. (0.477, 0.763)
	-- (0.477, 0.764) .. controls (0.478, 0.764) and (0.478, 0.764) .. (0.478, 0.764)
	-- (0.478, 0.765) .. controls (0.478, 0.765) and (0.478, 0.765) .. (0.479, 0.765)
	-- (0.479, 0.765) .. controls (0.48, 0.765) and (0.48, 0.765) .. (0.48, 0.765)
	-- (0.48, 0.766) .. controls (0.481, 0.766) and (0.481, 0.766) .. (0.481, 0.766)
	-- (0.481, 0.766) .. controls (0.482, 0.766) and (0.482, 0.767) .. (0.482, 0.767)
	-- (0.482, 0.767) .. controls (0.483, 0.767) and (0.483, 0.767) .. (0.483, 0.767)
	-- (0.483, 0.768) .. controls (0.483, 0.768) and (0.484, 0.768) .. (0.484, 0.768)
	-- (0.484, 0.768) .. controls (0.484, 0.768) and (0.485, 0.768) .. (0.485, 0.768)
	-- (0.485, 0.769) .. controls (0.486, 0.769) and (0.486, 0.769) .. (0.486, 0.769)
	-- (0.486, 0.769) .. controls (0.487, 0.769) and (0.487, 0.769) .. (0.487, 0.77)
	-- (0.487, 0.77) .. controls (0.487, 0.77) and (0.487, 0.77) .. (0.488, 0.77)
	-- (0.488, 0.771) .. controls (0.489, 0.771) and (0.489, 0.771) .. (0.489, 0.771)
	-- (0.489, 0.771) .. controls (0.49, 0.771) and (0.49, 0.771) .. (0.49, 0.771)
	-- (0.49, 0.772) .. controls (0.49, 0.772) and (0.49, 0.772) .. (0.491, 0.772)
	-- (0.491, 0.772) .. controls (0.492, 0.772) and (0.492, 0.772) .. (0.492, 0.772)
	-- (0.492, 0.773) .. controls (0.492, 0.773) and (0.492, 0.773) .. (0.493, 0.773)
	-- (0.493, 0.773) .. controls (0.494, 0.773) and (0.494, 0.773) .. (0.494, 0.773)
	-- (0.494, 0.774) .. controls (0.494, 0.774) and (0.494, 0.774) .. (0.495, 0.774)
	-- (0.495, 0.775) .. controls (0.496, 0.775) and (0.496, 0.775) .. (0.496, 0.775)
	-- (0.496, 0.775) .. controls (0.496, 0.775) and (0.497, 0.775) .. (0.497, 0.775)
	-- (0.497, 0.776) .. controls (0.497, 0.776) and (0.498, 0.776) .. (0.498, 0.776)
	-- (0.498, 0.776) .. controls (0.498, 0.776) and (0.498, 0.776) .. (0.499, 0.776)
	-- (0.499, 0.777) .. controls (0.499, 0.777) and (0.499, 0.777) .. (0.5, 0.777)
	-- (0.5, 0.777) .. controls (0.5, 0.777) and (0.501, 0.777) .. (0.501, 0.777)
	-- (0.501, 0.778) .. controls (0.501, 0.778) and (0.502, 0.778) .. (0.502, 0.778)
	-- (0.502, 0.778) .. controls (0.502, 0.778) and (0.503, 0.778) .. (0.503, 0.778)
	-- (0.503, 0.779) .. controls (0.503, 0.779) and (0.504, 0.779) .. (0.504, 0.779)
	-- (0.504, 0.78) .. controls (0.504, 0.78) and (0.504, 0.78) .. (0.505, 0.78)
	-- (0.505, 0.78) .. controls (0.505, 0.78) and (0.505, 0.78) .. (0.506, 0.78)
	-- (0.506, 0.781) .. controls (0.507, 0.781) and (0.507, 0.781) .. (0.507, 0.781)
	-- (0.507, 0.781) .. controls (0.507, 0.781) and (0.507, 0.781) .. (0.508, 0.781)
	-- (0.508, 0.782) .. controls (0.508, 0.782) and (0.509, 0.782) .. (0.509, 0.782)
	-- (0.509, 0.782) .. controls (0.51, 0.782) and (0.51, 0.782) .. (0.51, 0.782)
	-- (0.51, 0.783) .. controls (0.511, 0.783) and (0.511, 0.783) .. (0.511, 0.783)
	-- (0.511, 0.784) .. controls (0.512, 0.784) and (0.512, 0.784) .. (0.512, 0.784)
	-- (0.512, 0.784) .. controls (0.513, 0.784) and (0.513, 0.784) .. (0.513, 0.784)
	-- (0.513, 0.785) .. controls (0.514, 0.785) and (0.514, 0.785) .. (0.514, 0.785)
	-- (0.514, 0.785) .. controls (0.514, 0.785) and (0.515, 0.785) .. (0.515, 0.785)
	-- (0.515, 0.786) .. controls (0.516, 0.786) and (0.516, 0.786) .. (0.516, 0.786)
	-- (0.516, 0.787) .. controls (0.517, 0.787) and (0.517, 0.787) .. (0.517, 0.787)
	-- (0.517, 0.787) .. controls (0.517, 0.787) and (0.518, 0.787) .. (0.518, 0.787)
	-- (0.518, 0.788) .. controls (0.519, 0.788) and (0.519, 0.788) .. (0.519, 0.788)
	-- (0.519, 0.788) .. controls (0.519, 0.788) and (0.519, 0.788) .. (0.52, 0.788)
	-- (0.52, 0.789) .. controls (0.52, 0.789) and (0.521, 0.789) .. (0.521, 0.789)
	-- (0.521, 0.79) .. controls (0.522, 0.79) and (0.522, 0.79) .. (0.522, 0.79)
	-- (0.522, 0.79) .. controls (0.523, 0.79) and (0.523, 0.79) .. (0.523, 0.79)
	-- (0.523, 0.791) .. controls (0.523, 0.791) and (0.523, 0.791) .. (0.524, 0.791)
	-- (0.524, 0.791) .. controls (0.525, 0.791) and (0.525, 0.791) .. (0.525, 0.791)
	-- (0.525, 0.792) .. controls (0.526, 0.792) and (0.526, 0.792) .. (0.526, 0.792)
	-- (0.526, 0.792) .. controls (0.526, 0.792) and (0.526, 0.792) .. (0.527, 0.792)
	-- (0.527, 0.793) .. controls (0.527, 0.793) and (0.527, 0.793) .. (0.528, 0.793)
	-- (0.528, 0.794) .. controls (0.528, 0.794) and (0.529, 0.794) .. (0.529, 0.794)
	-- (0.529, 0.794) .. controls (0.53, 0.794) and (0.53, 0.794) .. (0.53, 0.794)
	-- (0.53, 0.795) .. controls (0.53, 0.795) and (0.53, 0.795) .. (0.531, 0.795)
	-- (0.531, 0.795) .. controls (0.531, 0.795) and (0.532, 0.795) .. (0.532, 0.795)
	-- (0.532, 0.796) .. controls (0.533, 0.796) and (0.533, 0.796) .. (0.533, 0.796)
	-- (0.533, 0.796) .. controls (0.533, 0.796) and (0.533, 0.796) .. (0.534, 0.796)
	-- (0.534, 0.797) .. controls (0.534, 0.797) and (0.534, 0.797) .. (0.535, 0.797)
	-- (0.535, 0.797) .. controls (0.535, 0.797) and (0.535, 0.798) .. (0.536, 0.798)
	-- (0.536, 0.798) .. controls (0.536, 0.798) and (0.536, 0.798) .. (0.537, 0.798)
	-- (0.537, 0.799) .. controls (0.537, 0.799) and (0.538, 0.799) .. (0.538, 0.799)
	-- (0.538, 0.799) .. controls (0.539, 0.799) and (0.539, 0.799) .. (0.539, 0.799)
	-- (0.539, 0.8) .. controls (0.539, 0.8) and (0.54, 0.8) .. (0.54, 0.8)
	-- (0.54, 0.8) .. controls (0.54, 0.8) and (0.541, 0.8) .. (0.541, 0.8)
	-- (0.541, 0.801) .. controls (0.541, 0.801) and (0.542, 0.801) .. (0.542, 0.801)
	-- (0.542, 0.801) .. controls (0.543, 0.801) and (0.543, 0.801) .. (0.543, 0.801)
	-- (0.543, 0.802) .. controls (0.543, 0.802) and (0.543, 0.802) .. (0.544, 0.802)
	-- (0.544, 0.802) .. controls (0.544, 0.802) and (0.545, 0.802) .. (0.545, 0.803)
	-- (0.545, 0.803) .. controls (0.545, 0.803) and (0.546, 0.803) .. (0.546, 0.803)
	-- (0.546, 0.804) .. controls (0.546, 0.804) and (0.547, 0.804) .. (0.547, 0.804)
	-- (0.547, 0.804) .. controls (0.547, 0.804) and (0.547, 0.804) .. (0.548, 0.804)
	-- (0.548, 0.805) .. controls (0.548, 0.805) and (0.548, 0.805) .. (0.549, 0.805)
	-- (0.549, 0.805) .. controls (0.55, 0.805) and (0.55, 0.805) .. (0.55, 0.805)
	-- (0.55, 0.806) .. controls (0.55, 0.806) and (0.551, 0.806) .. (0.551, 0.806)
	-- (0.551, 0.806) .. controls (0.551, 0.806) and (0.551, 0.806) .. (0.552, 0.806)
	-- (0.552, 0.807) .. controls (0.552, 0.807) and (0.552, 0.807) .. (0.553, 0.807)
	-- (0.553, 0.807) .. controls (0.553, 0.808) and (0.554, 0.808) .. (0.554, 0.808)
	-- (0.554, 0.808) .. controls (0.554, 0.808) and (0.554, 0.808) .. (0.555, 0.808)
	-- (0.555, 0.809) .. controls (0.555, 0.809) and (0.555, 0.809) .. (0.556, 0.809)
	-- (0.556, 0.809) .. controls (0.556, 0.809) and (0.557, 0.809) .. (0.557, 0.809)
	-- (0.557, 0.81) .. controls (0.557, 0.81) and (0.557, 0.81) .. (0.558, 0.81)
	-- (0.558, 0.81) .. controls (0.558, 0.81) and (0.559, 0.81) .. (0.559, 0.81)
	-- (0.559, 0.811) .. controls (0.56, 0.811) and (0.56, 0.811) .. (0.56, 0.811)
	-- (0.56, 0.811) .. controls (0.56, 0.811) and (0.561, 0.811) .. (0.561, 0.811)
	-- (0.561, 0.812) .. controls (0.561, 0.812) and (0.561, 0.812) .. (0.562, 0.812)
	-- (0.562, 0.813) .. controls (0.562, 0.813) and (0.563, 0.813) .. (0.563, 0.813)
	-- (0.563, 0.813) .. controls (0.563, 0.813) and (0.563, 0.813) .. (0.564, 0.813)
	-- (0.564, 0.814) .. controls (0.565, 0.814) and (0.565, 0.814) .. (0.565, 0.814)
	-- (0.565, 0.814) .. controls (0.565, 0.814) and (0.566, 0.814) .. (0.566, 0.814)
	-- (0.566, 0.815) .. controls (0.567, 0.815) and (0.567, 0.815) .. (0.567, 0.815)
	-- (0.567, 0.815) .. controls (0.567, 0.815) and (0.567, 0.815) .. (0.568, 0.815)
	-- (0.568, 0.816) .. controls (0.569, 0.816) and (0.569, 0.816) .. (0.569, 0.816)
	-- (0.569, 0.817) .. controls (0.57, 0.817) and (0.57, 0.817) .. (0.57, 0.817)
	-- (0.57, 0.817) .. controls (0.57, 0.817) and (0.57, 0.817) .. (0.571, 0.817)
	-- (0.571, 0.818) .. controls (0.572, 0.818) and (0.572, 0.818) .. (0.572, 0.818)
	-- (0.572, 0.818) .. controls (0.572, 0.818) and (0.572, 0.818) .. (0.573, 0.818)
	-- (0.573, 0.819) .. controls (0.573, 0.819) and (0.574, 0.819) .. (0.574, 0.819)
	-- (0.574, 0.819) .. controls (0.574, 0.819) and (0.574, 0.82) .. (0.575, 0.82)
	-- (0.575, 0.82) .. controls (0.576, 0.82) and (0.576, 0.82) .. (0.576, 0.82)
	-- (0.576, 0.821) .. controls (0.577, 0.821) and (0.577, 0.821) .. (0.577, 0.821)
	-- (0.577, 0.821) .. controls (0.577, 0.821) and (0.577, 0.821) .. (0.578, 0.821)
	-- (0.578, 0.822) .. controls (0.579, 0.822) and (0.579, 0.822) .. (0.579, 0.822)
	-- (0.579, 0.823) .. controls (0.579, 0.823) and (0.579, 0.823) .. (0.58, 0.823)
	-- (0.58, 0.823) .. controls (0.58, 0.823) and (0.581, 0.823) .. (0.581, 0.823)
	-- (0.581, 0.824) .. controls (0.581, 0.824) and (0.582, 0.824) .. (0.582, 0.824)
	-- (0.582, 0.825) .. controls (0.583, 0.825) and (0.583, 0.825) .. (0.583, 0.825)
	-- (0.583, 0.825) .. controls (0.584, 0.825) and (0.584, 0.825) .. (0.584, 0.825)
	-- (0.584, 0.826) .. controls (0.585, 0.826) and (0.585, 0.826) .. (0.585, 0.826)
	-- (0.585, 0.827) .. controls (0.586, 0.827) and (0.586, 0.827) .. (0.586, 0.827)
	-- (0.586, 0.827) .. controls (0.586, 0.827) and (0.587, 0.827) .. (0.587, 0.827)
	-- (0.587, 0.828) .. controls (0.587, 0.828) and (0.587, 0.828) .. (0.588, 0.828)
	-- (0.588, 0.829) .. controls (0.589, 0.829) and (0.589, 0.829) .. (0.589, 0.829)
	-- (0.589, 0.829) .. controls (0.589, 0.829) and (0.59, 0.829) .. (0.59, 0.829)
	-- (0.59, 0.83) .. controls (0.59, 0.83) and (0.591, 0.83) .. (0.591, 0.83)
	-- (0.591, 0.831) .. controls (0.591, 0.831) and (0.591, 0.831) .. (0.592, 0.831)
	-- (0.592, 0.831) .. controls (0.593, 0.831) and (0.593, 0.831) .. (0.593, 0.831)
	-- (0.593, 0.832) .. controls (0.593, 0.832) and (0.593, 0.832) .. (0.594, 0.832)
	-- (0.594, 0.833) .. controls (0.594, 0.833) and (0.594, 0.833) .. (0.595, 0.833)
	-- (0.595, 0.834) .. controls (0.596, 0.834) and (0.596, 0.834) .. (0.596, 0.834)
	-- (0.596, 0.834) .. controls (0.597, 0.834) and (0.597, 0.834) .. (0.597, 0.834)
	-- (0.597, 0.835) .. controls (0.597, 0.835) and (0.597, 0.835) .. (0.598, 0.835)
	-- (0.598, 0.836) .. controls (0.598, 0.836) and (0.598, 0.836) .. (0.599, 0.836)
	-- (0.599, 0.836) .. controls (0.599, 0.836) and (0.599, 0.836) .. (0.6, 0.836)
	-- (0.6, 0.837) .. controls (0.601, 0.837) and (0.601, 0.837) .. (0.601, 0.837)
	-- (0.601, 0.838) .. controls (0.601, 0.838) and (0.602, 0.838) .. (0.602, 0.838)
	-- (0.602, 0.839) .. controls (0.602, 0.839) and (0.603, 0.839) .. (0.603, 0.839)
	-- (0.603, 0.839) .. controls (0.603, 0.839) and (0.603, 0.839) .. (0.604, 0.839)
	-- (0.604, 0.84) .. controls (0.604, 0.84) and (0.605, 0.84) .. (0.605, 0.84)
	-- (0.605, 0.841) .. controls (0.605, 0.841) and (0.605, 0.841) .. (0.606, 0.841)
	-- (0.606, 0.842) .. controls (0.606, 0.842) and (0.606, 0.842) .. (0.607, 0.842)
	-- (0.607, 0.842) .. controls (0.608, 0.842) and (0.608, 0.842) .. (0.608, 0.842)
	-- (0.608, 0.843) .. controls (0.609, 0.843) and (0.609, 0.843) .. (0.609, 0.843)
	-- (0.609, 0.844) .. controls (0.609, 0.844) and (0.61, 0.844) .. (0.61, 0.844)
	-- (0.61, 0.845) .. controls (0.61, 0.845) and (0.611, 0.845) .. (0.611, 0.845)
	-- (0.611, 0.845) .. controls (0.611, 0.845) and (0.611, 0.845) .. (0.612, 0.845)
	-- (0.612, 0.846) .. controls (0.613, 0.846) and (0.613, 0.846) .. (0.613, 0.846)
	-- (0.613, 0.847) .. controls (0.614, 0.847) and (0.614, 0.847) .. (0.614, 0.847)
	-- (0.614, 0.848) .. controls (0.615, 0.848) and (0.615, 0.848) .. (0.615, 0.848)
	-- (0.615, 0.848) .. controls (0.615, 0.849) and (0.616, 0.849) .. (0.616, 0.849)
	-- (0.616, 0.849) .. controls (0.616, 0.849) and (0.616, 0.849) .. (0.617, 0.849)
	-- (0.617, 0.85) .. controls (0.618, 0.85) and (0.618, 0.85) .. (0.618, 0.85)
	-- (0.618, 0.851) .. controls (0.618, 0.851) and (0.618, 0.851) .. (0.619, 0.851)
	-- (0.619, 0.852) .. controls (0.619, 0.852) and (0.619, 0.852) .. (0.62, 0.852)
	-- (0.62, 0.853) .. controls (0.621, 0.853) and (0.621, 0.853) .. (0.621, 0.853)
	-- (0.621, 0.853) .. controls (0.621, 0.853) and (0.622, 0.853) .. (0.622, 0.853)
	-- (0.622, 0.854) .. controls (0.622, 0.854) and (0.623, 0.854) .. (0.623, 0.854)
	-- (0.623, 0.855) .. controls (0.624, 0.855) and (0.624, 0.855) .. (0.624, 0.855)
	-- (0.624, 0.856) .. controls (0.624, 0.856) and (0.625, 0.856) .. (0.625, 0.856)
	-- (0.625, 0.857) .. controls (0.625, 0.857) and (0.625, 0.857) .. (0.626, 0.857)
	-- (0.626, 0.857) .. controls (0.627, 0.857) and (0.627, 0.857) .. (0.627, 0.857)
	-- (0.627, 0.858) .. controls (0.628, 0.858) and (0.628, 0.858) .. (0.628, 0.858)
	-- (0.628, 0.859) .. controls (0.628, 0.859) and (0.629, 0.859) .. (0.629, 0.859)
	-- (0.629, 0.86) .. controls (0.629, 0.86) and (0.63, 0.86) .. (0.63, 0.86)
	-- (0.63, 0.861) .. controls (0.63, 0.861) and (0.631, 0.861) .. (0.631, 0.861)
	-- (0.631, 0.862) .. controls (0.632, 0.862) and (0.632, 0.862) .. (0.632, 0.862)
	-- (0.632, 0.862) .. controls (0.632, 0.862) and (0.632, 0.862) .. (0.633, 0.862)
	-- (0.633, 0.863) .. controls (0.634, 0.863) and (0.634, 0.863) .. (0.634, 0.863)
	-- (0.634, 0.864) .. controls (0.634, 0.864) and (0.634, 0.864) .. (0.635, 0.864)
	-- (0.635, 0.865) .. controls (0.635, 0.865) and (0.635, 0.865) .. (0.636, 0.865)
	-- (0.636, 0.866) .. controls (0.636, 0.866) and (0.636, 0.866) .. (0.637, 0.866)
	-- (0.637, 0.866) .. controls (0.638, 0.866) and (0.638, 0.867) .. (0.638, 0.867)
	-- (0.638, 0.867) .. controls (0.638, 0.867) and (0.638, 0.867) .. (0.639, 0.867)
	-- (0.639, 0.868) .. controls (0.64, 0.868) and (0.64, 0.868) .. (0.64, 0.868)
	-- (0.64, 0.869) .. controls (0.64, 0.869) and (0.641, 0.869) .. (0.641, 0.869)
	-- (0.641, 0.87) .. controls (0.641, 0.87) and (0.642, 0.87) .. (0.642, 0.87)
	-- (0.642, 0.87) .. controls (0.642, 0.87) and (0.642, 0.87) .. (0.643, 0.87)
	-- (0.643, 0.871) .. controls (0.644, 0.871) and (0.644, 0.871) .. (0.644, 0.871)
	-- (0.644, 0.872) .. controls (0.645, 0.872) and (0.645, 0.872) .. (0.645, 0.872)
	-- (0.645, 0.873) .. controls (0.645, 0.873) and (0.645, 0.873) .. (0.646, 0.873)
	-- (0.646, 0.874) .. controls (0.646, 0.874) and (0.646, 0.874) .. (0.647, 0.874)
	-- (0.647, 0.874) .. controls (0.647, 0.874) and (0.647, 0.874) .. (0.648, 0.875)
	-- (0.648, 0.875) .. controls (0.648, 0.875) and (0.648, 0.875) .. (0.649, 0.875)
	-- (0.649, 0.876) .. controls (0.649, 0.876) and (0.65, 0.876) .. (0.65, 0.876)
	-- (0.65, 0.877) .. controls (0.651, 0.877) and (0.651, 0.877) .. (0.651, 0.877)
	-- (0.651, 0.878) .. controls (0.652, 0.878) and (0.652, 0.878) .. (0.652, 0.878)
	-- (0.652, 0.878) .. controls (0.653, 0.878) and (0.653, 0.878) .. (0.653, 0.878)
	-- (0.653, 0.879) .. controls (0.653, 0.879) and (0.654, 0.879) .. (0.654, 0.879)
	-- (0.654, 0.88) .. controls (0.654, 0.88) and (0.655, 0.88) .. (0.655, 0.88)
	-- (0.655, 0.881) .. controls (0.656, 0.881) and (0.656, 0.881) .. (0.656, 0.881)
	-- (0.656, 0.882) .. controls (0.657, 0.882) and (0.657, 0.882) .. (0.657, 0.882)
	-- (0.657, 0.882) .. controls (0.658, 0.882) and (0.658, 0.882) .. (0.658, 0.882)
	-- (0.658, 0.883) .. controls (0.659, 0.883) and (0.659, 0.883) .. (0.659, 0.883)
	-- (0.659, 0.884) .. controls (0.659, 0.884) and (0.66, 0.884) .. (0.66, 0.884)
	-- (0.66, 0.885) .. controls (0.66, 0.885) and (0.661, 0.885) .. (0.661, 0.885)
	-- (0.661, 0.886) .. controls (0.661, 0.886) and (0.662, 0.886) .. (0.662, 0.886)
	-- (0.662, 0.886) .. controls (0.662, 0.886) and (0.663, 0.886) .. (0.663, 0.886)
	-- (0.663, 0.887) .. controls (0.663, 0.887) and (0.663, 0.887) .. (0.664, 0.887)
	-- (0.664, 0.888) .. controls (0.664, 0.888) and (0.665, 0.888) .. (0.665, 0.888)
	-- (0.665, 0.889) .. controls (0.666, 0.889) and (0.666, 0.889) .. (0.666, 0.889)
	-- (0.666, 0.89) .. controls (0.666, 0.89) and (0.666, 0.89) .. (0.667, 0.89)
	-- (0.667, 0.89) .. controls (0.667, 0.89) and (0.668, 0.89) .. (0.668, 0.89)
	-- (0.668, 0.891) .. controls (0.668, 0.891) and (0.668, 0.891) .. (0.669, 0.891)
	-- (0.669, 0.892) .. controls (0.67, 0.892) and (0.67, 0.892) .. (0.67, 0.892)
	-- (0.67, 0.893) .. controls (0.671, 0.893) and (0.671, 0.893) .. (0.671, 0.893)
	-- (0.671, 0.893) .. controls (0.671, 0.893) and (0.672, 0.893) .. (0.672, 0.893)
	-- (0.672, 0.894) .. controls (0.672, 0.894) and (0.672, 0.894) .. (0.673, 0.894)
	-- (0.673, 0.895) .. controls (0.673, 0.895) and (0.674, 0.895) .. (0.674, 0.895)
	-- (0.674, 0.895) .. controls (0.674, 0.896) and (0.674, 0.896) .. (0.675, 0.896)
	-- (0.675, 0.896) .. controls (0.676, 0.896) and (0.676, 0.896) .. (0.676, 0.896)
	-- (0.676, 0.897) .. controls (0.676, 0.897) and (0.676, 0.897) .. (0.677, 0.897)
	-- (0.677, 0.898) .. controls (0.678, 0.898) and (0.678, 0.898) .. (0.678, 0.898)
	-- (0.678, 0.898) .. controls (0.679, 0.898) and (0.679, 0.898) .. (0.679, 0.898)
	-- (0.679, 0.899) .. controls (0.68, 0.899) and (0.68, 0.899) .. (0.68, 0.899)
	-- (0.68, 0.9) .. controls (0.68, 0.9) and (0.68, 0.9) .. (0.681, 0.9)
	-- (0.681, 0.9) .. controls (0.681, 0.9) and (0.682, 0.9) .. (0.682, 0.901)
	-- (0.682, 0.901) .. controls (0.682, 0.901) and (0.683, 0.901) .. (0.683, 0.901)
	-- (0.683, 0.902) .. controls (0.683, 0.902) and (0.684, 0.902) .. (0.684, 0.902)
	-- (0.684, 0.902) .. controls (0.684, 0.902) and (0.684, 0.902) .. (0.685, 0.903)
	-- (0.685, 0.903) .. controls (0.685, 0.903) and (0.686, 0.903) .. (0.686, 0.903)
	-- (0.686, 0.904) .. controls (0.686, 0.904) and (0.687, 0.904) .. (0.687, 0.904)
	-- (0.687, 0.904) .. controls (0.687, 0.904) and (0.688, 0.905) .. (0.688, 0.905)
	-- (0.688, 0.905) .. controls (0.688, 0.905) and (0.689, 0.905) .. (0.689, 0.905)
	-- (0.689, 0.906) .. controls (0.69, 0.906) and (0.69, 0.906) .. (0.69, 0.906)
	-- (0.69, 0.907) .. controls (0.69, 0.907) and (0.691, 0.907) .. (0.691, 0.907)
	-- (0.691, 0.907) .. controls (0.692, 0.907) and (0.692, 0.907) .. (0.692, 0.907)
	-- (0.692, 0.908) .. controls (0.692, 0.908) and (0.692, 0.908) .. (0.693, 0.908)
	-- (0.693, 0.909) .. controls (0.693, 0.909) and (0.693, 0.909) .. (0.694, 0.909)
	-- (0.694, 0.909) .. controls (0.694, 0.909) and (0.695, 0.909) .. (0.695, 0.909)
	-- (0.695, 0.91) .. controls (0.695, 0.91) and (0.696, 0.91) .. (0.696, 0.91)
	-- (0.696, 0.911) .. controls (0.697, 0.911) and (0.697, 0.911) .. (0.697, 0.911)
	-- (0.697, 0.911) .. controls (0.697, 0.911) and (0.698, 0.911) .. (0.698, 0.911)
	-- (0.698, 0.912) .. controls (0.699, 0.912) and (0.699, 0.912) .. (0.699, 0.912)
	-- (0.699, 0.912) .. controls (0.699, 0.912) and (0.7, 0.912) .. (0.7, 0.913)
	-- (0.7, 0.913) .. controls (0.7, 0.913) and (0.7, 0.913) .. (0.701, 0.913)
	-- (0.701, 0.914) .. controls (0.701, 0.914) and (0.701, 0.914) .. (0.702, 0.914)
	-- (0.702, 0.914) .. controls (0.703, 0.914) and (0.703, 0.915) .. (0.703, 0.915)
	-- (0.703, 0.915) .. controls (0.703, 0.915) and (0.704, 0.915) .. (0.704, 0.915)
	-- (0.704, 0.916) .. controls (0.704, 0.916) and (0.705, 0.916) .. (0.705, 0.916)
	-- (0.705, 0.916) .. controls (0.706, 0.916) and (0.706, 0.916) .. (0.706, 0.916)
	-- (0.706, 0.917) .. controls (0.707, 0.917) and (0.707, 0.917) .. (0.707, 0.917)
	-- (0.707, 0.918) .. controls (0.708, 0.918) and (0.708, 0.918) .. (0.708, 0.918)
	-- (0.708, 0.918) .. controls (0.708, 0.918) and (0.708, 0.918) .. (0.709, 0.918)
	-- (0.709, 0.919) .. controls (0.709, 0.919) and (0.709, 0.919) .. (0.71, 0.919)
	-- (0.71, 0.919) .. controls (0.711, 0.919) and (0.711, 0.919) .. (0.711, 0.919)
	-- (0.711, 0.92) .. controls (0.711, 0.92) and (0.712, 0.92) .. (0.712, 0.92)
	-- (0.712, 0.921) .. controls (0.713, 0.921) and (0.713, 0.921) .. (0.713, 0.921)
	-- (0.713, 0.921) .. controls (0.713, 0.921) and (0.714, 0.921) .. (0.714, 0.921)
	-- (0.714, 0.922) .. controls (0.715, 0.922) and (0.715, 0.922) .. (0.715, 0.922)
	-- (0.715, 0.923) .. controls (0.715, 0.923) and (0.715, 0.923) .. (0.716, 0.923)
	-- (0.716, 0.923) .. controls (0.716, 0.923) and (0.716, 0.923) .. (0.717, 0.923)
	-- (0.717, 0.924) .. controls (0.717, 0.924) and (0.717, 0.924) .. (0.718, 0.924)
	-- (0.718, 0.924) .. controls (0.719, 0.925) and (0.719, 0.925) .. (0.719, 0.925)
	-- (0.719, 0.925) .. controls (0.719, 0.925) and (0.72, 0.925) .. (0.72, 0.925)
	-- (0.72, 0.926) .. controls (0.72, 0.926) and (0.721, 0.926) .. (0.721, 0.926)
	-- (0.721, 0.926) .. controls (0.721, 0.926) and (0.722, 0.926) .. (0.722, 0.926)
	-- (0.722, 0.927) .. controls (0.723, 0.927) and (0.723, 0.927) .. (0.723, 0.927)
	-- (0.723, 0.928) .. controls (0.723, 0.928) and (0.724, 0.928) .. (0.724, 0.928)
	-- (0.724, 0.928) .. controls (0.724, 0.928) and (0.724, 0.928) .. (0.725, 0.928)
	-- (0.725, 0.929) .. controls (0.726, 0.929) and (0.726, 0.929) .. (0.726, 0.929)
	-- (0.726, 0.93) .. controls (0.727, 0.93) and (0.727, 0.93) .. (0.727, 0.93)
	-- (0.727, 0.93) .. controls (0.727, 0.93) and (0.728, 0.93) .. (0.728, 0.93)
	-- (0.728, 0.931) .. controls (0.728, 0.931) and (0.729, 0.931) .. (0.729, 0.931)
	-- (0.729, 0.931) .. controls (0.729, 0.931) and (0.729, 0.931) .. (0.73, 0.931)
	-- (0.73, 0.932) .. controls (0.731, 0.932) and (0.731, 0.932) .. (0.731, 0.932)
	-- (0.731, 0.933) .. controls (0.731, 0.933) and (0.731, 0.933) .. (0.732, 0.933)
	-- (0.732, 0.933) .. controls (0.733, 0.933) and (0.733, 0.933) .. (0.733, 0.933)
	-- (0.733, 0.934) .. controls (0.734, 0.934) and (0.734, 0.934) .. (0.734, 0.934)
	-- (0.734, 0.935) .. controls (0.734, 0.935) and (0.735, 0.935) .. (0.735, 0.935)
	-- (0.735, 0.935) .. controls (0.735, 0.935) and (0.735, 0.935) .. (0.736, 0.935)
	-- (0.736, 0.936) .. controls (0.737, 0.936) and (0.737, 0.936) .. (0.737, 0.936)
	-- (0.737, 0.936) .. controls (0.737, 0.936) and (0.738, 0.937) .. (0.738, 0.937)
	-- (0.738, 0.937) .. controls (0.739, 0.937) and (0.739, 0.937) .. (0.739, 0.937)
	-- (0.739, 0.938) .. controls (0.739, 0.938) and (0.739, 0.938) .. (0.74, 0.938)
	-- (0.74, 0.938) .. controls (0.74, 0.938) and (0.741, 0.938) .. (0.741, 0.938)
	-- (0.741, 0.939) .. controls (0.741, 0.939) and (0.741, 0.939) .. (0.742, 0.939)
	-- (0.742, 0.94) .. controls (0.743, 0.94) and (0.743, 0.94) .. (0.743, 0.94)
	-- (0.743, 0.94) .. controls (0.744, 0.94) and (0.744, 0.94) .. (0.744, 0.94)
	-- (0.744, 0.941) .. controls (0.744, 0.941) and (0.744, 0.941) .. (0.745, 0.941)
	-- (0.745, 0.941) .. controls (0.746, 0.941) and (0.746, 0.942) .. (0.746, 0.942)
	-- (0.746, 0.942) .. controls (0.746, 0.942) and (0.746, 0.942) .. (0.747, 0.942)
	-- (0.747, 0.943) .. controls (0.748, 0.943) and (0.748, 0.943) .. (0.748, 0.943)
	-- (0.748, 0.943) .. controls (0.748, 0.943) and (0.748, 0.943) .. (0.749, 0.943)
	-- (0.749, 0.944) .. controls (0.75, 0.944) and (0.75, 0.944) .. (0.75, 0.944)
	-- (0.75, 0.945) .. controls (0.751, 0.945) and (0.751, 0.945) .. (0.751, 0.945)
	-- (0.751, 0.945) .. controls (0.752, 0.945) and (0.752, 0.945) .. (0.752, 0.945)
	-- (0.752, 0.946) .. controls (0.752, 0.946) and (0.752, 0.946) .. (0.753, 0.946)
	-- (0.753, 0.946) .. controls (0.754, 0.946) and (0.754, 0.947) .. (0.754, 0.947)
	-- (0.754, 0.947) .. controls (0.755, 0.947) and (0.755, 0.947) .. (0.755, 0.947)
	-- (0.755, 0.948) .. controls (0.755, 0.948) and (0.756, 0.948) .. (0.756, 0.948)
	-- (0.756, 0.948) .. controls (0.757, 0.948) and (0.757, 0.948) .. (0.757, 0.948)
	-- (0.757, 0.949) .. controls (0.758, 0.949) and (0.758, 0.949) .. (0.758, 0.949)
	-- (0.758, 0.95) .. controls (0.758, 0.95) and (0.759, 0.95) .. (0.759, 0.95)
	-- (0.759, 0.95) .. controls (0.759, 0.95) and (0.76, 0.95) .. (0.76, 0.95)
	-- (0.76, 0.951) .. controls (0.761, 0.951) and (0.761, 0.951) .. (0.761, 0.951)
	-- (0.761, 0.951) .. controls (0.762, 0.951) and (0.762, 0.951) .. (0.762, 0.952)
	-- (0.762, 0.952) .. controls (0.762, 0.952) and (0.762, 0.952) .. (0.763, 0.952)
	-- (0.763, 0.953) .. controls (0.763, 0.953) and (0.764, 0.953) .. (0.764, 0.953)
	-- (0.764, 0.953) .. controls (0.764, 0.953) and (0.765, 0.953) .. (0.765, 0.953)
	-- (0.765, 0.954) .. controls (0.765, 0.954) and (0.765, 0.954) .. (0.766, 0.954)
	-- (0.766, 0.954) .. controls (0.767, 0.954) and (0.767, 0.954) .. (0.767, 0.954)
	-- (0.767, 0.955) .. controls (0.767, 0.955) and (0.767, 0.955) .. (0.768, 0.955)
	-- (0.768, 0.955) .. controls (0.768, 0.955) and (0.769, 0.955) .. (0.769, 0.955)
	-- (0.769, 0.956) .. controls (0.77, 0.956) and (0.77, 0.956) .. (0.77, 0.956)
	-- (0.77, 0.956) .. controls (0.77, 0.956) and (0.77, 0.956) .. (0.771, 0.957)
	-- (0.771, 0.957) .. controls (0.771, 0.957) and (0.772, 0.957) .. (0.772, 0.957)
	-- (0.772, 0.958) .. controls (0.773, 0.958) and (0.773, 0.958) .. (0.773, 0.958)
	-- (0.773, 0.958) .. controls (0.773, 0.958) and (0.773, 0.958) .. (0.774, 0.958)
	-- (0.774, 0.959) .. controls (0.775, 0.959) and (0.775, 0.959) .. (0.775, 0.959)
	-- (0.775, 0.959) .. controls (0.775, 0.959) and (0.775, 0.959) .. (0.776, 0.959)
	-- (0.776, 0.96) .. controls (0.776, 0.96) and (0.777, 0.96) .. (0.777, 0.96)
	-- (0.777, 0.96) .. controls (0.777, 0.96) and (0.777, 0.96) .. (0.778, 0.96)
	-- (0.778, 0.961) .. controls (0.779, 0.961) and (0.779, 0.961) .. (0.779, 0.961)
	-- (0.779, 0.961) .. controls (0.779, 0.961) and (0.779, 0.961) .. (0.78, 0.961)
	-- (0.78, 0.962) .. controls (0.78, 0.962) and (0.78, 0.962) .. (0.781, 0.962)
	-- (0.781, 0.962) .. controls (0.781, 0.962) and (0.782, 0.962) .. (0.782, 0.962)
	-- (0.782, 0.963) .. controls (0.782, 0.963) and (0.782, 0.963) .. (0.783, 0.963)
	-- (0.783, 0.963) .. controls (0.783, 0.964) and (0.784, 0.964) .. (0.784, 0.964)
	-- (0.784, 0.964) .. controls (0.784, 0.964) and (0.784, 0.964) .. (0.785, 0.964)
	-- (0.785, 0.965) .. controls (0.786, 0.965) and (0.786, 0.965) .. (0.786, 0.965)
	-- (0.786, 0.965) .. controls (0.786, 0.965) and (0.786, 0.965) .. (0.787, 0.965)
	-- (0.787, 0.966) .. controls (0.788, 0.966) and (0.788, 0.966) .. (0.788, 0.966)
	-- (0.788, 0.966) .. controls (0.789, 0.966) and (0.789, 0.966) .. (0.789, 0.966)
	-- (0.789, 0.967) .. controls (0.789, 0.967) and (0.789, 0.967) .. (0.79, 0.967)
	-- (0.79, 0.967) .. controls (0.79, 0.967) and (0.79, 0.967) .. (0.791, 0.967)
	-- (0.791, 0.968) .. controls (0.791, 0.968) and (0.791, 0.968) .. (0.792, 0.968)
	-- (0.792, 0.968) .. controls (0.792, 0.968) and (0.792, 0.968) .. (0.793, 0.968)
	-- (0.793, 0.969) .. controls (0.793, 0.969) and (0.794, 0.969) .. (0.794, 0.969)
	-- (0.794, 0.969) .. controls (0.794, 0.969) and (0.795, 0.969) .. (0.795, 0.969)
	-- (0.795, 0.97) .. controls (0.795, 0.97) and (0.795, 0.97) .. (0.796, 0.97)
	-- (0.796, 0.97) .. controls (0.796, 0.97) and (0.796, 0.97) .. (0.797, 0.97)
	-- (0.797, 0.971) .. controls (0.798, 0.971) and (0.798, 0.971) .. (0.798, 0.971)
	-- (0.798, 0.971) .. controls (0.799, 0.971) and (0.799, 0.971) .. (0.799, 0.971)
	-- (0.799, 0.972) .. controls (0.8, 0.972) and (0.8, 0.972) .. (0.8, 0.972)
	-- (0.8, 0.972) .. controls (0.8, 0.972) and (0.801, 0.972) .. (0.801, 0.972)
	-- (0.801, 0.973) .. controls (0.801, 0.973) and (0.801, 0.973) .. (0.802, 0.973)
	-- (0.802, 0.973) .. controls (0.803, 0.973) and (0.803, 0.973) .. (0.803, 0.974)
	-- (0.803, 0.974) .. controls (0.804, 0.974) and (0.804, 0.974) .. (0.804, 0.974)
	-- (0.804, 0.974) .. controls (0.804, 0.974) and (0.805, 0.974) .. (0.805, 0.974)
	-- (0.805, 0.975) .. controls (0.806, 0.975) and (0.806, 0.975) .. (0.806, 0.975)
	-- (0.806, 0.975) .. controls (0.806, 0.975) and (0.807, 0.975) .. (0.807, 0.975)
	-- (0.807, 0.976) .. controls (0.808, 0.976) and (0.808, 0.976) .. (0.808, 0.976)
	-- (0.808, 0.976) .. controls (0.808, 0.976) and (0.809, 0.977) .. (0.809, 0.977)
	-- (0.809, 0.977) .. controls (0.81, 0.977) and (0.81, 0.977) .. (0.81, 0.977)
	-- (0.81, 0.978) .. controls (0.811, 0.978) and (0.811, 0.978) .. (0.811, 0.978)
	-- (0.811, 0.978) .. controls (0.811, 0.978) and (0.812, 0.978) .. (0.812, 0.978)
	-- (0.812, 0.979) .. controls (0.813, 0.979) and (0.813, 0.979) .. (0.813, 0.979)
	-- (0.813, 0.979) .. controls (0.813, 0.979) and (0.814, 0.979) .. (0.814, 0.979)
	-- (0.814, 0.98) .. controls (0.814, 0.98) and (0.815, 0.98) .. (0.815, 0.98)
	-- (0.815, 0.98) .. controls (0.815, 0.98) and (0.816, 0.98) .. (0.816, 0.98)
	-- (0.816, 0.981) .. controls (0.816, 0.981) and (0.817, 0.981) .. (0.817, 0.981)
	-- (0.817, 0.981) .. controls (0.817, 0.981) and (0.817, 0.981) .. (0.818, 0.981)
	-- (0.818, 0.982) .. controls (0.818, 0.982) and (0.818, 0.982) .. (0.819, 0.982)
	-- (0.819, 0.982) .. controls (0.82, 0.982) and (0.82, 0.982) .. (0.82, 0.983)
	-- (0.82, 0.983) .. controls (0.82, 0.983) and (0.821, 0.983) .. (0.821, 0.983)
	-- (0.821, 0.983) .. controls (0.822, 0.983) and (0.822, 0.983) .. (0.822, 0.983)
	-- (0.822, 0.984) .. controls (0.822, 0.984) and (0.822, 0.984) .. (0.823, 0.984)
	-- (0.823, 0.984) .. controls (0.823, 0.984) and (0.823, 0.984) .. (0.824, 0.984)
	-- (0.824, 0.985) .. controls (0.824, 0.985) and (0.825, 0.985) .. (0.825, 0.985)
	-- (0.825, 0.985) .. controls (0.826, 0.985) and (0.826, 0.985) .. (0.826, 0.985)
	-- (0.826, 0.986) .. controls (0.826, 0.986) and (0.827, 0.986) .. (0.827, 0.986)
	-- (0.827, 0.986) .. controls (0.827, 0.986) and (0.828, 0.986) .. (0.828, 0.986)
	-- (0.828, 0.987) .. controls (0.829, 0.987) and (0.829, 0.987) .. (0.829, 0.987)
	-- (0.829, 0.987) .. controls (0.829, 0.987) and (0.829, 0.987) .. (0.83, 0.987)
	-- (0.83, 0.988) .. controls (0.831, 0.988) and (0.831, 0.988) .. (0.831, 0.988)
	-- (0.831, 0.988) .. controls (0.831, 0.988) and (0.831, 0.988) .. (0.832, 0.988)
	-- (0.832, 0.989) .. controls (0.832, 0.989) and (0.833, 0.989) .. (0.833, 0.989)
	-- (0.833, 0.989) .. controls (0.833, 0.989) and (0.834, 0.989) .. (0.834, 0.989)
	-- (0.834, 0.99) .. controls (0.835, 0.99) and (0.835, 0.99) .. (0.835, 0.99)
	-- (0.835, 0.99) .. controls (0.836, 0.99) and (0.836, 0.99) .. (0.836, 0.99)
	-- (0.836, 0.991) .. controls (0.836, 0.991) and (0.837, 0.991) .. (0.837, 0.991)
	-- (0.837, 0.991) .. controls (0.837, 0.991) and (0.838, 0.992) .. (0.838, 0.992)
	-- (0.838, 0.992) .. controls (0.838, 0.992) and (0.838, 0.992) .. (0.839, 0.992)
	-- (0.839, 0.993) .. controls (0.839, 0.993) and (0.839, 0.993) .. (0.84, 0.993)
	-- (0.84, 0.993) .. controls (0.841, 0.993) and (0.841, 0.993) .. (0.841, 0.993)
	-- (0.841, 0.994) .. controls (0.841, 0.994) and (0.842, 0.994) .. (0.842, 0.994)
	-- (0.842, 0.994) .. controls (0.842, 0.994) and (0.842, 0.994) .. (0.843, 0.994)
	-- (0.843, 0.995) .. controls (0.843, 0.995) and (0.844, 0.995) .. (0.844, 0.995)
	-- (0.844, 0.995) .. controls (0.844, 0.995) and (0.844, 0.995) .. (0.845, 0.995)
	-- (0.845, 0.996) .. controls (0.846, 0.996) and (0.846, 0.996) .. (0.846, 0.996)
	-- (0.846, 0.996) .. controls (0.846, 0.996) and (0.847, 0.996) .. (0.847, 0.996)
	-- (0.847, 0.997) .. controls (0.847, 0.997) and (0.848, 0.997) .. (0.848, 0.997)
	-- (0.848, 0.997) .. controls (0.849, 0.997) and (0.849, 0.997) .. (0.849, 0.998)
	-- (0.849, 0.998) .. controls (0.849, 0.998) and (0.849, 0.998) .. (0.85, 0.998)
	-- (0.85, 0.999) .. controls (0.851, 0.999) and (0.851, 0.999) .. (0.851, 0.999)
	-- (0.851, 0.999) .. controls (0.851, 0.999) and (0.852, 0.999) .. (0.852, 0.999)
	-- (0.852, 1.0) .. controls (0.852, 1.0) and (0.853, 1.0) .. (0.853, 1.0)
	-- (0.853, 1.0) .. controls (0.853, 1.0) and (0.854, 1.0) .. (0.854, 1.0)
	-- (0.854, 1.001) .. controls (0.855, 1.001) and (0.855, 1.001) .. (0.855, 1.001)
	-- (0.855, 1.001) .. controls (0.855, 1.001) and (0.856, 1.001) .. (0.856, 1.001)
	-- (0.856, 1.002) .. controls (0.857, 1.002) and (0.857, 1.002) .. (0.857, 1.002)
	-- (0.857, 1.003) .. controls (0.857, 1.003) and (0.858, 1.003) .. (0.858, 1.003)
	-- (0.858, 1.003) .. controls (0.858, 1.003) and (0.858, 1.003) .. (0.859, 1.003)
	-- (0.859, 1.004) .. controls (0.859, 1.004) and (0.86, 1.004) .. (0.86, 1.004)
	-- (0.86, 1.004) .. controls (0.86, 1.004) and (0.86, 1.004) .. (0.861, 1.004)
	-- (0.861, 1.005) .. controls (0.862, 1.005) and (0.862, 1.005) .. (0.862, 1.005)
	-- (0.862, 1.006) .. controls (0.863, 1.006) and (0.863, 1.006) .. (0.863, 1.006)
	-- (0.863, 1.006) .. controls (0.864, 1.006) and (0.864, 1.006) .. (0.864, 1.006)
	-- (0.864, 1.007) .. controls (0.865, 1.007) and (0.865, 1.007) .. (0.865, 1.007)
	-- (0.865, 1.007) .. controls (0.865, 1.007) and (0.866, 1.007) .. (0.866, 1.008)
	-- (0.866, 1.008) .. controls (0.866, 1.008) and (0.866, 1.008) .. (0.867, 1.008)
	-- (0.867, 1.009) .. controls (0.867, 1.009) and (0.867, 1.009) .. (0.868, 1.009)
	-- (0.868, 1.009) .. controls (0.868, 1.009) and (0.868, 1.009) .. (0.869, 1.009)
	-- (0.869, 1.01) .. controls (0.87, 1.01) and (0.87, 1.01) .. (0.87, 1.01)
	-- (0.87, 1.011) .. controls (0.87, 1.011) and (0.871, 1.011) .. (0.871, 1.011)
	-- (0.871, 1.011) .. controls (0.871, 1.011) and (0.871, 1.011) .. (0.872, 1.011)
	-- (0.872, 1.012) .. controls (0.873, 1.012) and (0.873, 1.012) .. (0.873, 1.012)
	-- (0.873, 1.012) .. controls (0.873, 1.012) and (0.873, 1.012) .. (0.874, 1.013)
	-- (0.874, 1.013) .. controls (0.874, 1.013) and (0.875, 1.013) .. (0.875, 1.013)
	-- (0.875, 1.014) .. controls (0.876, 1.014) and (0.876, 1.014) .. (0.876, 1.014)
	-- (0.876, 1.014) .. controls (0.876, 1.014) and (0.876, 1.014) .. (0.877, 1.015)
	-- (0.877, 1.015) .. controls (0.878, 1.015) and (0.878, 1.015) .. (0.878, 1.015)
	-- (0.878, 1.016) .. controls (0.878, 1.016) and (0.879, 1.016) .. (0.879, 1.016)
	-- (0.879, 1.016) .. controls (0.879, 1.016) and (0.88, 1.017) .. (0.88, 1.017)
	-- (0.88, 1.017) .. controls (0.88, 1.017) and (0.881, 1.017) .. (0.881, 1.017)
	-- (0.881, 1.018) .. controls (0.882, 1.018) and (0.882, 1.018) .. (0.882, 1.018)
	-- (0.882, 1.018) .. controls (0.882, 1.019) and (0.883, 1.019) .. (0.883, 1.019)
	-- (0.883, 1.019) .. controls (0.883, 1.019) and (0.883, 1.019) .. (0.884, 1.019)
	-- (0.884, 1.02) .. controls (0.884, 1.02) and (0.884, 1.02) .. (0.885, 1.02)
	-- (0.885, 1.021) .. controls (0.886, 1.021) and (0.886, 1.021) .. (0.886, 1.021)
	-- (0.886, 1.021) .. controls (0.886, 1.021) and (0.887, 1.021) .. (0.887, 1.021)
	-- (0.887, 1.022) .. controls (0.887, 1.022) and (0.887, 1.022) .. (0.888, 1.022)
	-- (0.888, 1.022) .. controls (0.888, 1.023) and (0.889, 1.023) .. (0.889, 1.023)
	-- (0.889, 1.023) .. controls (0.89, 1.023) and (0.89, 1.023) .. (0.89, 1.023)
	-- (0.89, 1.024) .. controls (0.89, 1.024) and (0.891, 1.024) .. (0.891, 1.024)
	-- (0.891, 1.025) .. controls (0.891, 1.025) and (0.892, 1.025) .. (0.892, 1.025)
	-- (0.892, 1.025) .. controls (0.892, 1.025) and (0.892, 1.025) .. (0.893, 1.025)
	-- (0.893, 1.026) .. controls (0.893, 1.026) and (0.893, 1.026) .. (0.894, 1.026)
	-- (0.894, 1.027) .. controls (0.894, 1.027) and (0.895, 1.027) .. (0.895, 1.027)
	-- (0.895, 1.027) .. controls (0.895, 1.027) and (0.896, 1.027) .. (0.896, 1.027)
	-- (0.896, 1.028) .. controls (0.896, 1.028) and (0.896, 1.028) .. (0.897, 1.028)
	-- (0.897, 1.029) .. controls (0.898, 1.029) and (0.898, 1.029) .. (0.898, 1.029)
	-- (0.898, 1.029) .. controls (0.899, 1.029) and (0.899, 1.029) .. (0.899, 1.029)
	-- (0.899, 1.03) .. controls (0.899, 1.03) and (0.899, 1.03) .. (0.9, 1.03)
	-- (0.9, 1.031) .. controls (0.901, 1.031) and (0.901, 1.031) .. (0.901, 1.031)
	-- (0.901, 1.031) .. controls (0.902, 1.031) and (0.902, 1.031) .. (0.902, 1.031)
	-- (0.902, 1.032) .. controls (0.902, 1.032) and (0.903, 1.032) .. (0.903, 1.032)
	-- (0.903, 1.033) .. controls (0.903, 1.033) and (0.904, 1.033) .. (0.904, 1.033)
	-- (0.904, 1.033) .. controls (0.905, 1.033) and (0.905, 1.033) .. (0.905, 1.033)
	-- (0.905, 1.034) .. controls (0.906, 1.034) and (0.906, 1.034) .. (0.906, 1.034)
	-- (0.906, 1.035) .. controls (0.906, 1.035) and (0.906, 1.035) .. (0.907, 1.035)
	-- (0.907, 1.035) .. controls (0.907, 1.035) and (0.907, 1.035) .. (0.908, 1.035)
	-- (0.908, 1.036) .. controls (0.908, 1.036) and (0.909, 1.036) .. (0.909, 1.036)
	-- (0.909, 1.037) .. controls (0.909, 1.037) and (0.91, 1.037) .. (0.91, 1.037)
	-- (0.91, 1.037) .. controls (0.91, 1.037) and (0.911, 1.037) .. (0.911, 1.037)
	-- (0.911, 1.038) .. controls (0.911, 1.038) and (0.911, 1.038) .. (0.912, 1.038)
	-- (0.912, 1.039) .. controls (0.912, 1.039) and (0.912, 1.039) .. (0.913, 1.039)
	-- (0.913, 1.04) .. controls (0.914, 1.04) and (0.914, 1.04) .. (0.914, 1.04)
	-- (0.914, 1.04) .. controls (0.915, 1.04) and (0.915, 1.04) .. (0.915, 1.04)
	-- (0.915, 1.041) .. controls (0.916, 1.041) and (0.916, 1.041) .. (0.916, 1.041)
	-- (0.916, 1.042) .. controls (0.916, 1.042) and (0.916, 1.042) .. (0.917, 1.042)
	-- (0.917, 1.042) .. controls (0.918, 1.042) and (0.918, 1.042) .. (0.918, 1.042)
	-- (0.918, 1.043) .. controls (0.918, 1.043) and (0.918, 1.043) .. (0.919, 1.043)
	-- (0.919, 1.044) .. controls (0.919, 1.044) and (0.92, 1.044) .. (0.92, 1.044)
	-- (0.92, 1.044) .. controls (0.92, 1.044) and (0.92, 1.044) .. (0.921, 1.044)
	-- (0.921, 1.045) .. controls (0.921, 1.045) and (0.921, 1.045) .. (0.922, 1.045)
	-- (0.922, 1.046) .. controls (0.923, 1.046) and (0.923, 1.046) .. (0.923, 1.046)
	-- (0.923, 1.046) .. controls (0.923, 1.047) and (0.924, 1.047) .. (0.924, 1.047)
	-- (0.924, 1.047) .. controls (0.924, 1.047) and (0.925, 1.047) .. (0.925, 1.047)
	-- (0.925, 1.048) .. controls (0.926, 1.048) and (0.926, 1.048) .. (0.926, 1.048)
	-- (0.926, 1.049) .. controls (0.927, 1.049) and (0.927, 1.049) .. (0.927, 1.049)
	-- (0.927, 1.049) .. controls (0.927, 1.049) and (0.928, 1.049) .. (0.928, 1.05)
	-- (0.928, 1.05) .. controls (0.929, 1.05) and (0.929, 1.05) .. (0.929, 1.05)
	-- (0.929, 1.051) .. controls (0.93, 1.051) and (0.93, 1.051) .. (0.93, 1.051)
	-- (0.93, 1.052) .. controls (0.93, 1.052) and (0.931, 1.052) .. (0.931, 1.052)
	-- (0.931, 1.052) .. controls (0.932, 1.052) and (0.932, 1.052) .. (0.932, 1.053)
	-- (0.932, 1.053) .. controls (0.932, 1.053) and (0.933, 1.053) .. (0.933, 1.053)
	-- (0.933, 1.054) .. controls (0.933, 1.054) and (0.934, 1.054) .. (0.934, 1.054)
	-- (0.934, 1.055) .. controls (0.934, 1.055) and (0.935, 1.055) .. (0.935, 1.055)
	-- (0.935, 1.055) .. controls (0.935, 1.055) and (0.935, 1.055) .. (0.936, 1.055)
	-- (0.936, 1.056) .. controls (0.937, 1.056) and (0.937, 1.056) .. (0.937, 1.056)
	-- (0.937, 1.057) .. controls (0.938, 1.057) and (0.938, 1.057) .. (0.938, 1.057)
	-- (0.938, 1.058) .. controls (0.938, 1.058) and (0.939, 1.058) .. (0.939, 1.058)
	-- (0.939, 1.058) .. controls (0.94, 1.058) and (0.94, 1.059) .. (0.94, 1.059)
	-- (0.94, 1.059) .. controls (0.941, 1.059) and (0.941, 1.059) .. (0.941, 1.059)
	-- (0.941, 1.06) .. controls (0.942, 1.06) and (0.942, 1.06) .. (0.942, 1.06)
	-- (0.942, 1.061) .. controls (0.943, 1.061) and (0.943, 1.061) .. (0.943, 1.061)
	-- (0.943, 1.061) .. controls (0.944, 1.062) and (0.944, 1.062) .. (0.944, 1.062)
	-- (0.944, 1.062) .. controls (0.944, 1.062) and (0.945, 1.062) .. (0.945, 1.062)
	-- (0.945, 1.063) .. controls (0.946, 1.063) and (0.946, 1.063) .. (0.946, 1.063)
	-- (0.946, 1.064) .. controls (0.946, 1.064) and (0.947, 1.064) .. (0.947, 1.064)
	-- (0.947, 1.065) .. controls (0.947, 1.065) and (0.948, 1.065) .. (0.948, 1.065)
	-- (0.948, 1.065) .. controls (0.948, 1.065) and (0.949, 1.065) .. (0.949, 1.065)
	-- (0.949, 1.066) .. controls (0.949, 1.066) and (0.95, 1.066) .. (0.95, 1.066)
	-- (0.95, 1.067) .. controls (0.951, 1.067) and (0.951, 1.067) .. (0.951, 1.067)
	-- (0.951, 1.068) .. controls (0.952, 1.068) and (0.952, 1.068) .. (0.952, 1.068)
	-- (0.952, 1.068) .. controls (0.952, 1.068) and (0.952, 1.068) .. (0.953, 1.068)
	-- (0.953, 1.069) .. controls (0.953, 1.069) and (0.954, 1.069) .. (0.954, 1.069)
	-- (0.954, 1.07) .. controls (0.955, 1.07) and (0.955, 1.07) .. (0.955, 1.07)
	-- (0.955, 1.071) .. controls (0.956, 1.071) and (0.956, 1.071) .. (0.956, 1.071)
	-- (0.956, 1.071) .. controls (0.957, 1.071) and (0.957, 1.071) .. (0.957, 1.071)
	-- (0.957, 1.072) .. controls (0.957, 1.072) and (0.958, 1.072) .. (0.958, 1.072)
	-- (0.958, 1.073) .. controls (0.959, 1.073) and (0.959, 1.073) .. (0.959, 1.073)
	-- (0.959, 1.074) .. controls (0.96, 1.074) and (0.96, 1.074) .. (0.96, 1.074)
	-- (0.96, 1.074) .. controls (0.96, 1.074) and (0.96, 1.074) .. (0.961, 1.074)
	-- (0.961, 1.075) .. controls (0.962, 1.075) and (0.962, 1.075) .. (0.962, 1.075)
	-- (0.962, 1.076) .. controls (0.962, 1.076) and (0.963, 1.076) .. (0.963, 1.076)
	-- (0.963, 1.077) .. controls (0.963, 1.077) and (0.963, 1.077) .. (0.964, 1.077)
	-- (0.964, 1.077) .. controls (0.964, 1.077) and (0.964, 1.077) .. (0.965, 1.077)
	-- (0.965, 1.078) .. controls (0.966, 1.078) and (0.966, 1.079) .. (0.966, 1.079)
	-- (0.966, 1.079) .. controls (0.966, 1.079) and (0.967, 1.079) .. (0.967, 1.079)
	-- (0.967, 1.08) .. controls (0.967, 1.08) and (0.968, 1.08) .. (0.968, 1.08)
	-- (0.968, 1.08) .. controls (0.968, 1.081) and (0.969, 1.081) .. (0.969, 1.081)
	-- (0.969, 1.081) .. controls (0.969, 1.081) and (0.969, 1.081) .. (0.97, 1.081)
	-- (0.97, 1.082) .. controls (0.971, 1.082) and (0.971, 1.082) .. (0.971, 1.082)
	-- (0.971, 1.083) .. controls (0.972, 1.083) and (0.972, 1.083) .. (0.972, 1.083)
	-- (0.972, 1.084) .. controls (0.972, 1.084) and (0.973, 1.084) .. (0.973, 1.084)
	-- (0.973, 1.084) .. controls (0.973, 1.084) and (0.973, 1.084) .. (0.974, 1.084)
	-- (0.974, 1.085) .. controls (0.975, 1.085) and (0.975, 1.085) .. (0.975, 1.085)
	-- (0.975, 1.086) .. controls (0.976, 1.086) and (0.976, 1.086) .. (0.976, 1.086)
	-- (0.976, 1.087) .. controls (0.976, 1.087) and (0.976, 1.087) .. (0.977, 1.087)
	-- (0.977, 1.088) .. controls (0.978, 1.088) and (0.978, 1.088) .. (0.978, 1.088)
	-- (0.978, 1.088) .. controls (0.978, 1.088) and (0.979, 1.088) .. (0.979, 1.089)
	-- (0.979, 1.089) .. controls (0.98, 1.089) and (0.98, 1.089) .. (0.98, 1.089)
	-- (0.98, 1.09) .. controls (0.981, 1.09) and (0.981, 1.09) .. (0.981, 1.09)
	-- (0.981, 1.091) .. controls (0.982, 1.091) and (0.982, 1.091) .. (0.982, 1.091)
	-- (0.982, 1.092) .. controls (0.983, 1.092) and (0.983, 1.092) .. (0.983, 1.092)
	-- (0.983, 1.093) .. controls (0.983, 1.093) and (0.983, 1.093) .. (0.984, 1.093)
	-- (0.984, 1.093) .. controls (0.984, 1.093) and (0.985, 1.093) .. (0.985, 1.093)
	-- (0.985, 1.094) .. controls (0.986, 1.094) and (0.986, 1.094) .. (0.986, 1.094)
	-- (0.986, 1.095) .. controls (0.986, 1.095) and (0.987, 1.095) .. (0.987, 1.095)
	-- (0.987, 1.096) .. controls (0.988, 1.096) and (0.988, 1.096) .. (0.988, 1.096)
	-- (0.988, 1.097) .. controls (0.989, 1.097) and (0.989, 1.097) .. (0.989, 1.097)
	-- (0.989, 1.098) .. controls (0.989, 1.098) and (0.989, 1.098) .. (0.99, 1.098)
	-- (0.99, 1.099) .. controls (0.991, 1.099) and (0.991, 1.099) .. (0.991, 1.099)
	-- (0.991, 1.1) .. controls (0.992, 1.1) and (0.992, 1.1) .. (0.992, 1.1)
	-- (0.992, 1.1) .. controls (0.993, 1.1) and (0.993, 1.1) .. (0.993, 1.1)
	-- (0.993, 1.101) .. controls (0.993, 1.101) and (0.994, 1.101) .. (0.994, 1.101)
	-- (0.994, 1.102) .. controls (0.994, 1.102) and (0.995, 1.102) .. (0.995, 1.102)
	-- (0.995, 1.103) .. controls (0.996, 1.103) and (0.996, 1.103) .. (0.996, 1.103)
	-- (0.996, 1.104) .. controls (0.996, 1.104) and (0.997, 1.104) .. (0.997, 1.104)
	-- (0.997, 1.105) .. controls (0.998, 1.105) and (0.998, 1.105) .. (0.998, 1.105)
	-- (0.998, 1.106) .. controls (0.999, 1.106) and (0.999, 1.106) .. (0.999, 1.106)
	-- (0.999, 1.107) .. controls (1.0, 1.107) and (1.0, 1.107) .. (1.0, 1.107)
	;


==> figure/alo-comp/plot.tex <==
\input mac/m

\definecolor{cat1}{RGB}{0, 114, 190}
\definecolor{cat2}{RGB}{218, 83, 25}

\tikzpicture[xscale=12, yscale=5.0]

  \def\yaxis{-0.025}
  \def\xaxis{0.45}
  \def\ticksize{.1cm}
  \def\xtick{\ticksize/12}
  \def\ytick{\ticksize/5.0}

  \draw (\yaxis,0.58) -- (\yaxis, 1.1);
  \draw (0, \xaxis) -- (1, \xaxis);

  \scope[color=cat1, semithick]
\input figure/alo-comp/alo-cmd
  \endscope

  \scope[color=cat2, semithick]
\input figure/alo-comp/lo-cmd
  \endscope

  \draw (\yaxis, 0.58) node[left]{\sevenpoint$0.53$} -- +(\xtick, 0);
  \draw (\yaxis, 1.1) node[left]{\sevenpoint$1$} -- +(\xtick, 0);

  \foreach \x in {0, 1}
    \draw (\x, \xaxis) node[below]{\sevenpoint$\x$} -- +(0, \ytick);

  \draw[dotted, thick] (0.12, \xaxis) node[below, color=black]{\sevenpoint 0.12 0.13} -- (0.12, 0.58);
  \draw[dotted, thick] (0.13, \xaxis) -- (0.13, 0.58);

\draw (.65, .77) node[color=cat1]{ALO};
\draw (.55, 0.9) node[color=cat2]{LO};
\draw (0.52, \xaxis-.1) node{\sevenpoint$t / \sum_{j=1}^p |\hat{\beta}_j^{\rm OLS}|$};

\endtikzpicture

\subend


==> figure/diabetes-1/plot.tex <==
\input mac/m

\definecolor{cat1}{RGB}{0, 114, 190}
\definecolor{cat2}{RGB}{218, 83, 25}

\tikzpicture[xscale=12, yscale=1.2]
  % \draw[very thin,color=gray, xstep=.08, ystep=.2] (-0.01,-2.52) grid (1.01,1.01);

  % \draw[->] (-0.02,0) -- (1.02,0) node[right] {$x$};
  \def\yaxis{-0.025}
  % \def\xaxis{-2.65}
  \def\xaxis{-3.0}
  \def\ticksize{.1cm}
  \def\xtick{\ticksize/12}
  \def\ytick{\ticksize/1.2}

  \draw (\yaxis,-2.5) -- (\yaxis, 1.0);
  \draw (0, \xaxis) -- (1, \xaxis);

  \draw[very thin, color=gray] (\yaxis, 0) node[left, color=black]{\sevenpoint$0$} -- (1, 0);

  \draw[dotted, thick] (0.548, \xaxis) node[below, color=black]{\sevenpoint$0.55$} -- (0.548, 0.5)
          -- (\yaxis, 0.5) node[left, color=black]{\sevenpoint$0.5$};

  \scope[color=cat1, semithick]
  \input figure/diabetes-1/lo-cmd
  \endscope

  \scope[color=cat2, semithick]
  \input figure/diabetes-1/lo-d-cmd
  \endscope

  \foreach \y in {-2.5, 1}
    \draw (\yaxis, \y) node[left]{\sevenpoint$\y$} -- +(\xtick, 0);

  \foreach \x in {0, 1}
    \draw (\x, \xaxis) node[below]{\sevenpoint$\x$} -- +(0, \ytick);

% Figure Labels
\draw (.6, .7) node[color=cat1]{LO};
\draw (.66, -.3) node[color=cat2]{LO Derivative};
\draw (0.52, \xaxis-.7) node{\sevenpoint$t / \sum_{j=1}^p |\hat{\beta}_j^{\rm OLS}|$};


% Activations
\draw (0, -2.7) node[color=gray]{\sevenpoint+BMI};
\draw (0.017, -1.4) node[color=gray]{\sevenpoint+LTG};
\draw (0.19, -.65) node[color=gray]{\sevenpoint+BP};
\draw (0.2569, -0.4) node[color=gray]{\sevenpoint+HDL};
\draw (0.3614, 0.35) node[color=gray]{\sevenpoint+Sex};
\draw (0.4164, -0.4) node[color=gray]{\sevenpoint+GLU};
\draw (0.444, 0.2) node[color=gray]{\sevenpoint+TC};
\draw (0.525, 0.3) node[color=gray]{\sevenpoint+TCH};
\draw (0.62, 0.36) node[color=gray]{\sevenpoint+LDL};
\draw (0.65, 0.1) node[color=gray]{\sevenpoint+Age};
\draw (0.8099, -0.2) node[color=gray]{\sevenpoint-HDL};
\draw (0.827, 0.2) node[color=gray]{\sevenpoint+HDL};

\endtikzpicture

\subend


==> figure/diabetes-err/plot.tex <==
\input mac/m

\hsize=6in
\definecolor{cat1}{RGB}{0, 114, 190}
\definecolor{cat2}{RGB}{218, 83, 25}

\definecolor{c1}{RGB}{63, 144, 218}
\definecolor{c2}{RGB}{255, 169, 14}
\definecolor{c3}{RGB}{189, 31, 1}
\definecolor{c4}{RGB}{148, 164, 162}
\definecolor{c5}{RGB}{131, 45, 182}
\definecolor{c6}{RGB}{169, 107, 89}
\definecolor{c7}{RGB}{231, 99, 0}
\definecolor{c8}{RGB}{185, 172, 112}
\definecolor{c9}{RGB}{113, 117, 129}
\definecolor{c10}{RGB}{146, 218, 221}

\tikzpicture
  \def\yaxis{-0.025}
  \def\xaxis{-180}
  \def\ticksize{.1cm}
  \def\xscale{12}
  \def\yscale{0.01}
  \def\ymin{-158}
  \def\ymax{194}

  \scope[xscale=\xscale, yscale=\yscale]
  \def\xtick{\ticksize/\xscale}
  \def\ytick{\ticksize/\yscale}
  
  \scope[very thin, opacity=0.25]
  \input figure/diabetes-err/cmd
  \endscope


% min/max: -158.23301268992498 194.30612244897958
  % Y axis
  \draw (\yaxis, 0) node[left]{\sevenpoint0} -- (1, 0);
  \draw (\yaxis,\ymin) -- (\yaxis, \ymax);
  \foreach \y in {\ymin, \ymax}
    \draw (\yaxis, \y) node[left]{\sevenpoint$\y$} -- +(\xtick, 0);

  % X axis
  \draw (0, \xaxis) -- (1, \xaxis);
  \draw[dotted] (0.55, \xaxis) node[below]{\sevenpoint$0.55$} -- (0.55, \ymax-35);
  \foreach \x in {0, 1}
    \draw (\x, \xaxis) node[below]{\sevenpoint$\x$} -- +(0, \ytick);

  % Labels
  \draw (0.55, \xaxis-75) node{\sevenpoint$t / \sum_{j=1}^p |\hat{\beta}_j^{\rm OLS}|$};

  \endscope
\endtikzpicture

\subend



==> figure/riboflavin/lo-cmd.tex <==
\draw (0.0, 1.0) .. controls (0.003, 0.961) and (0.006, 0.927) .. (0.009, 0.899)
	-- (0.009, 0.892) .. controls (0.01, 0.89) and (0.01, 0.889) .. (0.01, 0.888)
	-- (0.01, 0.886) .. controls (0.01, 0.885) and (0.01, 0.884) .. (0.011, 0.883)
	-- (0.011, 0.88) .. controls (0.012, 0.88) and (0.012, 0.88) .. (0.012, 0.88)
	-- (0.012, 0.881) .. controls (0.012, 0.881) and (0.012, 0.881) .. (0.013, 0.881)
	-- (0.013, 0.881) .. controls (0.013, 0.881) and (0.014, 0.881) .. (0.014, 0.881)
	-- (0.014, 0.88) .. controls (0.015, 0.88) and (0.015, 0.879) .. (0.015, 0.879)
	-- (0.015, 0.877) .. controls (0.015, 0.877) and (0.016, 0.876) .. (0.016, 0.876)
	-- (0.016, 0.873) .. controls (0.016, 0.873) and (0.017, 0.873) .. (0.017, 0.873)
	-- (0.017, 0.87) .. controls (0.017, 0.87) and (0.017, 0.87) .. (0.018, 0.87)
	-- (0.018, 0.866) .. controls (0.018, 0.865) and (0.018, 0.865) .. (0.019, 0.865)
	-- (0.019, 0.861) .. controls (0.019, 0.86) and (0.019, 0.86) .. (0.02, 0.859)
	-- (0.02, 0.854) .. controls (0.02, 0.854) and (0.021, 0.853) .. (0.021, 0.853)
	-- (0.021, 0.85) .. controls (0.021, 0.848) and (0.022, 0.847) .. (0.022, 0.846)
	-- (0.022, 0.842) .. controls (0.023, 0.84) and (0.023, 0.837) .. (0.024, 0.835)
	-- (0.024, 0.835) .. controls (0.024, 0.832) and (0.025, 0.828) .. (0.025, 0.825)
	-- (0.025, 0.824) .. controls (0.026, 0.819) and (0.027, 0.815) .. (0.027, 0.81)
	-- (0.027, 0.809) .. controls (0.028, 0.807) and (0.028, 0.804) .. (0.029, 0.801)
	-- (0.029, 0.797) .. controls (0.03, 0.795) and (0.03, 0.794) .. (0.03, 0.792)
	-- (0.03, 0.792) .. controls (0.03, 0.791) and (0.03, 0.789) .. (0.031, 0.787)
	-- (0.031, 0.787) .. controls (0.031, 0.785) and (0.031, 0.782) .. (0.032, 0.779)
	-- (0.032, 0.778) .. controls (0.033, 0.773) and (0.033, 0.769) .. (0.034, 0.765)
	-- (0.034, 0.762) .. controls (0.035, 0.756) and (0.036, 0.751) .. (0.037, 0.746)
	-- (0.037, 0.744) .. controls (0.037, 0.743) and (0.037, 0.743) .. (0.038, 0.742)
	-- (0.038, 0.741) .. controls (0.038, 0.739) and (0.038, 0.737) .. (0.039, 0.734)
	-- (0.039, 0.731) .. controls (0.04, 0.728) and (0.041, 0.724) .. (0.041, 0.721)
	-- (0.041, 0.72) .. controls (0.042, 0.718) and (0.042, 0.717) .. (0.042, 0.715)
	-- (0.042, 0.715) .. controls (0.042, 0.714) and (0.043, 0.713) .. (0.043, 0.712)
	-- (0.043, 0.71) .. controls (0.043, 0.71) and (0.043, 0.709) .. (0.044, 0.708)
	-- (0.044, 0.703) .. controls (0.045, 0.703) and (0.045, 0.703) .. (0.045, 0.703)
	-- (0.045, 0.698) .. controls (0.045, 0.698) and (0.046, 0.698) .. (0.046, 0.698)
	-- (0.046, 0.694) .. controls (0.047, 0.693) and (0.047, 0.693) .. (0.047, 0.692)
	-- (0.047, 0.689) .. controls (0.047, 0.689) and (0.048, 0.689) .. (0.048, 0.688)
	-- (0.048, 0.685) .. controls (0.048, 0.684) and (0.049, 0.684) .. (0.049, 0.684)
	-- (0.049, 0.681) .. controls (0.049, 0.681) and (0.049, 0.68) .. (0.05, 0.679)
	-- (0.05, 0.676) .. controls (0.05, 0.676) and (0.051, 0.675) .. (0.051, 0.675)
	-- (0.051, 0.671) .. controls (0.051, 0.671) and (0.051, 0.671) .. (0.052, 0.671)
	-- (0.052, 0.667) .. controls (0.053, 0.667) and (0.053, 0.666) .. (0.053, 0.666)
	-- (0.053, 0.663) .. controls (0.054, 0.662) and (0.054, 0.662) .. (0.054, 0.661)
	-- (0.054, 0.659) .. controls (0.054, 0.658) and (0.055, 0.658) .. (0.055, 0.658)
	-- (0.055, 0.654) .. controls (0.056, 0.654) and (0.056, 0.654) .. (0.056, 0.654)
	-- (0.056, 0.651) .. controls (0.056, 0.65) and (0.056, 0.65) .. (0.057, 0.65)
	-- (0.057, 0.647) .. controls (0.057, 0.646) and (0.057, 0.646) .. (0.058, 0.646)
	-- (0.058, 0.643) .. controls (0.058, 0.642) and (0.059, 0.642) .. (0.059, 0.642)
	-- (0.059, 0.638) .. controls (0.06, 0.638) and (0.06, 0.638) .. (0.06, 0.638)
	-- (0.06, 0.635) .. controls (0.06, 0.635) and (0.06, 0.634) .. (0.061, 0.634)
	-- (0.061, 0.63) .. controls (0.062, 0.63) and (0.062, 0.63) .. (0.062, 0.63)
	-- (0.062, 0.626) .. controls (0.062, 0.626) and (0.063, 0.626) .. (0.063, 0.626)
	-- (0.063, 0.622) .. controls (0.063, 0.622) and (0.064, 0.621) .. (0.064, 0.621)
	-- (0.064, 0.617) .. controls (0.064, 0.617) and (0.064, 0.617) .. (0.065, 0.617)
	-- (0.065, 0.613) .. controls (0.066, 0.613) and (0.066, 0.613) .. (0.066, 0.613)
	-- (0.066, 0.609) .. controls (0.066, 0.609) and (0.067, 0.609) .. (0.067, 0.608)
	-- (0.067, 0.605) .. controls (0.067, 0.605) and (0.067, 0.604) .. (0.068, 0.604)
	-- (0.068, 0.601) .. controls (0.068, 0.6) and (0.068, 0.6) .. (0.069, 0.6)
	-- (0.069, 0.596) .. controls (0.07, 0.595) and (0.07, 0.595) .. (0.07, 0.594)
	-- (0.07, 0.591) .. controls (0.071, 0.591) and (0.071, 0.591) .. (0.071, 0.59)
	-- (0.071, 0.587) .. controls (0.071, 0.586) and (0.072, 0.586) .. (0.072, 0.585)
	-- (0.072, 0.582) .. controls (0.073, 0.581) and (0.073, 0.581) .. (0.073, 0.581)
	-- (0.073, 0.578) .. controls (0.073, 0.578) and (0.073, 0.577) .. (0.074, 0.576)
	-- (0.074, 0.573) .. controls (0.074, 0.572) and (0.075, 0.572) .. (0.075, 0.572)
	-- (0.075, 0.569) .. controls (0.075, 0.569) and (0.075, 0.568) .. (0.076, 0.567)
	-- (0.076, 0.564) .. controls (0.076, 0.564) and (0.077, 0.563) .. (0.077, 0.563)
	-- (0.077, 0.56) .. controls (0.077, 0.559) and (0.077, 0.559) .. (0.078, 0.559)
	-- (0.078, 0.555) .. controls (0.079, 0.554) and (0.079, 0.554) .. (0.079, 0.554)
	-- (0.079, 0.55) .. controls (0.079, 0.55) and (0.08, 0.55) .. (0.08, 0.55)
	-- (0.08, 0.546) .. controls (0.081, 0.545) and (0.081, 0.545) .. (0.081, 0.545)
	-- (0.081, 0.542) .. controls (0.081, 0.542) and (0.081, 0.541) .. (0.082, 0.541)
	-- (0.082, 0.537) .. controls (0.083, 0.537) and (0.083, 0.536) .. (0.083, 0.536)
	-- (0.083, 0.532) .. controls (0.084, 0.532) and (0.084, 0.532) .. (0.084, 0.532)
	-- (0.084, 0.529) .. controls (0.084, 0.528) and (0.085, 0.528) .. (0.085, 0.527)
	-- (0.085, 0.524) .. controls (0.086, 0.523) and (0.086, 0.522) .. (0.086, 0.52)
	-- (0.086, 0.519) .. controls (0.086, 0.519) and (0.086, 0.519) .. (0.087, 0.518)
	-- (0.087, 0.515) .. controls (0.088, 0.514) and (0.088, 0.513) .. (0.088, 0.512)
	-- (0.088, 0.511) .. controls (0.088, 0.511) and (0.088, 0.51) .. (0.089, 0.51)
	-- (0.089, 0.506) .. controls (0.089, 0.506) and (0.09, 0.505) .. (0.09, 0.505)
	-- (0.09, 0.501) .. controls (0.09, 0.501) and (0.091, 0.501) .. (0.091, 0.5)
	-- (0.091, 0.496) .. controls (0.092, 0.496) and (0.092, 0.495) .. (0.092, 0.495)
	-- (0.092, 0.492) .. controls (0.093, 0.492) and (0.093, 0.491) .. (0.093, 0.491)
	-- (0.093, 0.487) .. controls (0.094, 0.487) and (0.094, 0.487) .. (0.094, 0.486)
	-- (0.094, 0.483) .. controls (0.094, 0.483) and (0.095, 0.483) .. (0.095, 0.483)
	-- (0.095, 0.479) .. controls (0.096, 0.479) and (0.096, 0.479) .. (0.096, 0.478)
	-- (0.096, 0.475) .. controls (0.096, 0.475) and (0.097, 0.475) .. (0.097, 0.474)
	-- (0.097, 0.471) .. controls (0.098, 0.471) and (0.098, 0.47) .. (0.098, 0.47)
	-- (0.098, 0.467) .. controls (0.098, 0.467) and (0.099, 0.467) .. (0.099, 0.467)
	-- (0.099, 0.463) .. controls (0.1, 0.463) and (0.1, 0.463) .. (0.1, 0.463)
	-- (0.1, 0.46) .. controls (0.1, 0.46) and (0.1, 0.46) .. (0.101, 0.46)
	-- (0.101, 0.456) .. controls (0.102, 0.456) and (0.102, 0.456) .. (0.102, 0.456)
	-- (0.102, 0.453) .. controls (0.103, 0.453) and (0.103, 0.453) .. (0.103, 0.452)
	-- (0.103, 0.45) .. controls (0.103, 0.449) and (0.104, 0.449) .. (0.104, 0.449)
	-- (0.104, 0.446) .. controls (0.104, 0.446) and (0.105, 0.446) .. (0.105, 0.445)
	-- (0.105, 0.443) .. controls (0.105, 0.442) and (0.106, 0.442) .. (0.106, 0.441)
	-- (0.106, 0.439) .. controls (0.106, 0.439) and (0.107, 0.438) .. (0.107, 0.438)
	-- (0.107, 0.436) .. controls (0.107, 0.435) and (0.108, 0.435) .. (0.108, 0.435)
	-- (0.108, 0.433) .. controls (0.108, 0.432) and (0.109, 0.432) .. (0.109, 0.431)
	-- (0.109, 0.429) .. controls (0.109, 0.429) and (0.11, 0.429) .. (0.11, 0.429)
	-- (0.11, 0.429) .. controls (0.11, 0.428) and (0.11, 0.427) .. (0.111, 0.426)
	-- (0.111, 0.424) .. controls (0.112, 0.423) and (0.112, 0.422) .. (0.112, 0.422)
	-- (0.112, 0.421) .. controls (0.112, 0.42) and (0.113, 0.42) .. (0.113, 0.42)
	-- (0.113, 0.418) .. controls (0.113, 0.417) and (0.114, 0.417) .. (0.114, 0.417)
	-- (0.114, 0.415) .. controls (0.114, 0.415) and (0.114, 0.415) .. (0.115, 0.414)
	-- (0.115, 0.412) .. controls (0.116, 0.412) and (0.116, 0.412) .. (0.116, 0.411)
	-- (0.116, 0.409) .. controls (0.117, 0.409) and (0.117, 0.408) .. (0.117, 0.408)
	-- (0.117, 0.407) .. controls (0.117, 0.407) and (0.118, 0.406) .. (0.118, 0.406)
	-- (0.118, 0.404) .. controls (0.118, 0.404) and (0.118, 0.404) .. (0.119, 0.404)
	-- (0.119, 0.401) .. controls (0.12, 0.401) and (0.12, 0.401) .. (0.12, 0.401)
	-- (0.12, 0.399) .. controls (0.12, 0.399) and (0.121, 0.399) .. (0.121, 0.399)
	-- (0.121, 0.396) .. controls (0.121, 0.396) and (0.121, 0.396) .. (0.122, 0.396)
	-- (0.122, 0.394) .. controls (0.122, 0.394) and (0.123, 0.393) .. (0.123, 0.393)
	-- (0.123, 0.392) .. controls (0.123, 0.391) and (0.123, 0.391) .. (0.124, 0.391)
	-- (0.124, 0.389) .. controls (0.124, 0.389) and (0.125, 0.388) .. (0.125, 0.388)
	-- (0.125, 0.386) .. controls (0.126, 0.386) and (0.126, 0.385) .. (0.126, 0.384)
	-- (0.126, 0.384) .. controls (0.126, 0.383) and (0.127, 0.383) .. (0.127, 0.383)
	-- (0.127, 0.381) .. controls (0.127, 0.381) and (0.128, 0.38) .. (0.128, 0.38)
	-- (0.128, 0.378) .. controls (0.129, 0.378) and (0.129, 0.378) .. (0.129, 0.377)
	-- (0.129, 0.376) .. controls (0.129, 0.375) and (0.13, 0.375) .. (0.13, 0.374)
	-- (0.13, 0.372) .. controls (0.13, 0.372) and (0.131, 0.372) .. (0.131, 0.372)
	-- (0.131, 0.369) .. controls (0.132, 0.369) and (0.132, 0.369) .. (0.132, 0.368)
	-- (0.132, 0.368) .. controls (0.132, 0.367) and (0.133, 0.366) .. (0.133, 0.365)
	-- (0.133, 0.364) .. controls (0.133, 0.364) and (0.133, 0.364) .. (0.134, 0.364)
	-- (0.134, 0.361) .. controls (0.134, 0.361) and (0.135, 0.361) .. (0.135, 0.361)
	-- (0.135, 0.359) .. controls (0.135, 0.359) and (0.135, 0.359) .. (0.136, 0.359)
	-- (0.136, 0.358) .. controls (0.136, 0.357) and (0.136, 0.356) .. (0.137, 0.356)
	-- (0.137, 0.355) .. controls (0.137, 0.354) and (0.138, 0.354) .. (0.138, 0.353)
	-- (0.138, 0.352) .. controls (0.138, 0.352) and (0.139, 0.352) .. (0.139, 0.351)
	-- (0.139, 0.35) .. controls (0.14, 0.349) and (0.14, 0.349) .. (0.14, 0.348)
	-- (0.14, 0.348) .. controls (0.14, 0.347) and (0.141, 0.347) .. (0.141, 0.347)
	-- (0.141, 0.345) .. controls (0.142, 0.344) and (0.142, 0.344) .. (0.142, 0.343)
	-- (0.142, 0.343) .. controls (0.142, 0.343) and (0.143, 0.342) .. (0.143, 0.341)
	-- (0.143, 0.341) .. controls (0.143, 0.341) and (0.143, 0.34) .. (0.144, 0.34)
	-- (0.144, 0.338) .. controls (0.145, 0.337) and (0.145, 0.337) .. (0.145, 0.337)
	-- (0.145, 0.336) .. controls (0.146, 0.335) and (0.146, 0.334) .. (0.146, 0.334)
	-- (0.146, 0.333) .. controls (0.147, 0.333) and (0.147, 0.332) .. (0.147, 0.331)
	-- (0.147, 0.331) .. controls (0.147, 0.331) and (0.148, 0.331) .. (0.148, 0.331)
	-- (0.148, 0.329) .. controls (0.149, 0.329) and (0.149, 0.329) .. (0.149, 0.329)
	-- (0.149, 0.327) .. controls (0.149, 0.327) and (0.149, 0.327) .. (0.15, 0.327)
	-- (0.15, 0.325) .. controls (0.15, 0.325) and (0.15, 0.325) .. (0.151, 0.325)
	-- (0.151, 0.323) .. controls (0.151, 0.323) and (0.152, 0.323) .. (0.152, 0.323)
	-- (0.152, 0.322) .. controls (0.152, 0.322) and (0.152, 0.322) .. (0.153, 0.321)
	-- (0.153, 0.32) .. controls (0.153, 0.32) and (0.153, 0.32) .. (0.154, 0.32)
	-- (0.154, 0.318) .. controls (0.155, 0.318) and (0.155, 0.318) .. (0.155, 0.318)
	-- (0.155, 0.317) .. controls (0.156, 0.317) and (0.156, 0.317) .. (0.156, 0.317)
	-- (0.156, 0.316) .. controls (0.156, 0.315) and (0.157, 0.315) .. (0.157, 0.315)
	-- (0.157, 0.314) .. controls (0.157, 0.314) and (0.158, 0.314) .. (0.158, 0.313)
	-- (0.158, 0.312) .. controls (0.159, 0.312) and (0.159, 0.312) .. (0.159, 0.312)
	-- (0.159, 0.311) .. controls (0.16, 0.311) and (0.16, 0.311) .. (0.16, 0.311)
	-- (0.16, 0.31) .. controls (0.16, 0.31) and (0.16, 0.31) .. (0.161, 0.31)
	-- (0.161, 0.309) .. controls (0.161, 0.309) and (0.162, 0.309) .. (0.162, 0.309)
	-- (0.162, 0.308) .. controls (0.162, 0.308) and (0.163, 0.308) .. (0.163, 0.308)
	-- (0.163, 0.307) .. controls (0.163, 0.307) and (0.164, 0.307) .. (0.164, 0.307)
	-- (0.164, 0.306) .. controls (0.164, 0.306) and (0.165, 0.306) .. (0.165, 0.306)
	-- (0.165, 0.305) .. controls (0.165, 0.305) and (0.166, 0.305) .. (0.166, 0.305)
	-- (0.166, 0.304) .. controls (0.166, 0.304) and (0.166, 0.304) .. (0.167, 0.304)
	-- (0.167, 0.303) .. controls (0.167, 0.303) and (0.168, 0.303) .. (0.168, 0.303)
	-- (0.168, 0.302) .. controls (0.168, 0.302) and (0.168, 0.302) .. (0.169, 0.301)
	-- (0.169, 0.3) .. controls (0.17, 0.3) and (0.17, 0.3) .. (0.17, 0.3)
	-- (0.17, 0.299) .. controls (0.171, 0.299) and (0.171, 0.299) .. (0.171, 0.299)
	-- (0.171, 0.298) .. controls (0.171, 0.298) and (0.171, 0.298) .. (0.172, 0.297)
	-- (0.172, 0.296) .. controls (0.173, 0.296) and (0.173, 0.296) .. (0.173, 0.296)
	-- (0.173, 0.295) .. controls (0.173, 0.295) and (0.174, 0.295) .. (0.174, 0.294)
	-- (0.174, 0.293) .. controls (0.174, 0.293) and (0.175, 0.293) .. (0.175, 0.293)
	-- (0.175, 0.292) .. controls (0.175, 0.292) and (0.176, 0.291) .. (0.176, 0.291)
	-- (0.176, 0.29) .. controls (0.177, 0.29) and (0.177, 0.29) .. (0.177, 0.29)
	-- (0.177, 0.289) .. controls (0.177, 0.288) and (0.177, 0.288) .. (0.178, 0.288)
	-- (0.178, 0.287) .. controls (0.179, 0.287) and (0.179, 0.287) .. (0.179, 0.287)
	-- (0.179, 0.285) .. controls (0.179, 0.285) and (0.179, 0.285) .. (0.18, 0.285)
	-- (0.18, 0.284) .. controls (0.18, 0.284) and (0.181, 0.284) .. (0.181, 0.283)
	-- (0.181, 0.282) .. controls (0.181, 0.282) and (0.181, 0.282) .. (0.182, 0.282)
	-- (0.182, 0.281) .. controls (0.183, 0.281) and (0.183, 0.281) .. (0.183, 0.281)
	-- (0.183, 0.279) .. controls (0.183, 0.279) and (0.184, 0.279) .. (0.184, 0.279)
	-- (0.184, 0.278) .. controls (0.184, 0.278) and (0.185, 0.278) .. (0.185, 0.277)
	-- (0.185, 0.276) .. controls (0.185, 0.276) and (0.186, 0.276) .. (0.186, 0.276)
	-- (0.186, 0.275) .. controls (0.186, 0.275) and (0.187, 0.275) .. (0.187, 0.275)
	-- (0.187, 0.273) .. controls (0.187, 0.273) and (0.188, 0.273) .. (0.188, 0.273)
	-- (0.188, 0.272) .. controls (0.188, 0.272) and (0.188, 0.272) .. (0.189, 0.271)
	-- (0.189, 0.27) .. controls (0.189, 0.27) and (0.19, 0.27) .. (0.19, 0.27)
	-- (0.19, 0.268) .. controls (0.19, 0.268) and (0.19, 0.268) .. (0.191, 0.268)
	-- (0.191, 0.267) .. controls (0.191, 0.267) and (0.191, 0.267) .. (0.192, 0.267)
	-- (0.192, 0.265) .. controls (0.193, 0.265) and (0.193, 0.265) .. (0.193, 0.264)
	-- (0.193, 0.264) .. controls (0.193, 0.263) and (0.194, 0.263) .. (0.194, 0.263)
	-- (0.194, 0.262) .. controls (0.194, 0.262) and (0.194, 0.262) .. (0.195, 0.262)
	-- (0.195, 0.26) .. controls (0.195, 0.26) and (0.196, 0.26) .. (0.196, 0.26)
	-- (0.196, 0.26) .. controls (0.196, 0.259) and (0.196, 0.259) .. (0.197, 0.259)
	-- (0.197, 0.258) .. controls (0.198, 0.258) and (0.198, 0.258) .. (0.198, 0.258)
	-- (0.198, 0.257) .. controls (0.198, 0.257) and (0.199, 0.257) .. (0.199, 0.256)
	-- (0.199, 0.256) .. controls (0.199, 0.256) and (0.2, 0.256) .. (0.2, 0.255)
	-- (0.2, 0.255) .. controls (0.201, 0.255) and (0.201, 0.255) .. (0.201, 0.255)
	-- (0.201, 0.254) .. controls (0.202, 0.254) and (0.202, 0.254) .. (0.202, 0.254)
	-- (0.202, 0.253) .. controls (0.203, 0.253) and (0.203, 0.253) .. (0.203, 0.253)
	-- (0.203, 0.252) .. controls (0.204, 0.252) and (0.204, 0.252) .. (0.204, 0.252)
	-- (0.204, 0.252) .. controls (0.204, 0.252) and (0.204, 0.252) .. (0.205, 0.252)
	-- (0.205, 0.251) .. controls (0.205, 0.251) and (0.206, 0.251) .. (0.206, 0.251)
	-- (0.206, 0.251) .. controls (0.206, 0.25) and (0.206, 0.25) .. (0.207, 0.25)
	-- (0.207, 0.25) .. controls (0.207, 0.25) and (0.208, 0.25) .. (0.208, 0.25)
	-- (0.208, 0.249) .. controls (0.208, 0.249) and (0.208, 0.249) .. (0.209, 0.249)
	-- (0.209, 0.248) .. controls (0.209, 0.248) and (0.209, 0.248) .. (0.21, 0.248)
	-- (0.21, 0.247) .. controls (0.21, 0.247) and (0.211, 0.247) .. (0.211, 0.247)
	-- (0.211, 0.246) .. controls (0.211, 0.246) and (0.212, 0.246) .. (0.212, 0.246)
	-- (0.212, 0.246) .. controls (0.212, 0.246) and (0.213, 0.246) .. (0.213, 0.246)
	-- (0.213, 0.245) .. controls (0.213, 0.245) and (0.214, 0.245) .. (0.214, 0.245)
	-- (0.214, 0.244) .. controls (0.215, 0.244) and (0.215, 0.244) .. (0.215, 0.244)
	-- (0.215, 0.244) .. controls (0.215, 0.244) and (0.215, 0.244) .. (0.216, 0.243)
	-- (0.216, 0.243) .. controls (0.216, 0.243) and (0.217, 0.243) .. (0.217, 0.243)
	-- (0.217, 0.242) .. controls (0.217, 0.242) and (0.217, 0.242) .. (0.218, 0.242)
	-- (0.218, 0.242) .. controls (0.218, 0.242) and (0.218, 0.242) .. (0.219, 0.242)
	-- (0.219, 0.242) .. controls (0.22, 0.242) and (0.22, 0.241) .. (0.22, 0.241)
	-- (0.22, 0.241) .. controls (0.221, 0.241) and (0.221, 0.241) .. (0.221, 0.241)
	-- (0.221, 0.241) .. controls (0.222, 0.241) and (0.222, 0.241) .. (0.222, 0.241)
	-- (0.222, 0.241) .. controls (0.222, 0.241) and (0.222, 0.241) .. (0.223, 0.241)
	-- (0.223, 0.241) .. controls (0.224, 0.241) and (0.224, 0.241) .. (0.224, 0.241)
	-- (0.224, 0.24) .. controls (0.225, 0.24) and (0.225, 0.24) .. (0.225, 0.24)
	-- (0.225, 0.24) .. controls (0.225, 0.24) and (0.226, 0.24) .. (0.226, 0.24)
	-- (0.226, 0.24) .. controls (0.226, 0.24) and (0.226, 0.24) .. (0.227, 0.24)
	-- (0.227, 0.24) .. controls (0.227, 0.24) and (0.227, 0.24) .. (0.228, 0.24)
	-- (0.228, 0.24) .. controls (0.228, 0.24) and (0.228, 0.24) .. (0.229, 0.24)
	-- (0.229, 0.24) .. controls (0.229, 0.24) and (0.229, 0.24) .. (0.23, 0.24)
	-- (0.23, 0.24) .. controls (0.231, 0.24) and (0.231, 0.24) .. (0.231, 0.24)
	-- (0.231, 0.241) .. controls (0.231, 0.241) and (0.232, 0.241) .. (0.232, 0.241)
	-- (0.232, 0.241) .. controls (0.233, 0.241) and (0.233, 0.241) .. (0.233, 0.241)
	-- (0.233, 0.241) .. controls (0.234, 0.241) and (0.234, 0.241) .. (0.234, 0.241)
	-- (0.234, 0.241) .. controls (0.235, 0.241) and (0.235, 0.241) .. (0.235, 0.241)
	-- (0.235, 0.241) .. controls (0.236, 0.241) and (0.236, 0.241) .. (0.236, 0.241)
	-- (0.236, 0.241) .. controls (0.236, 0.241) and (0.237, 0.241) .. (0.237, 0.241)
	-- (0.237, 0.242) .. controls (0.238, 0.242) and (0.238, 0.242) .. (0.238, 0.242)
	-- (0.238, 0.242) .. controls (0.238, 0.242) and (0.238, 0.242) .. (0.239, 0.242)
	-- (0.239, 0.242) .. controls (0.24, 0.242) and (0.24, 0.242) .. (0.24, 0.242)
	-- (0.24, 0.242) .. controls (0.24, 0.242) and (0.24, 0.242) .. (0.241, 0.242)
	-- (0.241, 0.242) .. controls (0.241, 0.242) and (0.242, 0.242) .. (0.242, 0.242)
	-- (0.242, 0.242) .. controls (0.243, 0.242) and (0.243, 0.242) .. (0.243, 0.242)
	-- (0.243, 0.242) .. controls (0.244, 0.242) and (0.244, 0.242) .. (0.244, 0.242)
	-- (0.244, 0.242) .. controls (0.244, 0.242) and (0.244, 0.242) .. (0.245, 0.242)
	-- (0.245, 0.242) .. controls (0.245, 0.242) and (0.245, 0.242) .. (0.246, 0.242)
	-- (0.246, 0.242) .. controls (0.247, 0.242) and (0.247, 0.242) .. (0.247, 0.242)
	-- (0.247, 0.242) .. controls (0.247, 0.242) and (0.248, 0.242) .. (0.248, 0.242)
	-- (0.248, 0.242) .. controls (0.248, 0.242) and (0.249, 0.242) .. (0.249, 0.242)
	-- (0.249, 0.242) .. controls (0.249, 0.242) and (0.25, 0.242) .. (0.25, 0.242)
	-- (0.25, 0.242) .. controls (0.25, 0.242) and (0.251, 0.242) .. (0.251, 0.242)
	-- (0.251, 0.242) .. controls (0.252, 0.242) and (0.252, 0.242) .. (0.252, 0.242)
	-- (0.252, 0.243) .. controls (0.252, 0.243) and (0.253, 0.243) .. (0.253, 0.243)
	-- (0.253, 0.243) .. controls (0.254, 0.243) and (0.254, 0.243) .. (0.254, 0.243)
	-- (0.254, 0.243) .. controls (0.255, 0.243) and (0.255, 0.243) .. (0.255, 0.243)
	-- (0.255, 0.243) .. controls (0.256, 0.243) and (0.256, 0.243) .. (0.256, 0.243)
	-- (0.256, 0.243) .. controls (0.256, 0.243) and (0.256, 0.243) .. (0.257, 0.243)
	-- (0.257, 0.243) .. controls (0.257, 0.243) and (0.258, 0.243) .. (0.258, 0.243)
	-- (0.258, 0.243) .. controls (0.258, 0.243) and (0.258, 0.243) .. (0.259, 0.243)
	-- (0.259, 0.243) .. controls (0.259, 0.243) and (0.26, 0.243) .. (0.26, 0.243)
	-- (0.26, 0.243) .. controls (0.26, 0.243) and (0.26, 0.243) .. (0.261, 0.243)
	-- (0.261, 0.244) .. controls (0.261, 0.244) and (0.262, 0.244) .. (0.262, 0.244)
	-- (0.262, 0.244) .. controls (0.263, 0.244) and (0.263, 0.244) .. (0.263, 0.244)
	-- (0.263, 0.244) .. controls (0.263, 0.244) and (0.264, 0.244) .. (0.264, 0.244)
	-- (0.264, 0.244) .. controls (0.265, 0.244) and (0.265, 0.244) .. (0.265, 0.244)
	-- (0.265, 0.244) .. controls (0.266, 0.244) and (0.266, 0.244) .. (0.266, 0.244)
	-- (0.266, 0.244) .. controls (0.266, 0.244) and (0.267, 0.244) .. (0.267, 0.244)
	-- (0.267, 0.244) .. controls (0.268, 0.244) and (0.268, 0.244) .. (0.268, 0.244)
	-- (0.268, 0.245) .. controls (0.268, 0.245) and (0.268, 0.245) .. (0.269, 0.245)
	-- (0.269, 0.245) .. controls (0.27, 0.245) and (0.27, 0.245) .. (0.27, 0.245)
	-- (0.27, 0.245) .. controls (0.27, 0.245) and (0.27, 0.245) .. (0.271, 0.245)
	-- (0.271, 0.245) .. controls (0.272, 0.245) and (0.272, 0.245) .. (0.272, 0.245)
	-- (0.272, 0.246) .. controls (0.272, 0.246) and (0.273, 0.246) .. (0.273, 0.246)
	-- (0.273, 0.246) .. controls (0.273, 0.246) and (0.273, 0.246) .. (0.274, 0.246)
	-- (0.274, 0.246) .. controls (0.274, 0.246) and (0.275, 0.246) .. (0.275, 0.246)
	-- (0.275, 0.247) .. controls (0.275, 0.247) and (0.276, 0.247) .. (0.276, 0.247)
	-- (0.276, 0.247) .. controls (0.276, 0.247) and (0.276, 0.247) .. (0.277, 0.247)
	-- (0.277, 0.247) .. controls (0.278, 0.247) and (0.278, 0.248) .. (0.278, 0.248)
	-- (0.278, 0.248) .. controls (0.278, 0.248) and (0.279, 0.248) .. (0.279, 0.248)
	-- (0.279, 0.248) .. controls (0.279, 0.248) and (0.28, 0.248) .. (0.28, 0.248)
	-- (0.28, 0.249) .. controls (0.281, 0.249) and (0.281, 0.249) .. (0.281, 0.249)
	-- (0.281, 0.249) .. controls (0.281, 0.249) and (0.282, 0.249) .. (0.282, 0.249)
	-- (0.282, 0.25) .. controls (0.282, 0.25) and (0.282, 0.25) .. (0.283, 0.25)
	-- (0.283, 0.25) .. controls (0.283, 0.25) and (0.283, 0.25) .. (0.284, 0.25)
	-- (0.284, 0.251) .. controls (0.284, 0.251) and (0.285, 0.251) .. (0.285, 0.251)
	-- (0.285, 0.251) .. controls (0.285, 0.251) and (0.286, 0.251) .. (0.286, 0.251)
	-- (0.286, 0.252) .. controls (0.286, 0.252) and (0.286, 0.252) .. (0.287, 0.252)
	-- (0.287, 0.252) .. controls (0.287, 0.252) and (0.287, 0.252) .. (0.288, 0.252)
	-- (0.288, 0.253) .. controls (0.289, 0.253) and (0.289, 0.253) .. (0.289, 0.253)
	-- (0.289, 0.253) .. controls (0.29, 0.253) and (0.29, 0.253) .. (0.29, 0.253)
	-- (0.29, 0.254) .. controls (0.291, 0.254) and (0.291, 0.254) .. (0.291, 0.254)
	-- (0.291, 0.254) .. controls (0.291, 0.254) and (0.291, 0.254) .. (0.292, 0.254)
	-- (0.292, 0.255) .. controls (0.292, 0.255) and (0.293, 0.255) .. (0.293, 0.255)
	-- (0.293, 0.255) .. controls (0.293, 0.255) and (0.293, 0.255) .. (0.294, 0.255)
	-- (0.294, 0.255) .. controls (0.295, 0.255) and (0.295, 0.255) .. (0.295, 0.255)
	-- (0.295, 0.256) .. controls (0.295, 0.256) and (0.295, 0.256) .. (0.296, 0.256)
	-- (0.296, 0.256) .. controls (0.296, 0.256) and (0.297, 0.256) .. (0.297, 0.256)
	-- (0.297, 0.257) .. controls (0.297, 0.257) and (0.298, 0.257) .. (0.298, 0.257)
	-- (0.298, 0.257) .. controls (0.298, 0.257) and (0.299, 0.257) .. (0.299, 0.257)
	-- (0.299, 0.258) .. controls (0.3, 0.258) and (0.3, 0.258) .. (0.3, 0.258)
	-- (0.3, 0.258) .. controls (0.301, 0.258) and (0.301, 0.258) .. (0.301, 0.258)
	-- (0.301, 0.259) .. controls (0.302, 0.259) and (0.302, 0.259) .. (0.302, 0.259)
	-- (0.302, 0.259) .. controls (0.303, 0.259) and (0.303, 0.259) .. (0.303, 0.259)
	-- (0.303, 0.26) .. controls (0.303, 0.26) and (0.303, 0.26) .. (0.304, 0.26)
	-- (0.304, 0.26) .. controls (0.305, 0.26) and (0.305, 0.26) .. (0.305, 0.26)
	-- (0.305, 0.261) .. controls (0.306, 0.261) and (0.306, 0.261) .. (0.306, 0.261)
	-- (0.306, 0.261) .. controls (0.306, 0.261) and (0.307, 0.261) .. (0.307, 0.261)
	-- (0.307, 0.261) .. controls (0.307, 0.261) and (0.308, 0.261) .. (0.308, 0.261)
	-- (0.308, 0.262) .. controls (0.308, 0.262) and (0.308, 0.262) .. (0.309, 0.262)
	-- (0.309, 0.262) .. controls (0.309, 0.262) and (0.31, 0.262) .. (0.31, 0.262)
	-- (0.31, 0.262) .. controls (0.31, 0.262) and (0.311, 0.262) .. (0.311, 0.262)
	-- (0.311, 0.263) .. controls (0.311, 0.263) and (0.312, 0.263) .. (0.312, 0.263)
	-- (0.312, 0.263) .. controls (0.312, 0.263) and (0.312, 0.263) .. (0.313, 0.263)
	-- (0.313, 0.264) .. controls (0.314, 0.264) and (0.314, 0.264) .. (0.314, 0.264)
	-- (0.314, 0.264) .. controls (0.315, 0.264) and (0.315, 0.264) .. (0.315, 0.264)
	-- (0.315, 0.264) .. controls (0.315, 0.264) and (0.316, 0.264) .. (0.316, 0.264)
	-- (0.316, 0.265) .. controls (0.317, 0.265) and (0.317, 0.265) .. (0.317, 0.265)
	-- (0.317, 0.265) .. controls (0.317, 0.265) and (0.317, 0.265) .. (0.318, 0.265)
	-- (0.318, 0.265) .. controls (0.318, 0.265) and (0.319, 0.265) .. (0.319, 0.265)
	-- (0.319, 0.266) .. controls (0.32, 0.266) and (0.32, 0.266) .. (0.32, 0.266)
	-- (0.32, 0.266) .. controls (0.321, 0.266) and (0.321, 0.266) .. (0.321, 0.266)
	-- (0.321, 0.267) .. controls (0.322, 0.267) and (0.322, 0.267) .. (0.322, 0.267)
	-- (0.322, 0.267) .. controls (0.322, 0.267) and (0.322, 0.267) .. (0.323, 0.267)
	-- (0.323, 0.267) .. controls (0.324, 0.267) and (0.324, 0.267) .. (0.324, 0.267)
	-- (0.324, 0.268) .. controls (0.325, 0.268) and (0.325, 0.268) .. (0.325, 0.268)
	-- (0.325, 0.268) .. controls (0.325, 0.268) and (0.325, 0.268) .. (0.326, 0.268)
	-- (0.326, 0.269) .. controls (0.326, 0.269) and (0.326, 0.269) .. (0.327, 0.269)
	-- (0.327, 0.269) .. controls (0.327, 0.269) and (0.327, 0.269) .. (0.328, 0.269)
	-- (0.328, 0.269) .. controls (0.328, 0.269) and (0.329, 0.269) .. (0.329, 0.269)
	-- (0.329, 0.27) .. controls (0.33, 0.27) and (0.33, 0.27) .. (0.33, 0.27)
	-- (0.33, 0.27) .. controls (0.33, 0.27) and (0.33, 0.27) .. (0.331, 0.27)
	-- (0.331, 0.271) .. controls (0.331, 0.271) and (0.331, 0.271) .. (0.332, 0.271)
	-- (0.332, 0.271) .. controls (0.333, 0.271) and (0.333, 0.271) .. (0.333, 0.271)
	-- (0.333, 0.272) .. controls (0.334, 0.272) and (0.334, 0.272) .. (0.334, 0.272)
	-- (0.334, 0.272) .. controls (0.335, 0.272) and (0.335, 0.272) .. (0.335, 0.272)
	-- (0.335, 0.273) .. controls (0.335, 0.273) and (0.336, 0.273) .. (0.336, 0.273)
	-- (0.336, 0.273) .. controls (0.336, 0.273) and (0.336, 0.273) .. (0.337, 0.273)
	-- (0.337, 0.274) .. controls (0.337, 0.274) and (0.337, 0.274) .. (0.338, 0.274)
	-- (0.338, 0.274) .. controls (0.338, 0.274) and (0.339, 0.274) .. (0.339, 0.274)
	-- (0.339, 0.275) .. controls (0.34, 0.275) and (0.34, 0.275) .. (0.34, 0.275)
	-- (0.34, 0.275) .. controls (0.34, 0.275) and (0.34, 0.275) .. (0.341, 0.275)
	-- (0.341, 0.275) .. controls (0.342, 0.275) and (0.342, 0.275) .. (0.342, 0.275)
	-- (0.342, 0.276) .. controls (0.343, 0.276) and (0.343, 0.276) .. (0.343, 0.276)
	-- (0.343, 0.276) .. controls (0.344, 0.276) and (0.344, 0.276) .. (0.344, 0.276)
	-- (0.344, 0.276) .. controls (0.344, 0.276) and (0.344, 0.276) .. (0.345, 0.277)
	-- (0.345, 0.277) .. controls (0.345, 0.277) and (0.346, 0.277) .. (0.346, 0.277)
	-- (0.346, 0.277) .. controls (0.346, 0.277) and (0.347, 0.277) .. (0.347, 0.277)
	-- (0.347, 0.278) .. controls (0.348, 0.278) and (0.348, 0.278) .. (0.348, 0.278)
	-- (0.348, 0.278) .. controls (0.349, 0.278) and (0.349, 0.278) .. (0.349, 0.278)
	-- (0.349, 0.278) .. controls (0.349, 0.278) and (0.35, 0.278) .. (0.35, 0.279)
	-- (0.35, 0.279) .. controls (0.35, 0.279) and (0.35, 0.279) .. (0.351, 0.279)
	-- (0.351, 0.279) .. controls (0.352, 0.279) and (0.352, 0.279) .. (0.352, 0.279)
	-- (0.352, 0.28) .. controls (0.352, 0.28) and (0.353, 0.28) .. (0.353, 0.28)
	-- (0.353, 0.28) .. controls (0.353, 0.28) and (0.353, 0.28) .. (0.354, 0.28)
	-- (0.354, 0.281) .. controls (0.354, 0.281) and (0.355, 0.281) .. (0.355, 0.281)
	-- (0.355, 0.281) .. controls (0.355, 0.281) and (0.355, 0.281) .. (0.356, 0.281)
	-- (0.356, 0.281) .. controls (0.356, 0.281) and (0.357, 0.281) .. (0.357, 0.281)
	-- (0.357, 0.282) .. controls (0.357, 0.282) and (0.358, 0.282) .. (0.358, 0.282)
	-- (0.358, 0.282) .. controls (0.358, 0.282) and (0.358, 0.282) .. (0.359, 0.282)
	-- (0.359, 0.283) .. controls (0.359, 0.283) and (0.359, 0.283) .. (0.36, 0.283)
	-- (0.36, 0.283) .. controls (0.361, 0.283) and (0.361, 0.283) .. (0.361, 0.283)
	-- (0.361, 0.284) .. controls (0.362, 0.284) and (0.362, 0.284) .. (0.362, 0.284)
	-- (0.362, 0.284) .. controls (0.363, 0.284) and (0.363, 0.284) .. (0.363, 0.284)
	-- (0.363, 0.285) .. controls (0.363, 0.285) and (0.363, 0.285) .. (0.364, 0.285)
	-- (0.364, 0.285) .. controls (0.365, 0.285) and (0.365, 0.285) .. (0.365, 0.285)
	-- (0.365, 0.286) .. controls (0.365, 0.286) and (0.366, 0.286) .. (0.366, 0.286)
	-- (0.366, 0.286) .. controls (0.367, 0.286) and (0.367, 0.286) .. (0.367, 0.286)
	-- (0.367, 0.287) .. controls (0.367, 0.287) and (0.367, 0.287) .. (0.368, 0.287)
	-- (0.368, 0.287) .. controls (0.369, 0.287) and (0.369, 0.287) .. (0.369, 0.287)
	-- (0.369, 0.287) .. controls (0.369, 0.287) and (0.37, 0.288) .. (0.37, 0.288)
	-- (0.37, 0.288) .. controls (0.37, 0.288) and (0.371, 0.288) .. (0.371, 0.288)
	-- (0.371, 0.288) .. controls (0.371, 0.288) and (0.372, 0.288) .. (0.372, 0.288)
	-- (0.372, 0.289) .. controls (0.372, 0.289) and (0.372, 0.289) .. (0.373, 0.289)
	-- (0.373, 0.289) .. controls (0.373, 0.289) and (0.373, 0.289) .. (0.374, 0.289)
	-- (0.374, 0.29) .. controls (0.375, 0.29) and (0.375, 0.29) .. (0.375, 0.29)
	-- (0.375, 0.29) .. controls (0.376, 0.29) and (0.376, 0.29) .. (0.376, 0.29)
	-- (0.376, 0.291) .. controls (0.376, 0.291) and (0.377, 0.291) .. (0.377, 0.291)
	-- (0.377, 0.291) .. controls (0.377, 0.291) and (0.378, 0.291) .. (0.378, 0.291)
	-- (0.378, 0.292) .. controls (0.378, 0.292) and (0.379, 0.292) .. (0.379, 0.292)
	-- (0.379, 0.292) .. controls (0.38, 0.292) and (0.38, 0.292) .. (0.38, 0.292)
	-- (0.38, 0.293) .. controls (0.38, 0.293) and (0.38, 0.293) .. (0.381, 0.293)
	-- (0.381, 0.293) .. controls (0.381, 0.293) and (0.381, 0.293) .. (0.382, 0.293)
	-- (0.382, 0.294) .. controls (0.383, 0.294) and (0.383, 0.294) .. (0.383, 0.294)
	-- (0.383, 0.294) .. controls (0.383, 0.294) and (0.383, 0.294) .. (0.384, 0.294)
	-- (0.384, 0.294) .. controls (0.385, 0.294) and (0.385, 0.295) .. (0.385, 0.295)
	-- (0.385, 0.295) .. controls (0.385, 0.295) and (0.385, 0.295) .. (0.386, 0.295)
	-- (0.386, 0.295) .. controls (0.386, 0.295) and (0.386, 0.295) .. (0.387, 0.295)
	-- (0.387, 0.296) .. controls (0.388, 0.296) and (0.388, 0.296) .. (0.388, 0.296)
	-- (0.388, 0.296) .. controls (0.388, 0.296) and (0.389, 0.296) .. (0.389, 0.296)
	-- (0.389, 0.297) .. controls (0.389, 0.297) and (0.39, 0.297) .. (0.39, 0.297)
	-- (0.39, 0.297) .. controls (0.391, 0.297) and (0.391, 0.297) .. (0.391, 0.297)
	-- (0.391, 0.298) .. controls (0.391, 0.298) and (0.391, 0.298) .. (0.392, 0.298)
	-- (0.392, 0.298) .. controls (0.393, 0.298) and (0.393, 0.298) .. (0.393, 0.298)
	-- (0.393, 0.299) .. controls (0.394, 0.299) and (0.394, 0.299) .. (0.394, 0.299)
	-- (0.394, 0.299) .. controls (0.395, 0.299) and (0.395, 0.299) .. (0.395, 0.299)
	-- (0.395, 0.3) .. controls (0.395, 0.3) and (0.395, 0.3) .. (0.396, 0.3)
	-- (0.396, 0.3) .. controls (0.397, 0.3) and (0.397, 0.3) .. (0.397, 0.3)
	-- (0.397, 0.301) .. controls (0.397, 0.301) and (0.397, 0.301) .. (0.398, 0.301)
	-- (0.398, 0.301) .. controls (0.398, 0.301) and (0.398, 0.301) .. (0.399, 0.301)
	-- (0.399, 0.302) .. controls (0.399, 0.302) and (0.399, 0.302) .. (0.4, 0.302)
	-- (0.4, 0.302) .. controls (0.4, 0.302) and (0.4, 0.302) .. (0.401, 0.302)
	-- (0.401, 0.303) .. controls (0.401, 0.303) and (0.402, 0.303) .. (0.402, 0.303)
	-- (0.402, 0.303) .. controls (0.403, 0.303) and (0.403, 0.303) .. (0.403, 0.303)
	-- (0.403, 0.304) .. controls (0.403, 0.304) and (0.403, 0.304) .. (0.404, 0.304)
	-- (0.404, 0.304) .. controls (0.405, 0.304) and (0.405, 0.304) .. (0.405, 0.304)
	-- (0.405, 0.304) .. controls (0.405, 0.304) and (0.405, 0.305) .. (0.406, 0.305)
	-- (0.406, 0.305) .. controls (0.406, 0.305) and (0.406, 0.305) .. (0.407, 0.305)
	-- (0.407, 0.305) .. controls (0.408, 0.305) and (0.408, 0.306) .. (0.408, 0.306)
	-- (0.408, 0.306) .. controls (0.409, 0.306) and (0.409, 0.306) .. (0.409, 0.306)
	-- (0.409, 0.306) .. controls (0.409, 0.306) and (0.41, 0.306) .. (0.41, 0.306)
	-- (0.41, 0.307) .. controls (0.41, 0.307) and (0.41, 0.307) .. (0.411, 0.307)
	-- (0.411, 0.307) .. controls (0.411, 0.307) and (0.412, 0.307) .. (0.412, 0.307)
	-- (0.412, 0.308) .. controls (0.412, 0.308) and (0.412, 0.308) .. (0.413, 0.308)
	-- (0.413, 0.308) .. controls (0.414, 0.308) and (0.414, 0.308) .. (0.414, 0.308)
	-- (0.414, 0.309) .. controls (0.415, 0.309) and (0.415, 0.309) .. (0.415, 0.309)
	-- (0.415, 0.309) .. controls (0.415, 0.309) and (0.415, 0.309) .. (0.416, 0.309)
	-- (0.416, 0.31) .. controls (0.416, 0.31) and (0.416, 0.31) .. (0.417, 0.31)
	-- (0.417, 0.31) .. controls (0.418, 0.31) and (0.418, 0.31) .. (0.418, 0.31)
	-- (0.418, 0.311) .. controls (0.418, 0.311) and (0.418, 0.311) .. (0.419, 0.311)
	-- (0.419, 0.311) .. controls (0.42, 0.311) and (0.42, 0.311) .. (0.42, 0.311)
	-- (0.42, 0.312) .. controls (0.42, 0.312) and (0.421, 0.312) .. (0.421, 0.312)
	-- (0.421, 0.312) .. controls (0.421, 0.312) and (0.422, 0.312) .. (0.422, 0.312)
	-- (0.422, 0.313) .. controls (0.422, 0.313) and (0.423, 0.313) .. (0.423, 0.313)
	-- (0.423, 0.313) .. controls (0.423, 0.313) and (0.424, 0.313) .. (0.424, 0.313)
	-- (0.424, 0.314) .. controls (0.424, 0.314) and (0.424, 0.314) .. (0.425, 0.314)
	-- (0.425, 0.314) .. controls (0.425, 0.314) and (0.425, 0.314) .. (0.426, 0.314)
	-- (0.426, 0.314) .. controls (0.426, 0.315) and (0.427, 0.315) .. (0.427, 0.315)
	-- (0.427, 0.315) .. controls (0.428, 0.315) and (0.428, 0.315) .. (0.428, 0.315)
	-- (0.428, 0.315) .. controls (0.428, 0.316) and (0.429, 0.316) .. (0.429, 0.316)
	-- (0.429, 0.316) .. controls (0.43, 0.316) and (0.43, 0.316) .. (0.43, 0.316)
	-- (0.43, 0.316) .. controls (0.431, 0.316) and (0.431, 0.317) .. (0.431, 0.317)
	-- (0.431, 0.317) .. controls (0.431, 0.317) and (0.432, 0.317) .. (0.432, 0.317)
	-- (0.432, 0.317) .. controls (0.432, 0.317) and (0.432, 0.317) .. (0.433, 0.317)
	-- (0.433, 0.318) .. controls (0.434, 0.318) and (0.434, 0.318) .. (0.434, 0.318)
	-- (0.434, 0.318) .. controls (0.435, 0.318) and (0.435, 0.318) .. (0.435, 0.318)
	-- (0.435, 0.319) .. controls (0.436, 0.319) and (0.436, 0.319) .. (0.436, 0.319)
	-- (0.436, 0.319) .. controls (0.437, 0.319) and (0.437, 0.319) .. (0.437, 0.319)
	-- (0.437, 0.32) .. controls (0.437, 0.32) and (0.438, 0.32) .. (0.438, 0.32)
	-- (0.438, 0.32) .. controls (0.438, 0.32) and (0.438, 0.32) .. (0.439, 0.32)
	-- (0.439, 0.32) .. controls (0.44, 0.32) and (0.44, 0.32) .. (0.44, 0.32)
	-- (0.44, 0.321) .. controls (0.44, 0.321) and (0.44, 0.321) .. (0.441, 0.321)
	-- (0.441, 0.321) .. controls (0.441, 0.321) and (0.441, 0.321) .. (0.442, 0.321)
	-- (0.442, 0.322) .. controls (0.442, 0.322) and (0.443, 0.322) .. (0.443, 0.322)
	-- (0.443, 0.322) .. controls (0.443, 0.322) and (0.444, 0.322) .. (0.444, 0.322)
	-- (0.444, 0.322) .. controls (0.445, 0.322) and (0.445, 0.322) .. (0.445, 0.322)
	-- (0.445, 0.323) .. controls (0.445, 0.323) and (0.445, 0.323) .. (0.446, 0.323)
	-- (0.446, 0.323) .. controls (0.447, 0.323) and (0.447, 0.323) .. (0.447, 0.323)
	-- (0.447, 0.323) .. controls (0.447, 0.323) and (0.447, 0.323) .. (0.448, 0.323)
	-- (0.448, 0.324) .. controls (0.448, 0.324) and (0.448, 0.324) .. (0.449, 0.324)
	-- (0.449, 0.324) .. controls (0.449, 0.324) and (0.45, 0.324) .. (0.45, 0.324)
	-- (0.45, 0.324) .. controls (0.451, 0.324) and (0.451, 0.324) .. (0.451, 0.324)
	-- (0.451, 0.325) .. controls (0.451, 0.325) and (0.452, 0.325) .. (0.452, 0.325)
	-- (0.452, 0.325) .. controls (0.453, 0.325) and (0.453, 0.325) .. (0.453, 0.325)
	-- (0.453, 0.325) .. controls (0.453, 0.325) and (0.453, 0.325) .. (0.454, 0.325)
	-- (0.454, 0.325) .. controls (0.454, 0.326) and (0.454, 0.326) .. (0.455, 0.326)
	-- (0.455, 0.326) .. controls (0.455, 0.326) and (0.455, 0.326) .. (0.456, 0.326)
	-- (0.456, 0.326) .. controls (0.456, 0.326) and (0.457, 0.326) .. (0.457, 0.326)
	-- (0.457, 0.326) .. controls (0.457, 0.326) and (0.457, 0.326) .. (0.458, 0.326)
	-- (0.458, 0.327) .. controls (0.458, 0.327) and (0.458, 0.327) .. (0.459, 0.327)
	-- (0.459, 0.327) .. controls (0.459, 0.327) and (0.459, 0.327) .. (0.46, 0.327)
	-- (0.46, 0.327) .. controls (0.46, 0.327) and (0.46, 0.327) .. (0.461, 0.327)
	-- (0.461, 0.328) .. controls (0.462, 0.328) and (0.462, 0.328) .. (0.462, 0.328)
	-- (0.462, 0.328) .. controls (0.463, 0.328) and (0.463, 0.328) .. (0.463, 0.328)
	-- (0.463, 0.328) .. controls (0.464, 0.328) and (0.464, 0.328) .. (0.464, 0.328)
	-- (0.464, 0.329) .. controls (0.465, 0.329) and (0.465, 0.329) .. (0.465, 0.329)
	-- (0.465, 0.329) .. controls (0.466, 0.329) and (0.466, 0.329) .. (0.466, 0.329)
	-- (0.466, 0.329) .. controls (0.466, 0.329) and (0.467, 0.329) .. (0.467, 0.329)
	-- (0.467, 0.329) .. controls (0.468, 0.329) and (0.468, 0.329) .. (0.468, 0.329)
	-- (0.468, 0.33) .. controls (0.469, 0.33) and (0.469, 0.33) .. (0.469, 0.33)
	-- (0.469, 0.33) .. controls (0.47, 0.33) and (0.47, 0.33) .. (0.47, 0.33)
	-- (0.47, 0.33) .. controls (0.47, 0.33) and (0.471, 0.33) .. (0.471, 0.33)
	-- (0.471, 0.33) .. controls (0.471, 0.33) and (0.471, 0.33) .. (0.472, 0.33)
	-- (0.472, 0.331) .. controls (0.472, 0.331) and (0.473, 0.331) .. (0.473, 0.331)
	-- (0.473, 0.331) .. controls (0.473, 0.331) and (0.473, 0.331) .. (0.474, 0.331)
	-- (0.474, 0.331) .. controls (0.474, 0.331) and (0.475, 0.331) .. (0.475, 0.331)
	-- (0.475, 0.331) .. controls (0.476, 0.331) and (0.476, 0.331) .. (0.476, 0.331)
	-- (0.476, 0.332) .. controls (0.477, 0.332) and (0.477, 0.332) .. (0.477, 0.332)
	-- (0.477, 0.332) .. controls (0.478, 0.332) and (0.478, 0.332) .. (0.478, 0.332)
	-- (0.478, 0.332) .. controls (0.478, 0.332) and (0.479, 0.332) .. (0.479, 0.332)
	-- (0.479, 0.332) .. controls (0.479, 0.332) and (0.48, 0.332) .. (0.48, 0.332)
	-- (0.48, 0.332) .. controls (0.48, 0.332) and (0.481, 0.332) .. (0.481, 0.333)
	-- (0.481, 0.333) .. controls (0.481, 0.333) and (0.482, 0.333) .. (0.482, 0.333)
	-- (0.482, 0.333) .. controls (0.482, 0.333) and (0.482, 0.333) .. (0.483, 0.333)
	-- (0.483, 0.333) .. controls (0.483, 0.333) and (0.483, 0.333) .. (0.484, 0.333)
	-- (0.484, 0.334) .. controls (0.484, 0.334) and (0.484, 0.334) .. (0.485, 0.334)
	-- (0.485, 0.334) .. controls (0.485, 0.334) and (0.486, 0.334) .. (0.486, 0.334)
	-- (0.486, 0.334) .. controls (0.487, 0.334) and (0.487, 0.334) .. (0.487, 0.334)
	-- (0.487, 0.334) .. controls (0.488, 0.334) and (0.488, 0.334) .. (0.488, 0.334)
	-- (0.488, 0.335) .. controls (0.489, 0.335) and (0.489, 0.335) .. (0.489, 0.335)
	-- (0.489, 0.335) .. controls (0.49, 0.335) and (0.49, 0.335) .. (0.49, 0.335)
	-- (0.49, 0.335) .. controls (0.49, 0.335) and (0.49, 0.335) .. (0.491, 0.335)
	-- (0.491, 0.335) .. controls (0.491, 0.335) and (0.492, 0.335) .. (0.492, 0.335)
	-- (0.492, 0.336) .. controls (0.492, 0.336) and (0.492, 0.336) .. (0.493, 0.336)
	-- (0.493, 0.336) .. controls (0.494, 0.336) and (0.494, 0.336) .. (0.494, 0.336)
	-- (0.494, 0.336) .. controls (0.494, 0.336) and (0.494, 0.336) .. (0.495, 0.336)
	-- (0.495, 0.336) .. controls (0.495, 0.336) and (0.496, 0.336) .. (0.496, 0.336)
	-- (0.496, 0.337) .. controls (0.496, 0.337) and (0.497, 0.337) .. (0.497, 0.337)
	-- (0.497, 0.337) .. controls (0.497, 0.337) and (0.497, 0.337) .. (0.498, 0.337)
	-- (0.498, 0.337) .. controls (0.499, 0.337) and (0.499, 0.337) .. (0.499, 0.337)
	-- (0.499, 0.337) .. controls (0.5, 0.337) and (0.5, 0.337) .. (0.5, 0.337)
	-- (0.5, 0.338) .. controls (0.501, 0.338) and (0.501, 0.338) .. (0.501, 0.338)
	-- (0.501, 0.338) .. controls (0.501, 0.338) and (0.501, 0.338) .. (0.502, 0.338)
	-- (0.502, 0.338) .. controls (0.502, 0.338) and (0.502, 0.338) .. (0.503, 0.338)
	-- (0.503, 0.338) .. controls (0.504, 0.338) and (0.504, 0.338) .. (0.504, 0.338)
	-- (0.504, 0.338) .. controls (0.504, 0.338) and (0.505, 0.338) .. (0.505, 0.339)
	-- (0.505, 0.339) .. controls (0.505, 0.339) and (0.506, 0.339) .. (0.506, 0.339)
	-- (0.506, 0.339) .. controls (0.506, 0.339) and (0.506, 0.339) .. (0.507, 0.339)
	-- (0.507, 0.339) .. controls (0.508, 0.339) and (0.508, 0.339) .. (0.508, 0.339)
	-- (0.508, 0.339) .. controls (0.508, 0.339) and (0.508, 0.339) .. (0.509, 0.339)
	-- (0.509, 0.339) .. controls (0.509, 0.339) and (0.51, 0.339) .. (0.51, 0.339)
	-- (0.51, 0.34) .. controls (0.511, 0.34) and (0.511, 0.34) .. (0.511, 0.34)
	-- (0.511, 0.34) .. controls (0.511, 0.34) and (0.511, 0.34) .. (0.512, 0.34)
	-- (0.512, 0.34) .. controls (0.512, 0.34) and (0.512, 0.34) .. (0.513, 0.34)
	-- (0.513, 0.34) .. controls (0.513, 0.34) and (0.513, 0.34) .. (0.514, 0.34)
	-- (0.514, 0.341) .. controls (0.514, 0.341) and (0.514, 0.341) .. (0.515, 0.341)
	-- (0.515, 0.341) .. controls (0.515, 0.341) and (0.515, 0.341) .. (0.516, 0.341)
	-- (0.516, 0.341) .. controls (0.516, 0.341) and (0.517, 0.341) .. (0.517, 0.341)
	-- (0.517, 0.341) .. controls (0.518, 0.341) and (0.518, 0.341) .. (0.518, 0.341)
	-- (0.518, 0.342) .. controls (0.518, 0.342) and (0.518, 0.342) .. (0.519, 0.342)
	-- (0.519, 0.342) .. controls (0.519, 0.342) and (0.52, 0.342) .. (0.52, 0.342)
	-- (0.52, 0.342) .. controls (0.521, 0.342) and (0.521, 0.342) .. (0.521, 0.342)
	-- (0.521, 0.342) .. controls (0.522, 0.342) and (0.522, 0.342) .. (0.522, 0.342)
	-- (0.522, 0.342) .. controls (0.523, 0.342) and (0.523, 0.342) .. (0.523, 0.342)
	-- (0.523, 0.343) .. controls (0.523, 0.343) and (0.524, 0.343) .. (0.524, 0.343)
	-- (0.524, 0.343) .. controls (0.524, 0.343) and (0.525, 0.343) .. (0.525, 0.343)
	-- (0.525, 0.343) .. controls (0.526, 0.343) and (0.526, 0.343) .. (0.526, 0.343)
	-- (0.526, 0.343) .. controls (0.527, 0.343) and (0.527, 0.343) .. (0.527, 0.343)
	-- (0.527, 0.343) .. controls (0.527, 0.343) and (0.527, 0.343) .. (0.528, 0.343)
	-- (0.528, 0.343) .. controls (0.528, 0.343) and (0.529, 0.343) .. (0.529, 0.343)
	-- (0.529, 0.344) .. controls (0.529, 0.344) and (0.53, 0.344) .. (0.53, 0.344)
	-- (0.53, 0.344) .. controls (0.53, 0.344) and (0.531, 0.344) .. (0.531, 0.344)
	-- (0.531, 0.344) .. controls (0.532, 0.344) and (0.532, 0.344) .. (0.532, 0.344)
	-- (0.532, 0.344) .. controls (0.532, 0.344) and (0.532, 0.344) .. (0.533, 0.344)
	-- (0.533, 0.344) .. controls (0.533, 0.344) and (0.534, 0.344) .. (0.534, 0.344)
	-- (0.534, 0.344) .. controls (0.534, 0.344) and (0.535, 0.344) .. (0.535, 0.344)
	-- (0.535, 0.344) .. controls (0.536, 0.344) and (0.536, 0.344) .. (0.536, 0.344)
	-- (0.536, 0.344) .. controls (0.537, 0.344) and (0.537, 0.344) .. (0.537, 0.344)
	-- (0.537, 0.344) .. controls (0.537, 0.344) and (0.538, 0.344) .. (0.538, 0.344)
	-- (0.538, 0.344) .. controls (0.538, 0.344) and (0.539, 0.344) .. (0.539, 0.344)
	-- (0.539, 0.344) .. controls (0.539, 0.344) and (0.54, 0.344) .. (0.54, 0.344)
	-- (0.54, 0.344) .. controls (0.541, 0.344) and (0.541, 0.344) .. (0.541, 0.344)
	-- (0.541, 0.344) .. controls (0.541, 0.344) and (0.542, 0.344) .. (0.542, 0.344)
	-- (0.542, 0.344) .. controls (0.542, 0.344) and (0.543, 0.344) .. (0.543, 0.344)
	-- (0.543, 0.344) .. controls (0.543, 0.344) and (0.544, 0.344) .. (0.544, 0.344)
	-- (0.544, 0.344) .. controls (0.544, 0.344) and (0.545, 0.344) .. (0.545, 0.344)
	-- (0.545, 0.344) .. controls (0.545, 0.344) and (0.546, 0.344) .. (0.546, 0.344)
	-- (0.546, 0.344) .. controls (0.546, 0.344) and (0.546, 0.344) .. (0.547, 0.344)
	-- (0.547, 0.344) .. controls (0.548, 0.344) and (0.548, 0.344) .. (0.548, 0.344)
	-- (0.548, 0.344) .. controls (0.548, 0.344) and (0.548, 0.344) .. (0.549, 0.344)
	-- (0.549, 0.344) .. controls (0.55, 0.344) and (0.55, 0.344) .. (0.55, 0.344)
	-- (0.55, 0.344) .. controls (0.551, 0.344) and (0.551, 0.344) .. (0.551, 0.344)
	-- (0.551, 0.344) .. controls (0.552, 0.343) and (0.552, 0.343) .. (0.552, 0.343)
	-- (0.552, 0.343) .. controls (0.553, 0.343) and (0.553, 0.343) .. (0.553, 0.343)
	-- (0.553, 0.343) .. controls (0.554, 0.343) and (0.554, 0.343) .. (0.554, 0.343)
	-- (0.554, 0.343) .. controls (0.554, 0.343) and (0.554, 0.343) .. (0.555, 0.343)
	-- (0.555, 0.343) .. controls (0.556, 0.343) and (0.556, 0.343) .. (0.556, 0.343)
	-- (0.556, 0.343) .. controls (0.556, 0.343) and (0.556, 0.343) .. (0.557, 0.343)
	-- (0.557, 0.343) .. controls (0.557, 0.343) and (0.557, 0.343) .. (0.558, 0.343)
	-- (0.558, 0.343) .. controls (0.558, 0.343) and (0.559, 0.343) .. (0.559, 0.343)
	-- (0.559, 0.343) .. controls (0.56, 0.343) and (0.56, 0.343) .. (0.56, 0.343)
	-- (0.56, 0.343) .. controls (0.56, 0.343) and (0.561, 0.343) .. (0.561, 0.343)
	-- (0.561, 0.343) .. controls (0.562, 0.343) and (0.562, 0.343) .. (0.562, 0.343)
	-- (0.562, 0.342) .. controls (0.562, 0.342) and (0.563, 0.342) .. (0.563, 0.342)
	-- (0.563, 0.342) .. controls (0.564, 0.342) and (0.564, 0.342) .. (0.564, 0.342)
	-- (0.564, 0.342) .. controls (0.565, 0.342) and (0.565, 0.342) .. (0.565, 0.342)
	-- (0.565, 0.342) .. controls (0.566, 0.342) and (0.566, 0.342) .. (0.566, 0.342)
	-- (0.566, 0.342) .. controls (0.567, 0.342) and (0.567, 0.342) .. (0.567, 0.342)
	-- (0.567, 0.342) .. controls (0.568, 0.342) and (0.568, 0.342) .. (0.568, 0.342)
	-- (0.568, 0.342) .. controls (0.568, 0.342) and (0.569, 0.342) .. (0.569, 0.342)
	-- (0.569, 0.342) .. controls (0.569, 0.342) and (0.569, 0.342) .. (0.57, 0.342)
	-- (0.57, 0.342) .. controls (0.57, 0.342) and (0.571, 0.342) .. (0.571, 0.342)
	-- (0.571, 0.341) .. controls (0.571, 0.341) and (0.572, 0.341) .. (0.572, 0.341)
	-- (0.572, 0.341) .. controls (0.572, 0.341) and (0.572, 0.341) .. (0.573, 0.341)
	-- (0.573, 0.341) .. controls (0.573, 0.341) and (0.573, 0.341) .. (0.574, 0.341)
	-- (0.574, 0.341) .. controls (0.575, 0.341) and (0.575, 0.341) .. (0.575, 0.341)
	-- (0.575, 0.341) .. controls (0.575, 0.341) and (0.575, 0.341) .. (0.576, 0.341)
	-- (0.576, 0.341) .. controls (0.576, 0.341) and (0.576, 0.341) .. (0.577, 0.341)
	-- (0.577, 0.341) .. controls (0.578, 0.341) and (0.578, 0.341) .. (0.578, 0.341)
	-- (0.578, 0.341) .. controls (0.578, 0.341) and (0.578, 0.341) .. (0.579, 0.341)
	-- (0.579, 0.341) .. controls (0.579, 0.341) and (0.579, 0.341) .. (0.58, 0.341)
	-- (0.58, 0.341) .. controls (0.581, 0.341) and (0.581, 0.341) .. (0.581, 0.341)
	-- (0.581, 0.34) .. controls (0.582, 0.34) and (0.582, 0.34) .. (0.582, 0.34)
	-- (0.582, 0.34) .. controls (0.582, 0.34) and (0.583, 0.34) .. (0.583, 0.34)
	-- (0.583, 0.34) .. controls (0.583, 0.34) and (0.583, 0.34) .. (0.584, 0.34)
	-- (0.584, 0.34) .. controls (0.584, 0.34) and (0.585, 0.34) .. (0.585, 0.34)
	-- (0.585, 0.34) .. controls (0.585, 0.34) and (0.586, 0.34) .. (0.586, 0.34)
	-- (0.586, 0.34) .. controls (0.586, 0.34) and (0.586, 0.34) .. (0.587, 0.34)
	-- (0.587, 0.34) .. controls (0.588, 0.34) and (0.588, 0.34) .. (0.588, 0.34)
	-- (0.588, 0.34) .. controls (0.589, 0.34) and (0.589, 0.34) .. (0.589, 0.34)
	-- (0.589, 0.34) .. controls (0.589, 0.34) and (0.589, 0.34) .. (0.59, 0.34)
	-- (0.59, 0.339) .. controls (0.59, 0.339) and (0.591, 0.339) .. (0.591, 0.339)
	-- (0.591, 0.339) .. controls (0.592, 0.339) and (0.592, 0.339) .. (0.592, 0.339)
	-- (0.592, 0.339) .. controls (0.592, 0.339) and (0.593, 0.339) .. (0.593, 0.339)
	-- (0.593, 0.339) .. controls (0.593, 0.339) and (0.593, 0.339) .. (0.594, 0.339)
	-- (0.594, 0.339) .. controls (0.594, 0.339) and (0.595, 0.339) .. (0.595, 0.339)
	-- (0.595, 0.339) .. controls (0.595, 0.339) and (0.596, 0.339) .. (0.596, 0.339)
	-- (0.596, 0.338) .. controls (0.596, 0.338) and (0.596, 0.338) .. (0.597, 0.338)
	-- (0.597, 0.338) .. controls (0.597, 0.338) and (0.598, 0.338) .. (0.598, 0.338)
	-- (0.598, 0.338) .. controls (0.598, 0.338) and (0.599, 0.338) .. (0.599, 0.338)
	-- (0.599, 0.338) .. controls (0.599, 0.338) and (0.6, 0.338) .. (0.6, 0.338)
	-- (0.6, 0.338) .. controls (0.6, 0.338) and (0.6, 0.338) .. (0.601, 0.338)
	-- (0.601, 0.337) .. controls (0.602, 0.337) and (0.602, 0.337) .. (0.602, 0.337)
	-- (0.602, 0.337) .. controls (0.602, 0.337) and (0.602, 0.337) .. (0.603, 0.337)
	-- (0.603, 0.337) .. controls (0.603, 0.337) and (0.604, 0.337) .. (0.604, 0.337)
	-- (0.604, 0.337) .. controls (0.604, 0.337) and (0.604, 0.337) .. (0.605, 0.337)
	-- (0.605, 0.337) .. controls (0.605, 0.337) and (0.605, 0.337) .. (0.606, 0.337)
	-- (0.606, 0.337) .. controls (0.606, 0.337) and (0.607, 0.336) .. (0.607, 0.336)
	-- (0.607, 0.336) .. controls (0.607, 0.336) and (0.608, 0.336) .. (0.608, 0.336)
	-- (0.608, 0.336) .. controls (0.609, 0.336) and (0.609, 0.336) .. (0.609, 0.336)
	-- (0.609, 0.336) .. controls (0.61, 0.336) and (0.61, 0.336) .. (0.61, 0.336)
	-- (0.61, 0.336) .. controls (0.611, 0.336) and (0.611, 0.336) .. (0.611, 0.336)
	-- (0.611, 0.336) .. controls (0.612, 0.336) and (0.612, 0.336) .. (0.612, 0.336)
	-- (0.612, 0.336) .. controls (0.612, 0.336) and (0.613, 0.336) .. (0.613, 0.336)
	-- (0.613, 0.336) .. controls (0.614, 0.336) and (0.614, 0.336) .. (0.614, 0.336)
	-- (0.614, 0.335) .. controls (0.614, 0.335) and (0.615, 0.335) .. (0.615, 0.335)
	-- (0.615, 0.335) .. controls (0.616, 0.335) and (0.616, 0.335) .. (0.616, 0.335)
	-- (0.616, 0.335) .. controls (0.616, 0.335) and (0.617, 0.335) .. (0.617, 0.335)
	-- (0.617, 0.335) .. controls (0.618, 0.335) and (0.618, 0.335) .. (0.618, 0.335)
	-- (0.618, 0.335) .. controls (0.618, 0.335) and (0.618, 0.335) .. (0.619, 0.335)
	-- (0.619, 0.335) .. controls (0.619, 0.335) and (0.62, 0.335) .. (0.62, 0.335)
	-- (0.62, 0.335) .. controls (0.62, 0.335) and (0.621, 0.335) .. (0.621, 0.335)
	-- (0.621, 0.335) .. controls (0.622, 0.335) and (0.622, 0.335) .. (0.622, 0.335)
	-- (0.622, 0.335) .. controls (0.622, 0.335) and (0.622, 0.335) .. (0.623, 0.335)
	-- (0.623, 0.334) .. controls (0.624, 0.334) and (0.624, 0.334) .. (0.624, 0.334)
	-- (0.624, 0.334) .. controls (0.624, 0.334) and (0.625, 0.334) .. (0.625, 0.334)
	-- (0.625, 0.334) .. controls (0.626, 0.334) and (0.626, 0.334) .. (0.626, 0.334)
	-- (0.626, 0.334) .. controls (0.626, 0.334) and (0.626, 0.334) .. (0.627, 0.334)
	-- (0.627, 0.334) .. controls (0.628, 0.334) and (0.628, 0.334) .. (0.628, 0.334)
	-- (0.628, 0.334) .. controls (0.628, 0.334) and (0.628, 0.334) .. (0.629, 0.334)
	-- (0.629, 0.334) .. controls (0.629, 0.334) and (0.63, 0.334) .. (0.63, 0.334)
	-- (0.63, 0.334) .. controls (0.63, 0.334) and (0.63, 0.334) .. (0.631, 0.334)
	-- (0.631, 0.334) .. controls (0.632, 0.334) and (0.632, 0.334) .. (0.632, 0.334)
	-- (0.632, 0.334) .. controls (0.633, 0.334) and (0.633, 0.334) .. (0.633, 0.334)
	-- (0.633, 0.334) .. controls (0.633, 0.334) and (0.634, 0.334) .. (0.634, 0.334)
	-- (0.634, 0.334) .. controls (0.635, 0.334) and (0.635, 0.333) .. (0.635, 0.333)
	-- (0.635, 0.333) .. controls (0.635, 0.333) and (0.635, 0.333) .. (0.636, 0.333)
	-- (0.636, 0.333) .. controls (0.637, 0.333) and (0.637, 0.333) .. (0.637, 0.333)
	-- (0.637, 0.333) .. controls (0.637, 0.333) and (0.637, 0.333) .. (0.638, 0.333)
	-- (0.638, 0.333) .. controls (0.638, 0.333) and (0.639, 0.333) .. (0.639, 0.333)
	-- (0.639, 0.333) .. controls (0.639, 0.333) and (0.64, 0.333) .. (0.64, 0.333)
	-- (0.64, 0.333) .. controls (0.641, 0.333) and (0.641, 0.333) .. (0.641, 0.333)
	-- (0.641, 0.333) .. controls (0.641, 0.333) and (0.642, 0.333) .. (0.642, 0.333)
	-- (0.642, 0.333) .. controls (0.642, 0.333) and (0.643, 0.333) .. (0.643, 0.333)
	-- (0.643, 0.333) .. controls (0.643, 0.333) and (0.643, 0.333) .. (0.644, 0.333)
	-- (0.644, 0.333) .. controls (0.644, 0.333) and (0.645, 0.333) .. (0.645, 0.333)
	-- (0.645, 0.333) .. controls (0.645, 0.333) and (0.646, 0.333) .. (0.646, 0.333)
	-- (0.646, 0.333) .. controls (0.647, 0.333) and (0.647, 0.333) .. (0.647, 0.333)
	-- (0.647, 0.333) .. controls (0.647, 0.333) and (0.648, 0.333) .. (0.648, 0.333)
	-- (0.648, 0.332) .. controls (0.649, 0.332) and (0.649, 0.332) .. (0.649, 0.332)
	-- (0.649, 0.332) .. controls (0.649, 0.332) and (0.649, 0.332) .. (0.65, 0.332)
	-- (0.65, 0.332) .. controls (0.651, 0.332) and (0.651, 0.332) .. (0.651, 0.332)
	-- (0.651, 0.332) .. controls (0.652, 0.332) and (0.652, 0.332) .. (0.652, 0.332)
	-- (0.652, 0.332) .. controls (0.652, 0.332) and (0.652, 0.332) .. (0.653, 0.332)
	-- (0.653, 0.332) .. controls (0.653, 0.332) and (0.654, 0.332) .. (0.654, 0.332)
	-- (0.654, 0.332) .. controls (0.654, 0.332) and (0.655, 0.332) .. (0.655, 0.332)
	-- (0.655, 0.331) .. controls (0.656, 0.331) and (0.656, 0.331) .. (0.656, 0.331)
	-- (0.656, 0.331) .. controls (0.657, 0.331) and (0.657, 0.331) .. (0.657, 0.331)
	-- (0.657, 0.331) .. controls (0.658, 0.331) and (0.658, 0.331) .. (0.658, 0.331)
	-- (0.658, 0.331) .. controls (0.658, 0.331) and (0.658, 0.331) .. (0.659, 0.331)
	-- (0.659, 0.331) .. controls (0.659, 0.331) and (0.66, 0.331) .. (0.66, 0.331)
	-- (0.66, 0.331) .. controls (0.66, 0.331) and (0.66, 0.331) .. (0.661, 0.331)
	-- (0.661, 0.331) .. controls (0.662, 0.331) and (0.662, 0.331) .. (0.662, 0.331)
	-- (0.662, 0.33) .. controls (0.662, 0.33) and (0.662, 0.33) .. (0.663, 0.33)
	-- (0.663, 0.33) .. controls (0.663, 0.33) and (0.663, 0.33) .. (0.664, 0.33)
	-- (0.664, 0.33) .. controls (0.664, 0.33) and (0.665, 0.33) .. (0.665, 0.33)
	-- (0.665, 0.33) .. controls (0.666, 0.33) and (0.666, 0.33) .. (0.666, 0.33)
	-- (0.666, 0.33) .. controls (0.666, 0.33) and (0.666, 0.33) .. (0.667, 0.33)
	-- (0.667, 0.329) .. controls (0.667, 0.329) and (0.668, 0.329) .. (0.668, 0.329)
	-- (0.668, 0.329) .. controls (0.668, 0.329) and (0.669, 0.329) .. (0.669, 0.329)
	-- (0.669, 0.329) .. controls (0.669, 0.329) and (0.67, 0.329) .. (0.67, 0.329)
	-- (0.67, 0.329) .. controls (0.671, 0.329) and (0.671, 0.329) .. (0.671, 0.329)
	-- (0.671, 0.329) .. controls (0.671, 0.329) and (0.671, 0.329) .. (0.672, 0.329)
	-- (0.672, 0.328) .. controls (0.673, 0.328) and (0.673, 0.328) .. (0.673, 0.328)
	-- (0.673, 0.328) .. controls (0.673, 0.328) and (0.674, 0.328) .. (0.674, 0.328)
	-- (0.674, 0.328) .. controls (0.675, 0.328) and (0.675, 0.328) .. (0.675, 0.328)
	-- (0.675, 0.328) .. controls (0.676, 0.328) and (0.676, 0.328) .. (0.676, 0.328)
	-- (0.676, 0.328) .. controls (0.677, 0.328) and (0.677, 0.328) .. (0.677, 0.328)
	-- (0.677, 0.328) .. controls (0.677, 0.328) and (0.678, 0.328) .. (0.678, 0.328)
	-- (0.678, 0.328) .. controls (0.678, 0.328) and (0.678, 0.328) .. (0.679, 0.328)
	-- (0.679, 0.327) .. controls (0.679, 0.327) and (0.68, 0.327) .. (0.68, 0.327)
	-- (0.68, 0.327) .. controls (0.68, 0.327) and (0.681, 0.327) .. (0.681, 0.327)
	-- (0.681, 0.327) .. controls (0.681, 0.327) and (0.682, 0.327) .. (0.682, 0.327)
	-- (0.682, 0.327) .. controls (0.682, 0.327) and (0.683, 0.327) .. (0.683, 0.327)
	-- (0.683, 0.327) .. controls (0.684, 0.327) and (0.684, 0.327) .. (0.684, 0.327)
	-- (0.684, 0.326) .. controls (0.684, 0.326) and (0.684, 0.326) .. (0.685, 0.326)
	-- (0.685, 0.326) .. controls (0.685, 0.326) and (0.686, 0.326) .. (0.686, 0.326)
	-- (0.686, 0.326) .. controls (0.686, 0.326) and (0.687, 0.326) .. (0.687, 0.326)
	-- (0.687, 0.326) .. controls (0.687, 0.326) and (0.688, 0.326) .. (0.688, 0.326)
	-- (0.688, 0.326) .. controls (0.689, 0.326) and (0.689, 0.326) .. (0.689, 0.326)
	-- (0.689, 0.326) .. controls (0.689, 0.326) and (0.689, 0.326) .. (0.69, 0.326)
	-- (0.69, 0.326) .. controls (0.69, 0.326) and (0.691, 0.326) .. (0.691, 0.325)
	-- (0.691, 0.325) .. controls (0.691, 0.325) and (0.692, 0.325) .. (0.692, 0.325)
	-- (0.692, 0.325) .. controls (0.693, 0.325) and (0.693, 0.325) .. (0.693, 0.325)
	-- (0.693, 0.325) .. controls (0.693, 0.325) and (0.693, 0.325) .. (0.694, 0.325)
	-- (0.694, 0.325) .. controls (0.694, 0.325) and (0.694, 0.325) .. (0.695, 0.325)
	-- (0.695, 0.325) .. controls (0.696, 0.325) and (0.696, 0.325) .. (0.696, 0.325)
	-- (0.696, 0.325) .. controls (0.696, 0.325) and (0.696, 0.325) .. (0.697, 0.325)
	-- (0.697, 0.325) .. controls (0.697, 0.325) and (0.697, 0.325) .. (0.698, 0.325)
	-- (0.698, 0.325) .. controls (0.698, 0.325) and (0.698, 0.325) .. (0.699, 0.325)
	-- (0.699, 0.325) .. controls (0.7, 0.325) and (0.7, 0.325) .. (0.7, 0.325)
	-- (0.7, 0.325) .. controls (0.701, 0.325) and (0.701, 0.325) .. (0.701, 0.325)
	-- (0.701, 0.324) .. controls (0.702, 0.324) and (0.702, 0.324) .. (0.702, 0.324)
	-- (0.702, 0.324) .. controls (0.702, 0.324) and (0.703, 0.324) .. (0.703, 0.324)
	-- (0.703, 0.324) .. controls (0.704, 0.324) and (0.704, 0.324) .. (0.704, 0.324)
	-- (0.704, 0.324) .. controls (0.705, 0.324) and (0.705, 0.324) .. (0.705, 0.324)
	-- (0.705, 0.324) .. controls (0.705, 0.324) and (0.706, 0.324) .. (0.706, 0.324)
	-- (0.706, 0.324) .. controls (0.707, 0.324) and (0.707, 0.324) .. (0.707, 0.324)
	-- (0.707, 0.324) .. controls (0.707, 0.324) and (0.708, 0.324) .. (0.708, 0.324)
	-- (0.708, 0.324) .. controls (0.709, 0.324) and (0.709, 0.324) .. (0.709, 0.324)
	-- (0.709, 0.324) .. controls (0.71, 0.324) and (0.71, 0.324) .. (0.71, 0.324)
	-- (0.71, 0.323) .. controls (0.71, 0.323) and (0.711, 0.323) .. (0.711, 0.323)
	-- (0.711, 0.323) .. controls (0.712, 0.323) and (0.712, 0.323) .. (0.712, 0.323)
	-- (0.712, 0.323) .. controls (0.713, 0.323) and (0.713, 0.323) .. (0.713, 0.323)
	-- (0.713, 0.323) .. controls (0.714, 0.323) and (0.714, 0.323) .. (0.714, 0.323)
	-- (0.714, 0.323) .. controls (0.714, 0.323) and (0.715, 0.323) .. (0.715, 0.323)
	-- (0.715, 0.323) .. controls (0.715, 0.323) and (0.716, 0.323) .. (0.716, 0.323)
	-- (0.716, 0.323) .. controls (0.716, 0.323) and (0.717, 0.323) .. (0.717, 0.323)
	-- (0.717, 0.323) .. controls (0.717, 0.323) and (0.717, 0.323) .. (0.718, 0.323)
	-- (0.718, 0.323) .. controls (0.719, 0.323) and (0.719, 0.323) .. (0.719, 0.323)
	-- (0.719, 0.323) .. controls (0.72, 0.323) and (0.72, 0.323) .. (0.72, 0.323)
	-- (0.72, 0.323) .. controls (0.72, 0.323) and (0.721, 0.323) .. (0.721, 0.323)
	-- (0.721, 0.323) .. controls (0.721, 0.323) and (0.721, 0.323) .. (0.722, 0.323)
	-- (0.722, 0.323) .. controls (0.723, 0.323) and (0.723, 0.323) .. (0.723, 0.323)
	-- (0.723, 0.323) .. controls (0.724, 0.323) and (0.724, 0.323) .. (0.724, 0.323)
	-- (0.724, 0.323) .. controls (0.724, 0.323) and (0.724, 0.323) .. (0.725, 0.323)
	-- (0.725, 0.323) .. controls (0.725, 0.323) and (0.726, 0.323) .. (0.726, 0.323)
	-- (0.726, 0.323) .. controls (0.726, 0.323) and (0.726, 0.323) .. (0.727, 0.323)
	-- (0.727, 0.323) .. controls (0.727, 0.323) and (0.727, 0.323) .. (0.728, 0.323)
	-- (0.728, 0.323) .. controls (0.728, 0.323) and (0.728, 0.323) .. (0.729, 0.323)
	-- (0.729, 0.323) .. controls (0.73, 0.323) and (0.73, 0.323) .. (0.73, 0.323)
	-- (0.73, 0.323) .. controls (0.73, 0.323) and (0.73, 0.323) .. (0.731, 0.323)
	-- (0.731, 0.323) .. controls (0.731, 0.323) and (0.732, 0.323) .. (0.732, 0.323)
	-- (0.732, 0.323) .. controls (0.733, 0.323) and (0.733, 0.323) .. (0.733, 0.323)
	-- (0.733, 0.323) .. controls (0.734, 0.323) and (0.734, 0.323) .. (0.734, 0.323)
	-- (0.734, 0.323) .. controls (0.734, 0.323) and (0.735, 0.323) .. (0.735, 0.323)
	-- (0.735, 0.322) .. controls (0.736, 0.322) and (0.736, 0.322) .. (0.736, 0.322)
	-- (0.736, 0.322) .. controls (0.737, 0.322) and (0.737, 0.322) .. (0.737, 0.322)
	-- (0.737, 0.322) .. controls (0.737, 0.322) and (0.737, 0.322) .. (0.738, 0.322)
	-- (0.738, 0.322) .. controls (0.739, 0.322) and (0.739, 0.322) .. (0.739, 0.322)
	-- (0.739, 0.322) .. controls (0.739, 0.322) and (0.739, 0.322) .. (0.74, 0.322)
	-- (0.74, 0.322) .. controls (0.74, 0.322) and (0.741, 0.322) .. (0.741, 0.322)
	-- (0.741, 0.322) .. controls (0.741, 0.322) and (0.741, 0.322) .. (0.742, 0.322)
	-- (0.742, 0.322) .. controls (0.742, 0.322) and (0.743, 0.322) .. (0.743, 0.322)
	-- (0.743, 0.322) .. controls (0.744, 0.322) and (0.744, 0.322) .. (0.744, 0.322)
	-- (0.744, 0.321) .. controls (0.745, 0.321) and (0.745, 0.321) .. (0.745, 0.321)
	-- (0.745, 0.321) .. controls (0.745, 0.321) and (0.745, 0.321) .. (0.746, 0.321)
	-- (0.746, 0.321) .. controls (0.746, 0.321) and (0.747, 0.321) .. (0.747, 0.321)
	-- (0.747, 0.321) .. controls (0.748, 0.321) and (0.748, 0.321) .. (0.748, 0.321)
	-- (0.748, 0.321) .. controls (0.748, 0.321) and (0.748, 0.321) .. (0.749, 0.321)
	-- (0.749, 0.321) .. controls (0.749, 0.321) and (0.749, 0.321) .. (0.75, 0.321)
	-- (0.75, 0.321) .. controls (0.751, 0.321) and (0.751, 0.321) .. (0.751, 0.321)
	-- (0.751, 0.322) .. controls (0.751, 0.322) and (0.751, 0.322) .. (0.752, 0.322)
	-- (0.752, 0.322) .. controls (0.752, 0.322) and (0.752, 0.322) .. (0.753, 0.322)
	-- (0.753, 0.322) .. controls (0.753, 0.322) and (0.753, 0.322) .. (0.754, 0.322)
	-- (0.754, 0.322) .. controls (0.755, 0.322) and (0.755, 0.322) .. (0.755, 0.322)
	-- (0.755, 0.322) .. controls (0.755, 0.322) and (0.755, 0.322) .. (0.756, 0.322)
	-- (0.756, 0.322) .. controls (0.757, 0.322) and (0.757, 0.322) .. (0.757, 0.322)
	-- (0.757, 0.322) .. controls (0.758, 0.322) and (0.758, 0.322) .. (0.758, 0.322)
	-- (0.758, 0.322) .. controls (0.758, 0.322) and (0.759, 0.322) .. (0.759, 0.322)
	-- (0.759, 0.322) .. controls (0.76, 0.322) and (0.76, 0.322) .. (0.76, 0.322)
	-- (0.76, 0.323) .. controls (0.76, 0.323) and (0.761, 0.323) .. (0.761, 0.323)
	-- (0.761, 0.323) .. controls (0.762, 0.323) and (0.762, 0.323) .. (0.762, 0.323)
	-- (0.762, 0.323) .. controls (0.762, 0.323) and (0.762, 0.323) .. (0.763, 0.323)
	-- (0.763, 0.323) .. controls (0.764, 0.323) and (0.764, 0.323) .. (0.764, 0.323)
	-- (0.764, 0.323) .. controls (0.764, 0.323) and (0.764, 0.323) .. (0.765, 0.323)
	-- (0.765, 0.323) .. controls (0.765, 0.323) and (0.765, 0.323) .. (0.766, 0.323)
	-- (0.766, 0.324) .. controls (0.767, 0.324) and (0.767, 0.324) .. (0.767, 0.324)
	-- (0.767, 0.324) .. controls (0.768, 0.324) and (0.768, 0.324) .. (0.768, 0.324)
	-- (0.768, 0.324) .. controls (0.769, 0.324) and (0.769, 0.324) .. (0.769, 0.324)
	-- (0.769, 0.324) .. controls (0.77, 0.324) and (0.77, 0.324) .. (0.77, 0.324)
	-- (0.77, 0.324) .. controls (0.77, 0.324) and (0.771, 0.324) .. (0.771, 0.324)
	-- (0.771, 0.324) .. controls (0.771, 0.324) and (0.771, 0.324) .. (0.772, 0.324)
	-- (0.772, 0.324) .. controls (0.773, 0.324) and (0.773, 0.324) .. (0.773, 0.324)
	-- (0.773, 0.325) .. controls (0.773, 0.325) and (0.774, 0.325) .. (0.774, 0.325)
	-- (0.774, 0.325) .. controls (0.775, 0.325) and (0.775, 0.325) .. (0.775, 0.325)
	-- (0.775, 0.325) .. controls (0.775, 0.325) and (0.776, 0.325) .. (0.776, 0.325)
	-- (0.776, 0.325) .. controls (0.776, 0.325) and (0.777, 0.325) .. (0.777, 0.325)
	-- (0.777, 0.325) .. controls (0.777, 0.325) and (0.778, 0.325) .. (0.778, 0.325)
	-- (0.778, 0.325) .. controls (0.778, 0.326) and (0.778, 0.326) .. (0.779, 0.326)
	-- (0.779, 0.326) .. controls (0.779, 0.326) and (0.779, 0.326) .. (0.78, 0.326)
	-- (0.78, 0.326) .. controls (0.781, 0.326) and (0.781, 0.326) .. (0.781, 0.326)
	-- (0.781, 0.326) .. controls (0.781, 0.326) and (0.781, 0.326) .. (0.782, 0.326)
	-- (0.782, 0.327) .. controls (0.783, 0.327) and (0.783, 0.327) .. (0.783, 0.327)
	-- (0.783, 0.327) .. controls (0.784, 0.327) and (0.784, 0.327) .. (0.784, 0.327)
	-- (0.784, 0.327) .. controls (0.784, 0.327) and (0.785, 0.327) .. (0.785, 0.327)
	-- (0.785, 0.328) .. controls (0.785, 0.328) and (0.786, 0.328) .. (0.786, 0.328)
	-- (0.786, 0.328) .. controls (0.786, 0.328) and (0.786, 0.328) .. (0.787, 0.328)
	-- (0.787, 0.328) .. controls (0.787, 0.328) and (0.787, 0.328) .. (0.788, 0.328)
	-- (0.788, 0.328) .. controls (0.788, 0.328) and (0.789, 0.328) .. (0.789, 0.328)
	-- (0.789, 0.329) .. controls (0.789, 0.329) and (0.79, 0.329) .. (0.79, 0.329)
	-- (0.79, 0.329) .. controls (0.79, 0.329) and (0.79, 0.329) .. (0.791, 0.329)
	-- (0.791, 0.329) .. controls (0.792, 0.329) and (0.792, 0.329) .. (0.792, 0.329)
	-- (0.792, 0.33) .. controls (0.792, 0.33) and (0.792, 0.33) .. (0.793, 0.33)
	-- (0.793, 0.33) .. controls (0.793, 0.33) and (0.793, 0.33) .. (0.794, 0.33)
	-- (0.794, 0.33) .. controls (0.795, 0.33) and (0.795, 0.33) .. (0.795, 0.33)
	-- (0.795, 0.33) .. controls (0.795, 0.33) and (0.796, 0.33) .. (0.796, 0.33)
	-- (0.796, 0.331) .. controls (0.796, 0.331) and (0.797, 0.331) .. (0.797, 0.331)
	-- (0.797, 0.331) .. controls (0.797, 0.331) and (0.797, 0.331) .. (0.798, 0.331)
	-- (0.798, 0.331) .. controls (0.798, 0.331) and (0.799, 0.331) .. (0.799, 0.331)
	-- (0.799, 0.331) .. controls (0.8, 0.331) and (0.8, 0.331) .. (0.8, 0.331)
	-- (0.8, 0.331) .. controls (0.8, 0.331) and (0.801, 0.331) .. (0.801, 0.331)
	-- (0.801, 0.332) .. controls (0.802, 0.332) and (0.802, 0.332) .. (0.802, 0.332)
	-- (0.802, 0.332) .. controls (0.802, 0.332) and (0.802, 0.332) .. (0.803, 0.332)
	-- (0.803, 0.332) .. controls (0.804, 0.332) and (0.804, 0.332) .. (0.804, 0.332)
	-- (0.804, 0.332) .. controls (0.804, 0.332) and (0.804, 0.332) .. (0.805, 0.332)
	-- (0.805, 0.332) .. controls (0.806, 0.332) and (0.806, 0.332) .. (0.806, 0.332)
	-- (0.806, 0.333) .. controls (0.806, 0.333) and (0.806, 0.333) .. (0.807, 0.333)
	-- (0.807, 0.333) .. controls (0.807, 0.333) and (0.807, 0.333) .. (0.808, 0.333)
	-- (0.808, 0.333) .. controls (0.808, 0.333) and (0.808, 0.333) .. (0.809, 0.333)
	-- (0.809, 0.333) .. controls (0.809, 0.333) and (0.81, 0.333) .. (0.81, 0.333)
	-- (0.81, 0.333) .. controls (0.81, 0.333) and (0.81, 0.333) .. (0.811, 0.333)
	-- (0.811, 0.333) .. controls (0.812, 0.333) and (0.812, 0.333) .. (0.812, 0.333)
	-- (0.812, 0.333) .. controls (0.813, 0.333) and (0.813, 0.333) .. (0.813, 0.333)
	-- (0.813, 0.333) .. controls (0.813, 0.333) and (0.814, 0.333) .. (0.814, 0.333)
	-- (0.814, 0.333) .. controls (0.815, 0.333) and (0.815, 0.333) .. (0.815, 0.333)
	-- (0.815, 0.334) .. controls (0.816, 0.334) and (0.816, 0.334) .. (0.816, 0.334)
	-- (0.816, 0.334) .. controls (0.816, 0.334) and (0.817, 0.334) .. (0.817, 0.334)
	-- (0.817, 0.334) .. controls (0.817, 0.334) and (0.817, 0.334) .. (0.818, 0.334)
	-- (0.818, 0.334) .. controls (0.818, 0.334) and (0.819, 0.334) .. (0.819, 0.334)
	-- (0.819, 0.335) .. controls (0.819, 0.335) and (0.819, 0.335) .. (0.82, 0.335)
	-- (0.82, 0.335) .. controls (0.82, 0.335) and (0.82, 0.335) .. (0.821, 0.335)
	-- (0.821, 0.335) .. controls (0.821, 0.335) and (0.821, 0.335) .. (0.822, 0.335)
	-- (0.822, 0.335) .. controls (0.823, 0.335) and (0.823, 0.335) .. (0.823, 0.335)
	-- (0.823, 0.335) .. controls (0.823, 0.335) and (0.823, 0.335) .. (0.824, 0.335)
	-- (0.824, 0.335) .. controls (0.825, 0.335) and (0.825, 0.335) .. (0.825, 0.335)
	-- (0.825, 0.335) .. controls (0.825, 0.335) and (0.825, 0.335) .. (0.826, 0.335)
	-- (0.826, 0.335) .. controls (0.826, 0.335) and (0.826, 0.335) .. (0.827, 0.335)
	-- (0.827, 0.335) .. controls (0.827, 0.335) and (0.827, 0.335) .. (0.828, 0.335)
	-- (0.828, 0.336) .. controls (0.828, 0.336) and (0.828, 0.336) .. (0.829, 0.336)
	-- (0.829, 0.336) .. controls (0.83, 0.336) and (0.83, 0.336) .. (0.83, 0.336)
	-- (0.83, 0.336) .. controls (0.83, 0.336) and (0.83, 0.336) .. (0.831, 0.336)
	-- (0.831, 0.336) .. controls (0.831, 0.336) and (0.832, 0.336) .. (0.832, 0.336)
	-- (0.832, 0.336) .. controls (0.833, 0.336) and (0.833, 0.336) .. (0.833, 0.336)
	-- (0.833, 0.336) .. controls (0.834, 0.336) and (0.834, 0.336) .. (0.834, 0.336)
	-- (0.834, 0.337) .. controls (0.835, 0.337) and (0.835, 0.337) .. (0.835, 0.337)
	-- (0.835, 0.337) .. controls (0.836, 0.337) and (0.836, 0.337) .. (0.836, 0.337)
	-- (0.836, 0.337) .. controls (0.837, 0.337) and (0.837, 0.337) .. (0.837, 0.337)
	-- (0.837, 0.338) .. controls (0.838, 0.338) and (0.838, 0.338) .. (0.838, 0.338)
	-- (0.838, 0.338) .. controls (0.838, 0.338) and (0.838, 0.338) .. (0.839, 0.338)
	-- (0.839, 0.338) .. controls (0.839, 0.338) and (0.84, 0.338) .. (0.84, 0.338)
	-- (0.84, 0.339) .. controls (0.84, 0.339) and (0.84, 0.339) .. (0.841, 0.339)
	-- (0.841, 0.339) .. controls (0.841, 0.339) and (0.841, 0.339) .. (0.842, 0.339)
	-- (0.842, 0.339) .. controls (0.843, 0.339) and (0.843, 0.339) .. (0.843, 0.339)
	-- (0.843, 0.34) .. controls (0.843, 0.34) and (0.843, 0.34) .. (0.844, 0.34)
	-- (0.844, 0.34) .. controls (0.844, 0.34) and (0.845, 0.34) .. (0.845, 0.34)
	-- (0.845, 0.341) .. controls (0.845, 0.341) and (0.846, 0.341) .. (0.846, 0.341)
	-- (0.846, 0.341) .. controls (0.847, 0.341) and (0.847, 0.341) .. (0.847, 0.341)
	-- (0.847, 0.341) .. controls (0.847, 0.341) and (0.848, 0.341) .. (0.848, 0.341)
	-- (0.848, 0.341) .. controls (0.848, 0.341) and (0.848, 0.341) .. (0.849, 0.341)
	-- (0.849, 0.342) .. controls (0.849, 0.342) and (0.85, 0.342) .. (0.85, 0.342)
	-- (0.85, 0.342) .. controls (0.85, 0.342) and (0.85, 0.342) .. (0.851, 0.342)
	-- (0.851, 0.342) .. controls (0.852, 0.342) and (0.852, 0.342) .. (0.852, 0.342)
	-- (0.852, 0.343) .. controls (0.853, 0.343) and (0.853, 0.343) .. (0.853, 0.343)
	-- (0.853, 0.343) .. controls (0.853, 0.343) and (0.854, 0.343) .. (0.854, 0.343)
	-- (0.854, 0.343) .. controls (0.855, 0.343) and (0.855, 0.343) .. (0.855, 0.343)
	-- (0.855, 0.343) .. controls (0.856, 0.343) and (0.856, 0.343) .. (0.856, 0.343)
	-- (0.856, 0.343) .. controls (0.856, 0.343) and (0.856, 0.344) .. (0.857, 0.344)
	-- (0.857, 0.344) .. controls (0.857, 0.344) and (0.858, 0.344) .. (0.858, 0.344)
	-- (0.858, 0.344) .. controls (0.858, 0.344) and (0.859, 0.344) .. (0.859, 0.344)
	-- (0.859, 0.344) .. controls (0.86, 0.344) and (0.86, 0.344) .. (0.86, 0.344)
	-- (0.86, 0.345) .. controls (0.86, 0.345) and (0.86, 0.345) .. (0.861, 0.345)
	-- (0.861, 0.345) .. controls (0.861, 0.345) and (0.862, 0.345) .. (0.862, 0.345)
	-- (0.862, 0.345) .. controls (0.862, 0.345) and (0.863, 0.345) .. (0.863, 0.345)
	-- (0.863, 0.345) .. controls (0.863, 0.345) and (0.864, 0.345) .. (0.864, 0.345)
	-- (0.864, 0.345) .. controls (0.864, 0.345) and (0.864, 0.346) .. (0.865, 0.346)
	-- (0.865, 0.346) .. controls (0.866, 0.346) and (0.866, 0.346) .. (0.866, 0.346)
	-- (0.866, 0.346) .. controls (0.866, 0.346) and (0.866, 0.346) .. (0.867, 0.346)
	-- (0.867, 0.346) .. controls (0.867, 0.346) and (0.867, 0.346) .. (0.868, 0.346)
	-- (0.868, 0.346) .. controls (0.868, 0.346) and (0.868, 0.346) .. (0.869, 0.346)
	-- (0.869, 0.346) .. controls (0.87, 0.346) and (0.87, 0.346) .. (0.87, 0.346)
	-- (0.87, 0.346) .. controls (0.871, 0.346) and (0.871, 0.346) .. (0.871, 0.346)
	-- (0.871, 0.346) .. controls (0.872, 0.346) and (0.872, 0.346) .. (0.872, 0.346)
	-- (0.872, 0.346) .. controls (0.873, 0.346) and (0.873, 0.346) .. (0.873, 0.346)
	-- (0.873, 0.346) .. controls (0.873, 0.346) and (0.873, 0.346) .. (0.874, 0.346)
	-- (0.874, 0.347) .. controls (0.874, 0.347) and (0.874, 0.347) .. (0.875, 0.347)
	-- (0.875, 0.347) .. controls (0.875, 0.347) and (0.875, 0.347) .. (0.876, 0.347)
	-- (0.876, 0.347) .. controls (0.876, 0.347) and (0.877, 0.347) .. (0.877, 0.347)
	-- (0.877, 0.347) .. controls (0.877, 0.347) and (0.878, 0.347) .. (0.878, 0.347)
	-- (0.878, 0.348) .. controls (0.878, 0.348) and (0.878, 0.348) .. (0.879, 0.348)
	-- (0.879, 0.348) .. controls (0.879, 0.348) and (0.879, 0.348) .. (0.88, 0.348)
	-- (0.88, 0.348) .. controls (0.88, 0.348) and (0.88, 0.348) .. (0.881, 0.348)
	-- (0.881, 0.348) .. controls (0.881, 0.348) and (0.881, 0.348) .. (0.882, 0.348)
	-- (0.882, 0.348) .. controls (0.882, 0.348) and (0.882, 0.348) .. (0.883, 0.348)
	-- (0.883, 0.349) .. controls (0.884, 0.349) and (0.884, 0.349) .. (0.884, 0.349)
	-- (0.884, 0.349) .. controls (0.884, 0.349) and (0.884, 0.349) .. (0.885, 0.349)
	-- (0.885, 0.349) .. controls (0.885, 0.349) and (0.886, 0.349) .. (0.886, 0.349)
	-- (0.886, 0.349) .. controls (0.886, 0.349) and (0.886, 0.349) .. (0.887, 0.349)
	-- (0.887, 0.349) .. controls (0.887, 0.349) and (0.887, 0.349) .. (0.888, 0.349)
	-- (0.888, 0.35) .. controls (0.888, 0.35) and (0.889, 0.35) .. (0.889, 0.35)
	-- (0.889, 0.35) .. controls (0.89, 0.35) and (0.89, 0.35) .. (0.89, 0.35)
	-- (0.89, 0.35) .. controls (0.89, 0.35) and (0.891, 0.35) .. (0.891, 0.35)
	-- (0.891, 0.351) .. controls (0.891, 0.351) and (0.891, 0.351) .. (0.892, 0.351)
	-- (0.892, 0.352) .. controls (0.892, 0.352) and (0.893, 0.352) .. (0.893, 0.352)
	-- (0.893, 0.352) .. controls (0.893, 0.352) and (0.894, 0.352) .. (0.894, 0.352)
	-- (0.894, 0.353) .. controls (0.895, 0.353) and (0.895, 0.353) .. (0.895, 0.353)
	-- (0.895, 0.353) .. controls (0.895, 0.353) and (0.896, 0.353) .. (0.896, 0.353)
	-- (0.896, 0.353) .. controls (0.897, 0.353) and (0.897, 0.353) .. (0.897, 0.353)
	-- (0.897, 0.353) .. controls (0.897, 0.353) and (0.898, 0.353) .. (0.898, 0.353)
	-- (0.898, 0.353) .. controls (0.898, 0.354) and (0.898, 0.354) .. (0.899, 0.354)
	-- (0.899, 0.354) .. controls (0.899, 0.354) and (0.9, 0.354) .. (0.9, 0.354)
	-- (0.9, 0.354) .. controls (0.901, 0.354) and (0.901, 0.354) .. (0.901, 0.354)
	-- (0.901, 0.354) .. controls (0.902, 0.354) and (0.902, 0.354) .. (0.902, 0.354)
	-- (0.902, 0.354) .. controls (0.902, 0.354) and (0.903, 0.354) .. (0.903, 0.354)
	-- (0.903, 0.354) .. controls (0.903, 0.354) and (0.903, 0.354) .. (0.904, 0.354)
	-- (0.904, 0.353) .. controls (0.905, 0.353) and (0.905, 0.353) .. (0.905, 0.353)
	-- (0.905, 0.353) .. controls (0.905, 0.353) and (0.906, 0.353) .. (0.906, 0.353)
	-- (0.906, 0.353) .. controls (0.906, 0.353) and (0.907, 0.353) .. (0.907, 0.353)
	-- (0.907, 0.353) .. controls (0.908, 0.353) and (0.908, 0.353) .. (0.908, 0.353)
	-- (0.908, 0.353) .. controls (0.909, 0.353) and (0.909, 0.353) .. (0.909, 0.353)
	-- (0.909, 0.353) .. controls (0.909, 0.353) and (0.909, 0.353) .. (0.91, 0.353)
	-- (0.91, 0.353) .. controls (0.91, 0.353) and (0.91, 0.353) .. (0.911, 0.353)
	-- (0.911, 0.353) .. controls (0.912, 0.353) and (0.912, 0.353) .. (0.912, 0.353)
	-- (0.912, 0.353) .. controls (0.913, 0.353) and (0.913, 0.353) .. (0.913, 0.352)
	-- (0.913, 0.352) .. controls (0.913, 0.352) and (0.913, 0.352) .. (0.914, 0.352)
	-- (0.914, 0.352) .. controls (0.914, 0.352) and (0.914, 0.352) .. (0.915, 0.352)
	-- (0.915, 0.352) .. controls (0.915, 0.352) and (0.915, 0.352) .. (0.916, 0.352)
	-- (0.916, 0.351) .. controls (0.917, 0.351) and (0.917, 0.351) .. (0.917, 0.351)
	-- (0.917, 0.352) .. controls (0.918, 0.352) and (0.918, 0.352) .. (0.918, 0.352)
	-- (0.918, 0.352) .. controls (0.918, 0.352) and (0.918, 0.352) .. (0.919, 0.352)
	-- (0.919, 0.352) .. controls (0.919, 0.352) and (0.919, 0.352) .. (0.92, 0.352)
	-- (0.92, 0.351) .. controls (0.92, 0.351) and (0.92, 0.351) .. (0.921, 0.351)
	-- (0.921, 0.351) .. controls (0.922, 0.351) and (0.922, 0.351) .. (0.922, 0.351)
	-- (0.922, 0.351) .. controls (0.923, 0.351) and (0.923, 0.351) .. (0.923, 0.351)
	-- (0.923, 0.351) .. controls (0.924, 0.351) and (0.924, 0.351) .. (0.924, 0.351)
	-- (0.924, 0.351) .. controls (0.924, 0.351) and (0.925, 0.351) .. (0.925, 0.351)
	-- (0.925, 0.351) .. controls (0.925, 0.351) and (0.925, 0.351) .. (0.926, 0.351)
	-- (0.926, 0.351) .. controls (0.927, 0.351) and (0.927, 0.351) .. (0.927, 0.351)
	-- (0.927, 0.351) .. controls (0.927, 0.351) and (0.927, 0.351) .. (0.928, 0.351)
	-- (0.928, 0.35) .. controls (0.928, 0.35) and (0.928, 0.35) .. (0.929, 0.35)
	-- (0.929, 0.35) .. controls (0.929, 0.35) and (0.929, 0.35) .. (0.93, 0.35)
	-- (0.93, 0.35) .. controls (0.93, 0.35) and (0.93, 0.35) .. (0.931, 0.35)
	-- (0.931, 0.349) .. controls (0.932, 0.349) and (0.932, 0.349) .. (0.932, 0.349)
	-- (0.932, 0.349) .. controls (0.933, 0.349) and (0.933, 0.349) .. (0.933, 0.349)
	-- (0.933, 0.349) .. controls (0.934, 0.349) and (0.934, 0.349) .. (0.934, 0.349)
	-- (0.934, 0.348) .. controls (0.934, 0.348) and (0.935, 0.348) .. (0.935, 0.348)
	-- (0.935, 0.348) .. controls (0.935, 0.348) and (0.935, 0.348) .. (0.936, 0.348)
	-- (0.936, 0.347) .. controls (0.937, 0.347) and (0.937, 0.347) .. (0.937, 0.347)
	-- (0.937, 0.347) .. controls (0.937, 0.347) and (0.937, 0.347) .. (0.938, 0.347)
	-- (0.938, 0.346) .. controls (0.939, 0.346) and (0.939, 0.346) .. (0.939, 0.346)
	-- (0.939, 0.345) .. controls (0.94, 0.345) and (0.94, 0.345) .. (0.94, 0.345)
	-- (0.94, 0.345) .. controls (0.94, 0.345) and (0.941, 0.345) .. (0.941, 0.345)
	-- (0.941, 0.344) .. controls (0.941, 0.344) and (0.942, 0.344) .. (0.942, 0.344)
	-- (0.942, 0.344) .. controls (0.942, 0.344) and (0.943, 0.344) .. (0.943, 0.344)
	-- (0.943, 0.343) .. controls (0.943, 0.343) and (0.944, 0.343) .. (0.944, 0.343)
	-- (0.944, 0.343) .. controls (0.944, 0.343) and (0.944, 0.343) .. (0.945, 0.343)
	-- (0.945, 0.343) .. controls (0.946, 0.343) and (0.946, 0.343) .. (0.946, 0.343)
	-- (0.946, 0.342) .. controls (0.947, 0.342) and (0.947, 0.342) .. (0.947, 0.342)
	-- (0.947, 0.342) .. controls (0.947, 0.342) and (0.948, 0.342) .. (0.948, 0.342)
	-- (0.948, 0.342) .. controls (0.948, 0.342) and (0.948, 0.342) .. (0.949, 0.342)
	-- (0.949, 0.341) .. controls (0.949, 0.341) and (0.949, 0.341) .. (0.95, 0.341)
	-- (0.95, 0.341) .. controls (0.951, 0.341) and (0.951, 0.341) .. (0.951, 0.341)
	-- (0.951, 0.34) .. controls (0.951, 0.34) and (0.952, 0.34) .. (0.952, 0.34)
	-- (0.952, 0.34) .. controls (0.952, 0.34) and (0.953, 0.34) .. (0.953, 0.34)
	-- (0.953, 0.339) .. controls (0.953, 0.339) and (0.953, 0.339) .. (0.954, 0.339)
	-- (0.954, 0.339) .. controls (0.954, 0.339) and (0.954, 0.339) .. (0.955, 0.339)
	-- (0.955, 0.339) .. controls (0.956, 0.339) and (0.956, 0.339) .. (0.956, 0.339)
	-- (0.956, 0.338) .. controls (0.956, 0.338) and (0.956, 0.338) .. (0.957, 0.338)
	-- (0.957, 0.338) .. controls (0.957, 0.338) and (0.958, 0.338) .. (0.958, 0.338)
	-- (0.958, 0.338) .. controls (0.958, 0.338) and (0.958, 0.338) .. (0.959, 0.337)
	-- (0.959, 0.337) .. controls (0.96, 0.337) and (0.96, 0.337) .. (0.96, 0.337)
	-- (0.96, 0.337) .. controls (0.96, 0.337) and (0.96, 0.337) .. (0.961, 0.337)
	-- (0.961, 0.337) .. controls (0.962, 0.337) and (0.962, 0.337) .. (0.962, 0.337)
	-- (0.962, 0.336) .. controls (0.963, 0.336) and (0.963, 0.336) .. (0.963, 0.336)
	-- (0.963, 0.336) .. controls (0.963, 0.336) and (0.963, 0.336) .. (0.964, 0.336)
	-- (0.964, 0.336) .. controls (0.965, 0.336) and (0.965, 0.336) .. (0.965, 0.336)
	-- (0.965, 0.335) .. controls (0.966, 0.335) and (0.966, 0.335) .. (0.966, 0.335)
	-- (0.966, 0.335) .. controls (0.966, 0.335) and (0.967, 0.335) .. (0.967, 0.335)
	-- (0.967, 0.335) .. controls (0.967, 0.335) and (0.968, 0.335) .. (0.968, 0.335)
	-- (0.968, 0.335) .. controls (0.968, 0.335) and (0.969, 0.335) .. (0.969, 0.335)
	-- (0.969, 0.335) .. controls (0.969, 0.335) and (0.97, 0.335) .. (0.97, 0.335)
	-- (0.97, 0.335) .. controls (0.97, 0.335) and (0.971, 0.335) .. (0.971, 0.335)
	-- (0.971, 0.335) .. controls (0.972, 0.335) and (0.972, 0.335) .. (0.972, 0.335)
	-- (0.972, 0.334) .. controls (0.972, 0.334) and (0.972, 0.334) .. (0.973, 0.334)
	-- (0.973, 0.334) .. controls (0.973, 0.334) and (0.974, 0.334) .. (0.974, 0.334)
	-- (0.974, 0.335) .. controls (0.974, 0.335) and (0.975, 0.335) .. (0.975, 0.335)
	-- (0.975, 0.335) .. controls (0.975, 0.335) and (0.975, 0.335) .. (0.976, 0.335)
	-- (0.976, 0.335) .. controls (0.976, 0.335) and (0.977, 0.335) .. (0.977, 0.335)
	-- (0.977, 0.335) .. controls (0.977, 0.335) and (0.977, 0.335) .. (0.978, 0.335)
	-- (0.978, 0.335) .. controls (0.978, 0.335) and (0.978, 0.335) .. (0.979, 0.335)
	-- (0.979, 0.335) .. controls (0.979, 0.335) and (0.98, 0.335) .. (0.98, 0.335)
	-- (0.98, 0.335) .. controls (0.98, 0.335) and (0.98, 0.335) .. (0.981, 0.335)
	-- (0.981, 0.335) .. controls (0.981, 0.335) and (0.982, 0.335) .. (0.982, 0.335)
	-- (0.982, 0.335) .. controls (0.982, 0.335) and (0.982, 0.335) .. (0.983, 0.335)
	-- (0.983, 0.336) .. controls (0.983, 0.336) and (0.984, 0.336) .. (0.984, 0.336)
	-- (0.984, 0.336) .. controls (0.984, 0.336) and (0.985, 0.336) .. (0.985, 0.336)
	-- (0.985, 0.336) .. controls (0.986, 0.336) and (0.986, 0.336) .. (0.986, 0.336)
	-- (0.986, 0.336) .. controls (0.987, 0.336) and (0.987, 0.336) .. (0.987, 0.336)
	-- (0.987, 0.336) .. controls (0.987, 0.336) and (0.987, 0.336) .. (0.988, 0.336)
	-- (0.988, 0.336) .. controls (0.988, 0.336) and (0.989, 0.336) .. (0.989, 0.336)
	-- (0.989, 0.337) .. controls (0.989, 0.337) and (0.989, 0.337) .. (0.99, 0.337)
	-- (0.99, 0.337) .. controls (0.99, 0.337) and (0.991, 0.337) .. (0.991, 0.337)
	-- (0.991, 0.337) .. controls (0.991, 0.337) and (0.992, 0.337) .. (0.992, 0.337)
	-- (0.992, 0.337) .. controls (0.992, 0.337) and (0.993, 0.337) .. (0.993, 0.337)
	-- (0.993, 0.337) .. controls (0.993, 0.337) and (0.993, 0.337) .. (0.994, 0.337)
	-- (0.994, 0.337) .. controls (0.994, 0.337) and (0.994, 0.337) .. (0.995, 0.337)
	-- (0.995, 0.337) .. controls (0.995, 0.337) and (0.995, 0.337) .. (0.996, 0.337)
	-- (0.996, 0.337) .. controls (0.996, 0.337) and (0.997, 0.337) .. (0.997, 0.337)
	-- (0.997, 0.337) .. controls (0.998, 0.337) and (0.998, 0.337) .. (0.998, 0.337)
	-- (0.998, 0.337) .. controls (0.998, 0.337) and (0.998, 0.337) .. (0.999, 0.337)
	-- (0.999, 0.337) .. controls (1.0, 0.337) and (1.0, 0.337) .. (1.0, 0.337)
	;


==> figure/riboflavin/plot.tex <==
\input mac/m

\definecolor{cat1}{RGB}{0, 114, 190}
\definecolor{cat2}{RGB}{218, 83, 25}

\tikzpicture[xscale=12, yscale=1.2]
  % \draw[very thin,color=gray, xstep=.08, ystep=.2] (-0.01,-2.52) grid (1.01,1.01);

  % \draw[->] (-0.02,0) -- (1.02,0) node[right] {$x$};
  \def\yaxis{-0.025}
  % \def\xaxis{-2.65}
  \def\xaxis{-3.5}
  \def\ticksize{.1cm}
  \def\xtick{\ticksize/12}
  \def\ytick{\ticksize/1.2}

  \draw (\yaxis,-3.0) -- (\yaxis, 1.0);
  \draw (0, \xaxis) -- (1, \xaxis);

  \draw[very thin, color=gray] (\yaxis, 0) node[left, color=black]{\sevenpoint$0$} -- (1, 0);

  \draw[dotted, thick] (0.226, \xaxis) node[below, color=black]{\sevenpoint\kern-1em$0.226$ \rlap{early stopping point}} -- (0.226, 0.240)
          -- (\yaxis, 0.240) node[left, color=black]{\sevenpoint$0.240$};

  \draw[dotted, thick] (0.25, \xaxis)  -- (0.25, 0.23);

  \scope[color=cat1, semithick]
  \input figure/riboflavin/lo-cmd
  \endscope

  \scope[color=cat2, semithick]
  \clip (.1, -3) rectangle (1, 1);
  \input figure/riboflavin/lo-d-cmd
  \endscope

  \foreach \y in {-3, 1}
    \draw (\yaxis, \y) node[left]{\sevenpoint$\y$} -- +(\xtick, 0);

  \foreach \x in {0, 0.5, 1}
    \draw (\x, \xaxis) node[below]{\sevenpoint$\x$} -- +(0, \ytick);

% Figure Labels
\draw (.6, .7) node[color=cat1]{LO};
\draw (.66, -.4) node[color=cat2]{LO Derivative};
\draw (0.52, \xaxis-.7) node{\sevenpoint$t / \sum_{j=1}^p |\hat{\beta}_j^{\rm OLS}|$};

\endtikzpicture

\subend


==> mac/bib.tex <==
\def\citewishart{1} % Anderson
\def\citecvsurvey{2} % Arlot
\def\citeloci{3} % Bayle
\def\citeriboflavin{4} % Buhlmann
\def\citecv{5} % Burman
\def\citelars{6} % Efron
\def\citegeo{7} % Fadil
\def\citematrix{8} % Golub
\def\citegcv{9} % Golub, Heath
\def\citeriboflavinfirst{10} % Lee
\def\citelarslike{11} % Osborne
\def\citealo{12} % Rad, Maleki
\def\citelop{13} % Rad, Zhou
\def\citerobotsrc{14} % Rasmussen
\def\citeconvex{15} % Rockafellar
\def\citesparse{16} % Rosset
\def\citeseismology{17} % Stein
\def\citelasso{18} % Tibshirani
\def\citeunique{19} % Tibshirani
\def\citegenerallasso{20} % Tibshirani, Taylor
\def\citerobotarm{21} % Vijayakumar
\def\citealop{22} % Wang
\def\citelo{23} % Zou


==> mac/fonts.tex <==
% List available fonts:
%    mtxrun --script fonts --list --all

\font\header=cmb10 scaled \magstephalf

\font\ninerm=cmr9
\font\eightrm=cmr8
\font\sixrm=cmr6

\font\ninei=cmmi9
\font\eighti=cmmi8
\font\sixi=cmmi6
\skewchar\ninei='177 \skewchar\eighti='177 \skewchar\sixi='177

\font\ninesy=cmsy9
\font\eightsy=cmsy8
\font\sixsy=cmsy6
\skewchar\ninesy='60 \skewchar\eightsy='60 \skewchar\sixsy='60

\font\eightss=cmssq8

\font\eightssi=cmssqi8

\font\ninebf=cmbx9
\font\eightbf=cmbx8
\font\sixbf=cmbx6

\font\ninett=cmtt9
\font\eighttt=cmtt8
\font\seventt=cmtt8

\hyphenchar\tentt=-1 % inhibit hyphenation in typewriter type
\hyphenchar\ninett=-1
\hyphenchar\eighttt=-1
\hyphenchar\seventt=-1

\font\tencmmib=cmmib10  
\font\ninecmmib=cmmib9  
\font\eightcmmib=cmmib8  
\font\sevencmmib=cmmib7
\font\sixcmmib=cmmib6
\font\fivecmmib=cmmib5
\skewchar\tencmmib='177 \skewchar\ninecmmib='177 \skewchar\eightcmmib='177 \skewchar\sevencmmib='177

\newfam\bfit
\textfont\bfit=\tencmmib \scriptfont\bfit=\sevencmmib
  \scriptscriptfont\bfit=\fivecmmib

\font\ninesl=cmsl9
\font\eightsl=cmsl8
\font\sevensl=cmsl8

\font\nineit=cmti9
\font\eightit=cmti8
\font\sevenit=cmti7

\font\tenu=cmu10 % unslanted text italic
\font\magnifiedfiverm=cmr5 at 10pt
\font\cmman=cmman % font used for miscellaneous Computer Modern variations

\font\tenamsb=msbm10
\newfam\bbfam
\textfont\bbfam\tenamsb
\def\bbb{\fam\bbfam}

\newskip\ttglue
\def\tenpoint{\def\rm{\fam0\tenrm}%
  \textfont0=\tenrm \scriptfont0=\sevenrm \scriptscriptfont0=\fiverm
  \textfont1=\teni \scriptfont1=\seveni \scriptscriptfont1=\fivei
  \textfont2=\tensy \scriptfont2=\sevensy \scriptscriptfont2=\fivesy
  \textfont3=\tenex \scriptfont3=\tenex \scriptscriptfont3=\tenex
  \textfont7=\tentt \scriptfont7=\seventt \scriptscriptfont7=\seventt
  \textfont\bfit=\tencmmib \scriptfont\bfit=\sevencmmib
    \scriptscriptfont\bfit=\fivecmmib

  \def\it{\fam\itfam\tenit}%
  \textfont\itfam=\tenit
  \def\sl{\fam\slfam\tensl}%
  \textfont\slfam=\tensl
  \def\bf{\fam\bffam\tenbf}%
  \textfont\bffam=\tenbf \scriptfont\bffam=\sevenbf
   \scriptscriptfont\bffam=\fivebf
  \def\tt{\fam\ttfam\tentt}%
  \textfont\ttfam=\tentt
  \tt \ttglue=.5em plus.25em minus.15em
  \normalbaselineskip=12pt
  \let\sc=\eightrm
  \let\big=\tenbig
  \setbox\strutbox=\hbox{\vrule height8.5pt depth3.5pt width\z@}%
  \normalbaselines\rm}

\def\ninepoint{\def\rm{\fam0\ninerm}%
  \textfont0=\ninerm \scriptfont0=\sixrm \scriptscriptfont0=\fiverm
  \textfont1=\ninei \scriptfont1=\seveni \scriptscriptfont1=\fivei
  \textfont2=\ninesy \scriptfont2=\sixsy \scriptscriptfont2=\fivesy
  \textfont3=\tenex \scriptfont3=\tenex \scriptscriptfont3=\tenex

  \textfont\bfit=\ninecmmib \scriptfont\bfit=\sixcmmib
    \scriptscriptfont\bfit=\fivecmmib

  \def\it{\fam\itfam\nineit}%
  \textfont\itfam=\nineit
  \def\sl{\fam\slfam\ninesl}%
  \textfont\slfam=\ninesl
  \def\bf{\fam\bffam\ninebf}%
  \textfont\bffam=\ninebf \scriptfont\bffam=\sixbf
   \scriptscriptfont\bffam=\fivebf
  \def\tt{\fam\ttfam\ninett}%
  \textfont\ttfam=\ninett
  \tt \ttglue=.5em plus.25em minus.15em
  \normalbaselineskip=11pt
  \let\sc=\sevenrm
  \let\big=\ninebig
  \setbox\strutbox=\hbox{\vrule height8pt depth3pt width\z@}%
  \normalbaselines\rm}

\def\eightpoint{\def\rm{\fam0\eightrm}%
  \textfont0=\eightrm \scriptfont0=\sixrm \scriptscriptfont0=\fiverm
  \textfont1=\eighti \scriptfont1=\seveni \scriptscriptfont1=\fivei
  \textfont2=\eightsy \scriptfont2=\sixsy \scriptscriptfont2=\fivesy
  \textfont3=\tenex \scriptfont3=\tenex \scriptscriptfont3=\tenex

  \textfont\bfit=\eightcmmib \scriptfont\bfit=\sixcmmib
    \scriptscriptfont\bfit=\fivecmmib

  \def\it{\fam\itfam\eightit}%
  \textfont\itfam=\eightit
  \def\sl{\fam\slfam\eightsl}%
  \textfont\slfam=\eightsl
  \def\bf{\fam\bffam\eightbf}%
  \textfont\bffam=\eightbf \scriptfont\bffam=\sixbf
   \scriptscriptfont\bffam=\fivebf
  \def\tt{\fam\ttfam\eighttt}%
  \textfont\ttfam=\eighttt
  \tt \ttglue=.5em plus.25em minus.15em
  \normalbaselineskip=9pt
  \let\sc=\sixrm
  \let\big=\eightbig
  \setbox\strutbox=\hbox{\vrule height7pt depth2pt width\z@}%
  \normalbaselines\rm}

\def\sevenpoint{\def\rm{\fam0\sevenrm}%
  \textfont0=\sevenrm \scriptfont0=\sixrm \scriptscriptfont0=\fiverm
  \textfont1=\seveni \scriptfont1=\seveni \scriptscriptfont1=\fivei
  \textfont2=\sevensy \scriptfont2=\sixsy \scriptscriptfont2=\fivesy
  \textfont3=\tenex \scriptfont3=\tenex \scriptscriptfont3=\tenex

  \textfont\bfit=\sevencmmib \scriptfont\bfit=\fivecmmib
    \scriptscriptfont\bfit=\fivecmmib

  \def\it{\fam\itfam\sevenit}%
  \textfont\itfam=\sevenit
  \def\sl{\fam\slfam\sevensl}%
  \textfont\slfam=\sevensl
  \def\bf{\fam\bffam\sevenbf}%
  \textfont\bffam=\sevenbf \scriptfont\bffam=\sixbf
   \scriptscriptfont\bffam=\fivebf
  \def\tt{\fam\ttfam\seventt}%
  \textfont\ttfam=\seventt
  \tt \ttglue=.5em plus.25em minus.15em
  \normalbaselineskip=8pt
  \let\sc=\sixrm
  \let\big=\sevenbig
  \setbox\strutbox=\hbox{\vrule height6pt depth1pt width\z@}%
  \normalbaselines\rm}

\def\tenmath{\tenpoint\fam-1 } % use after $ in ninepoint sections
\def\tenbig#1{{\hbox{$\left#1\vbox to8.5pt{}\right.\n@space$}}}
\def\ninebig#1{{\hbox{$\textfont0=\tenrm\textfont2=\tensy
  \left#1\vbox to7.25pt{}\right.\n@space$}}}
\def\eightbig#1{{\hbox{$\textfont0=\ninerm\textfont2=\ninesy
  \left#1\vbox to6.5pt{}\right.\n@space$}}}

\mathchardef\betap="710C
\mathchardef\gammap="710D


==> mac/layout.tex <==
\pdfpagewidth=8.5in
\pdfpageheight=11in

\newdimen\leftmargin
\leftmargin=.75in

\newdimen\textwidth
\textwidth=5.5in

\newdimen\rightbuffer
\rightbuffer=.3in

\newdimen\rightskipwidth
\rightskipwidth=\pdfpagewidth
\advance \rightskipwidth by -\rightbuffer
\advance \rightskipwidth by -\textwidth
\advance \rightskipwidth by -\leftmargin
\rightskip=\rightskipwidth plus 4pt minus 4pt

\leftskip=\rightskipwidth plus 0pt minus 0pt
\hoffset=-\rightskip
\advance\hoffset by \leftmargin

\hsize=\pdfpagewidth
\advance\hsize by -\rightbuffer
\advance\hsize by -\hoffset
\advance\hoffset by -1in

\abovedisplayskip=6pt plus 3pt minus 1pt
\belowdisplayskip=6pt plus 3pt minus 1pt
\abovedisplayshortskip=0pt plus 3pt
\belowdisplayshortskip=4pt plus 3pt

\def\xskip{\hskip 7pt plus 3pt minus 4pt}


==> mac/m-impl.tex <==
\def\mIncludeGuard{1}

\catcode`@=11 % borrow the private macros of PLAIN (with care)

\input tikz

\input mac/layout
\input mac/fonts
\input mac/sym
\input mac/op
\input mac/bib
\tenpoint

\let\bgroup={
\let\egroup=}

% sections
\newcount\secno
\secno=1
\def\newsec#1{\noindent{\bf\the\secno.\enspace #1. }\global\advance\secno by 1}

% equations
\newcount\equationno
\equationno=1
\def\filleqno#1{\expandafter\xdef\csname eq#1\endcsname{\the\equationno}%
\eqno{\hskip-\rightskip(\the\equationno)\hskip\rightskip}\global\advance\equationno by 1}

% block quotes
\def\beginquote{$$\vbox\bgroup\narrower\ninepoint\noindent}
\def\endquote{\egroup$$}

% fn definitions
\def\fndef#1{\left\{\vcenter{\leftskip=0pt\rightskip=0pt\raggedright\abovedisplayskip=1pt plus 1 pt minus 1pt\parindent=0pt\kern 2pt\relax#1}\right.}

% Figures
\newcount\numfigs
\numfigs=1
\def\displayfigure#1#2#3#4{%
$$\halign{\hbox to \displaywidth{##}\cr
\setbox0=\vbox{\hbox{\input #2 }}
\dimen0=\leftskip\advance\dimen0 by #1
\hskip\dimen0\copy0\dimen0=\ht0
\vbox to \dimen0{\vfil\hbox{#3}\vfil}
\hfil\vbox to \dimen0{
\rightskip=0pt\leftskip=0pt\hsize=2.1in\raggedright\eightpoint\noindent%
{\bf Figure \the\numfigs.\global\advance\numfigs by 1}\ \it%
#4
\vfil
}\cr
}$$}

% Tables
\newcount\numtables
\numtables=1
\def\displaytable#1#2#3#4{%
$$\halign{\hbox to \displaywidth{##}\cr
\setbox0=\vbox{\input #2 }
\dimen0=\leftskip\advance\dimen0 by #1
\hskip\dimen0\copy0\dimen0=\ht0
\vbox to \dimen0{\vfil\hbox{#3}\vfil}
\hfil\vbox to \dimen0{
\rightskip=0pt\leftskip=0pt\hsize=2.1in\raggedright\eightpoint\noindent%
{\bf Table \the\numtables.\global\advance\numtables by 1}\ \it%
#4
\vfil
}\cr
}$$}

% algos
\newdimen\algindent
\def\algindentset#1{\setbox0\hbox{{\bf #1.\kern.25em}}\algindent=\wd0\relax}

\def\algbegin #1 #2{\algindentset{#21}\alg #1 #2} % when steps all have 1 digit
\def\alg#1(#2). {\medbreak % Usage: \algbegin Algorithm A (algname). This...
  \noindent{\bf#1}({\it#2\/}).\xskip\ignorespaces}
\def\aalgbegin #1 #2{\algindentset{#211}\alg #1 #2} % when 10 or more steps

\def\algstep #1.{\smallskip\noindent
  \hbox to\algindent{\bf\hfil #1.\kern.25em}%
  \hangindent=\algindent\hangafter=1\ignorespaces}

\def\algstepbegin #1.{\smallskip\noindent\begingroup%
  \hbox to\algindent{\bf\hfil #1.\kern.25em}%
  \hangindent=\algindent\hangafter=1\ignorespaces
  \everypar={\hangindent=\algindent\ignorespaces}\ignorespaces}

\def\algstepend{\endgroup}
  


==> mac/op.tex <==
\def\argmin{\mathop{\rm arg\,min}}
\def\rank{\mathop{\rm rank}}
\def\sign{\mathop{\rm sign}}
\def\pe{\mathop{\rm pe}}
\def\tr{\mathop{\rm tr}}


==> mac/sym.tex <==

\def\X{{\bf X}}
\def\x{{\bf x}}
\def\e{{\bf e}}
\def\l{{\bf l}}
\def\y{{\bf y}}
\def\r{{\bf r}}
\def\rg{{\fam\bfit \betap}}
\def\rghat{{\bf \hat{\fam\bfit\betap}}}
\def\rgtrue{{\bf \fam\bfit\betap}_{\rm true}}
\def\rgols{\rghat^{\rm OLS}}
\def\Re{{\bbb R}}

\def\F{{\bf F}}
\def\U{{\bf U}}
\def\L{{\cal L}}
\def\A{{\cal A}}
\def\Amat{{\bf A}}
\def\Q{{\bf Q}}
\def\R{{\bf R}}
\def\G{{\bf G}}
\def\H{{\bf H}}
\def\s{{\bf s}}

\def\half{{1\over2}}

\def\u{{\bf u}}
\def\v{{\bf v}}
\def\w{{\bf w}}
\def\nullv{{\bf 0}}

\def\gammab{{\fam\bfit \gammap}}
\def\xib{{\fam\bfit \xi}}

\def\idx#1{^{(#1)}}
\def\idxp#1{^{(#1)\prime}}

\def\phz{\phantom{0}}

\def\eqdef{:=}

\def\qed{\quad\vrule height8pt width2pt depth1pt}

% functions
\def\activer{{\tt active}}
\def\signs{{\tt signs}}
\def\complete{{\tt complete}}
\def\step{{\tt step}}

% \arrows makes things like <--- text --->
\def\arrows#1#2{% #1=width, #2=text
  {\setbox0=\hbox{$\mkern-2mu\mathord-\mkern-2mu$}
    \hbox to #1{\kern-.055556em$\leftarrow\mkern-6mu$%
      \cleaders\copy0\hfil
      \kern.4em #2\kern.4em
      \cleaders\copy0\hfil
      $\mkern-6mu\rightarrow$\kern-.055556em}}}

\def\arrowfill#1{%
\setbox0=\hbox{$\mkern-2mu\mathord-\mkern-2mu$}%
\kern-0.055556em$|\mkern-8mu\leftarrow\mkern-6mu$\cleaders\copy0%
\hfil\kern.4em{}#1\kern.4em\cleaders\copy0\hfil%
$\mkern-6mu\rightarrow\mkern-8mu|$}


==> table/bench-sim.tex <==
\sevenpoint%
\tabskip=15pt\halign{
\hfil # \hfil& \hfil # \hfil & \hfil # \hfil & \hfil # \hfil& \hfil # \hfil\cr
& & & Num Active & Avg Elapse Over\cr
n & p & k & Regressors & 10 Runs (sec)\cr\noalign{\smallskip}
\phz800 & \phz800 & 10 & \phz38.4 & \phz12.05\cr
\phz800 & \phz800 & 50 & \phz70.4 & \phz20.81\cr
\phz800 & 1600 & 10 & \phz57.3 & \phz36.90\cr
\phz800 & 1600 & 50 & \phz92.0 & \phz59.27\cr
1600 & \phz800 & 10 & \phz51.0 & \phz52.01\cr
1600 & \phz800 & 50 & 110.0 & 101.34\cr
1600 & 1600 & 10 & \phz86.2 & 227.33\cr
1600 & 1600 & 50 & 106.4 & 217.25\cr
}


==> table/bench-sim2.tex <==
\sevenpoint%
\tabskip=5pt\halign{
\hfil # \hfil& \hfil # \hfil & \hfil # \hfil \quad & 
\hfil # \hfil& \hfil # \hfil & \hfil # \hfil \quad & 
\hfil # \hfil& \hfil # \hfil & \hfil # \hfil\cr
& & & \omit\span\omit\span \hfil \strut LO\hfil &
\omit\span\omit\span \hfil \strut ALO\hfil \cr\noalign{\smallskip}
& & & 
Num Active & Prediction & Avg Elapse Over & 
Num Active & Prediction & Avg Elapse Over\cr
n & p & k 
& Regressors & Error & 10 Runs (sec)
& Regressors & Error & 10 Runs (sec)\cr\noalign{\smallskip}
\phz800 & \phz800 & 10 & \phz47.2 & 0.075 & \phz13.42 & \phz44.8 & 0.075 & \phz0.026 \cr
\phz800 & \phz800 & 50 & \phz68.2 & 0.136 & \phz16.75 & \phz50.0 & 0.137 & \phz0.025 \cr
\phz800 & 1600 & 10 & \phz58.6 & 0.090 & \phz28.90 & \phz32.5 & 0.088 & \phz0.039 \cr
\phz800 & 1600 & 50 & \phz60.0 & 0.182 & \phz36.18 & \phz49.5 & 0.184 & \phz0.048 \cr
1600 & \phz800 & 10 & \phz48.2 & 0.033 & \phz45.22 & \phz52.2 & 0.033 & \phz0.061 \cr
1600 & \phz800 & 50 & 118.8 & 0.096 & 101.23 & 114.5 & 0.095 & \phz0.085 \cr
1600 & 1600 & 10 & \phz62.7 & 0.060 & 166.56 & \phz75.4 & 0.058 & \phz0.139 \cr
1600 & 1600 & 50 & 123.5 & 0.113 & 235.81 & 105.7 & 0.113 & \phz0.164 \cr
}



==> table/benchmark.tex <==
\sevenpoint%
\tabskip=10pt\halign{
\kern-6em\hfil# & 
\hfil# & \hfil# &
\hfil#\hfil &
\hfil#\hfil &
\hfil#\hfil
& \hfil#\hfil\cr
&&& 
Num Active &  & &
Avg Elapse Over\cr
Dataset & n & p & 
Regressors & 
\smash{$t / \sum_j|\beta_j^{\rm OLS}|$} & 
LO &
5 Runs (sec)\cr\noalign{\vskip 5pt}
\tt diabetes & 442 & \phz10 & \phz\phz7 & 0.55 & 0.50 & \phz\phz0.004\cr
\tt California housing & 20640 & \phz8 & \phz\phz8 & 0.97 & 0.40 & \phz\phz0.092\cr
\tt diabetes (Q) & 442 & 64 & \phz15 & 0.03 & 0.49 & \phz\phz0.220\cr
\tt riboflavin (E) & 71 & 4088 & \phz20 & 0.23 & 0.24 & \phz\phz0.571\cr
\tt SARCOS inverse & 44484 & 21 & \phz20 & 0.99 & 0.07 & \phz\phz1.161\cr
\tt California housing (Q) & 20640 & 44 & \phz39 & 0.33 & 0.35 & \phz\phz2.680\cr
\tt riboflavin & 71 & 4088 & \phz20 & 0.23 & 0.24 & \phz\phz3.385\cr
\tt SARCOS inverse (QE) & 44484 & 252 & \phz58 & 0.09 & 0.05 & \phz16.351\cr
\tt SARCOS inverse (Q) & 44484 & 252 & 252 & 0.99 & 0.03 & 349.229\cr
}



==> table/diabetes-optimums.tex <==
\sevenpoint
\halign{\indent# \quad & \hfil# \hfil\quad & \tt# \cr
$t/\sum_{j=1}^p |\hat{\beta}_j^{\rm OLS}|$ & LO &\omit Active Regressors\hfil\cr\noalign{\smallskip}
\hfil0.360\hfil & 0.52952 & BMI, LTG, BP, HDL\hfil\cr
\hfil0.442\hfil & 0.51180 & BMI, LTG, BP, HDL, Sex, GLU\hfil\cr
\hfil0.548\hfil & 0.50052\rlap{*} & BMI, LTG, BP, HDL, Sex, GLU, TC\hfil\cr
\hfil0.597\hfil & 0.50058 & BMI, LTG, BP, HDL, Sex, GLU, TC, TCH\hfil\cr
\hfil0.819\hfil & 0.50090 & BMI, LTG, BP, Sex, GLU, TC, TCH, LDL, Age\hfil\cr
\hfil0.860\hfil & 0.50182 & BMI, LTG, BP, HDL, Sex, GLU, TC, TCH, LDL, Age\hfil\cr
\hfil0.887\hfil & 0.50178 & BMI, LTG, BP, HDL, Sex, GLU, TC, TCH, LDL, Age\hfil\cr
}


==> table/diabetes-preview.tex <==
\sevenpoint
\tabskip=2.5pt\halign{\hfil# \hfil& \hfil# \hfil& \hfil# \hfil& \hfil# \hfil& \hfil# \hfil&
\hfil# \hfil& \hfil# \hfil& \hfil# \hfil& \hfil# \hfil& \hfil# \hfil& \hfil# \hfil& \hfil\quad#\hfil\cr
& \hfil Body Mass\hfil & & & \hfil Blood \hfil\cr
& \hfil Index\hfil & & & \hfil Pressure \hfil &
\multispan6\arrowfill{Blood Measurements}\phantom{x}&
\hfil Progression \hfil \cr\noalign{\vskip 1pt}
Patient & \hfil BMI\hfil & Age & Sex & \hfil BP\hfil &
TC & LDL & HDL & TCH & LTG & GLU & \hfil of Diabetes\hfil\cr\noalign{\smallskip}
\phz\phz1 & 32.1 & 59 & F & 101 &
157 & \phz93.2 & 38 & 4 & 4.9 & 87 &
151\cr
\phz\phz2 & 21.6 & 48 & M & \phz87 & 183 & 103.2 & 70 & 3 & 3.9 & 69 & \phz75\cr
\vdots & \vdots & \vdots & \vdots & \vdots & \vdots & \vdots & \vdots &
\vdots & \vdots & \vdots & \vdots\cr
441 & 30.0 & 36 & M & 95 & 201 & 125.2 & 42 & 5 & 5.1 & 85 & 220\cr
442 & 19.6 & 36 & M & 71 & 250 & 133.2 & 97 & 3 & 4.6 & 92 & \phz57\cr
}


==> table/riboflavin-preview.tex <==
\sevenpoint\tabskip=2.5pt
\halign{\indent\hfil # \hfil & \hfil # \quad \hfil & \hfil # \hfil 
& \hfil # \hfil & \hfil # \hfil & \hfil # \hfil
& \hfil # \hfil & \hfil \quad# \hfil\cr
& \multispan6\arrowfill{4088 Genes} & Log Riboflavin\cr\noalign{\vskip 1pt}
Sample & AADK\_at & AAPA\_at & ABH\_at & $\cdots$ & YYZB\_at & zur\_at &
Production Rate
\cr\noalign{\smallskip}
\phz1 & 8.492 & 8.111 & 8.321 & $\cdots$ & 7.173 & 7.427 & -6.644\cr
\phz2 & 7.639 & 7.240 & 7.793 & $\cdots$ & 7.187 & 7.545 & -6.948\cr
\vdots & \vdots & \vdots & \vdots & $\ddots$ & \vdots & \vdots & \vdots\cr
70 & 7.343 & 7.743 & 7.709 & $\cdots$ & 7.539 & 7.310 & -6.764\cr
71 & 6.856 & 8.275 & 7.989 & $\cdots$ & 7.230 & 6.656 & -7.587\cr
}


==> table/sim1.tex <==
\sevenpoint\tabskip=5pt
\halign{%
\hfil#\hfil & \hfil# \hfil& \hfil#\hfil \quad & \hfil# \hfil& \hfil#\hfil & \quad\hfil#\hfil  & \hfil#\hfil \quad & 
\hfil#\hfil & \hfil#\hfil\cr
& Num & Prediction & 
\omit\span\hfil \strut 5-fold \hfil &
\omit\span\omit \hfil \strut 10-fold \hfil &
\omit\span\omit \hfil \strut LO \hfil \cr
t & Active & Error & 
Bias & Var &
Bias & Var &
Bias & Var\cr\noalign{\vskip 2pt}
\input data/sim1-data
}


==> table/sim2.tex <==
\sevenpoint\tabskip=2em\halign{\hfil# & \hfil#\hfil & \hfil#\hfil & \hfil#\hfil\cr
& $t$ & Num Active & Prediction Error\cr\noalign{\vskip 5 pt}
oracle optimum & 0.819 & 15.93 & 0.194\cr
LO optimum & 0.959 & 15.62 & 0.217\cr 
\noalign{\vskip7pt}
delta (${\rm LO} - {\rm oracle}$) & 0.140 & -0.31 & 0.024\cr
stddev of delta & 0.640 & \phz7.54 & 0.063\cr
}

